On the Role of Attention in Prompt-tuning

Prompt-tuning is an emerging strategy to adapt large language models (LLM) to downstream tasks by learning a (soft-)prompt parameter from data. Despite its success in LLMs, there is limited theoretical understanding of the power of prompt-tuning and the role of the attention mechanism in prompting. In this work, we explore prompt-tuning for one-layer attention architectures and study contextual mixture-models where each input token belongs to a context-relevant or -irrelevant set. We isolate the role of prompt-tuning through a self-contained prompt-attention model. Our contributions are as follows: (1) We show that softmax-prompt-attention is provably more expressive than softmax-self-attention and linear-prompt-attention under our contextual data model. (2) We analyze the initial trajectory of gradient descent and show that it learns the prompt and prediction head with near-optimal sample complexity and demonstrate how prompt can provably attend to sparse context-relevant tokens. (3) Assuming a known prompt but an unknown prediction head, we characterize the exact finite sample performance of prompt-attention which reveals the fundamental performance limits and the precise benefit of the context information. We also provide experiments that verify our theoretical insights on real datasets and demonstrate how prompt-tuning enables the model to attend to context-relevant information.

==> asymp_01_26.tex <==
\section{Contrasting Population Error of \Prml with Baselines}

\subsection{Insight from the discrete dataset model}
In this section, we establish separation results between \Prml and the baselines of self-attention and linear attention. We will accomplish this focusing on the discrete dataset model where irrelevant tokens are noiseless ($\z_t=0$ for $t\in[T]$).

We first observe that if $\del=(\delq,\delw)$ admits a single value, even a linear model can solve our discrete dataset model.
\begin{observation}[Linear model solves simple discrete data] \label{obv 1}Suppose $\delq=\Delta^q$ and $\delw=\Delta^w$ almost surely for two scalars $\Delta^q,\Delta^w$. Set $\wstar'=(\Iden-\qstab\qstab^\top)\wstar$.
As long as $\Delta^w\neq \zeta/(1-\zeta)$ and $\wstar'\neq 0$, then, $\flin(\wstar')$ or $\flin(-\wstar')$ achieves perfect accuracy.
\end{observation}
This means that, in order to test the expressivity of $\fat,\fsat,\flin$, $(\delq,\delw)$ should better have two or more values. Perhaps surprisingly, we prove that, as soon as, $(\delq,\delw)$ is a binary distribution, $\fsat,\flin$ can indeed provably fail. Importantly, this failure happens in the regime $\delq\leq 0$ where \prml thrives. %\todoasr{@Samet: In Sec.~\ref{sec:data_model} you are assuming that $\delta^q \in \{0, \Delta\}$.}

%I relaxed it now. I just made it more general \delta_q,\delta_w as long as \delta_q<=0 % Okay, sounds good.

\begin{theorem}[Separation of Population Accuracy] \label{separate thm} Consider the discrete dataset model where we set $\bSi=0$ in \eqref{eq:CGMM}. The following statements hold:
\begin{enumerate}
% be the projections of $\qstar,\wstar$ on the orthogonal complements of each other respectively
\item \textbf{\Prml:} Set correlation coefficient $\rho=\wstab^\top\qstab$. Suppose $\rho^2<1$, $\delq\geq 0$, and $|\delw|\leq C$ almost surely. Define $\qstar'=(\Iden-\wstab\wstab^\top)\qstar,\wstar'=(\Iden-\qstab\qstab^\top)\wstar$. For $\Gamma>\frac{1}{\tn{\qstar}^2(1-\rho^2)}\log(\frac{C(1-\zeta)}{\zeta})$, by choosing $\thetab=(\wstar',\Gamma\qstar')$, $\fat_{\thetab}$ achieves perfect classification accuracy on \eqref{eq:CGMM}.
\item  \textbf{Self-attention:} In \eqref{eq:CGMM}, choose $(\delq,\delw)$ to be $(0,0)$ or $(\red{\Delta,\Delta})$ equally-likely with $\Delta>(1-\zeta)^{-2}$. 
\begin{itemize}
\item For any choice of $(\Vb=\ones\vb^\top,\W)$, $\fsat(\ones\vb^\top,\W)$ achieves 50\% accuracy (i.e.~random guess).
\item For any choice of $(\Vb,\W)$, there exists a \eqref{eq:CGMM} distribution with adversarial relevance set choices such that $\fsat(\Vb,\W)$ achieves 50\% accuracy.
\end{itemize}


\item  \textbf{Linear \Prml:} In \eqref{eq:CGMM}, choose $(\delq,\delw)$ to be $(0,0)$ or $(\red{\Delta,-\Delta})$ equally-likely with $\Delta>\sqrt{\zeta/(1-\zeta)}$. For any choice of $(\w,\qb)$, $\flinatt(\w,\qb)$ achieves at most 75\% accuracy.
\end{enumerate}
\end{theorem}
\begin{figure}%\vspace{-23pt}
\begin{center}
    \includegraphics[width=0.4\textwidth]{baselines.pdf}
    \end{center}
  \vspace{-18pt}
  \caption{\small{This figure depicts the outcome of our Theorem \ref{separate thm}.}}
  %is treated as a machine learning algorithm that 
  %$prefix, and we utilize auto-regressive transformers. $
  \label{fig:icl}%\vspace{-12pt}
  %\vspace{-10pt}
\end{figure} 
Above, all results, with the exception of self-attention with general $\Vb$, hold for arbitrary, including adversarial, relevance set choices. The reason is that tokens are pooled and the particular choice of $\Rc$ does not matter. Only for $\fsat(\Vb,\W)$, we need to adapt the relevance set $\Rc$ to the output layer $\Vb$ (as well as $(y,\del)$ variables) to facilitate misclassification. Otherwise, with the hindsight knowledge of the relevance set, $\Vb$ can intelligently process individual tokens of the self-attention output to filter out ``confusing'' tokens. \red{To be more concrete, for the same dataset model (equally-likely over $(0,0),(\Delta,\Delta)$), self-attention can achieve perfect accuracy by choosing $\Vb=\ones_{\Rc}\wstar^\top$ where $\ones_{\Rc}$ is the vector of ones over the relevant set $\Rc$ that filters out the attention outputs associated to the irrelevant tokens (see Lemma \ref{lem satt success}).} 

At a high-level, the reason \prml can provably beat self-attention is simple: \Prml is optimized for the context and cleanly \emph{attends} the relevant contextual information. In contrast, self-attention scores are fully feature-based, this means that, contextual information is mixed with other features and can be lost during aggregation of the attention output.

%Here, adversarial relevance set means that, $\Rc$ can be chosen adaptively to the label $y$, out-of-context term $\del$, and the self-attention model weights $(\Vb,\W)$ to cause misclassification.

\subsection{Sharp Characterization of Accuracy} 
While discrete dataset model is insightful, incorporating noise is crucial for understanding the fundamental limits of the benefits of context in attention. To this end, let us focus on the core dataset model where we set $\delq=\delw=0$ and explore the role of noise in population accuracy. Also assume that noise is standard normal (i.e.~$\subg{\bSi}:=\Nn(0,\Iden)$. 

\noindent$\bullet$  \emph{Linear model.} Observe that linear model aggregates tokens to obtain a simple Gaussian mixture distribution. Specifically, aggregated tokens are exactly distributed as $\frac{1}{T}\X^T\ones_T\sim \Nn(\zeta\wstar,\frac{1-\zeta}{T}\Iden)$ where $\zeta$ is the sparsity level. This leads to the following well-known result.
\begin{fact} For linear models, optimal accuracy obeys $\min_{\w} \acc(\flin(\w))=Q(\sqrt{\frac{\zeta^2T}{1-\zeta}}\tn{\wstar})$ where $Q(\cdot)$ is the tail function of the standard normal distribution.
\end{fact}

Thus, the linear model can achieve small error as long as $\tn{\wstar}\gtrsim \sqrt{T}/\zeta$.

%$\bullet$ \textbf{Linear model.} Suppose $\bSi=\Iden$ and assume noise is Gaussian and denote the standard normal tail by $Q(\cdot)$. Let $g\sim\Nc(0,1)$. For any $\w$, we have that $y\flin(\w)\sim y\w^\top\wstar+\w^\top\qstar+g\sqrt{\frac{1-\zeta}{T}}\tn{\w}$. Thus, the error is minimized by setting $\w=\wstar/\tn{\wstar}$ and we have


\noindent$\bullet$ \emph{\Prml model.} Since \prml strictly generalizes linear model, its accuracy has to be at least as good. The theorem below quantifies this and demonstrates that how \ctx vector can enable an optimal weighting of relevant and irrelevant tokens to maximize accuracy.



\begin{theorem}\label{thm sharp and precise} Consider the \prml model $\fat_{\thetab}$. Set $Q=\tn{\qstar}^2,W=T\tn{\wstar}^2$, suppose $\wstar\perp\qstar$, and let $\taut,\taub>0$ be hyperparameters. Consider the following algorithm which uses the hindsight knowledge of $\qstar$ to estimate $\wstar$ and make prediction:
\begin{enumerate}
\item $\hat{\w}=(\Iden-\qstab\qstab) \nabla \Lc_{\w}(0,\taut\qstab)$.
\item Set $\thetab=(\hat{\w},\taub\qstab)$.
\end{enumerate}
Suppose $\zeta^2W,1-\zeta,\alpha:=n/d,e^Q,e^\taut$ each lie between two positive absolute constants. Suppose $T$ is polynomially large in $n$ and these constants and $\ordet{\cdot}$ hides polynomial terms in $n$. Define \emph{inverse-signal-to-noise-ratio}: $\isnr{\alpha,\taut}=\frac{(1-\zeta)e^{2\taut(\taut-\sqrt{Q})}}{\alpha\zeta^2W}$. With probability $1-2e^{-t^2/2}-\ordet{T^{-1/3}}$ over the training data, the test error obeys $\err(\fat_{\thetab})=$
\[
 \Qc\left(\frac{e^{\sqrt{Q}\taub-\taub^2}}{\sqrt{1+(1\mp\frac{1+t}{\sqrt{d}})\isnr{\alpha,\taut}}}\cdot \sqrt{\frac{\zeta^2W}{1-\zeta}}\right)\pm \ordet{T^{-1/3}}.
\]
Above, $\mp,\pm$ highlights the upper/lower range of the test error (see \eqref{exact Q bound} for exact statement). In the limit $T,d\rightarrow\infty$, the test error converges in probability to 
\[
\err(\alpha,\zeta,Q,W,\taut,\taub)=\Qc\left(\frac{e^{\sqrt{Q}\taub-\taub^2}}{\sqrt{1+\isnr{\alpha,\taut}}}\cdot \sqrt{\frac{\zeta^2W}{1-\zeta}}\right)
\]
In this limit, optimal hyperparameters are $\taut=\taub=\sqrt{Q}/2$ and leads to optimal $\isnr{\alpha}:=\frac{(1-\zeta)e^{-Q/2}}{\alpha\zeta^2W}$ and the error
\[
\err(\alpha,\zeta,Q,W)=\Qc\left(\frac{e^{Q/4}}{\sqrt{1+\isnr{\alpha}}}\cdot \sqrt{\frac{\zeta^2W}{1-\zeta}}\right)
\]
\end{theorem}

\red{Here, a few remarks are in place. First, we remark that when $Q=0$, our bound reduces to $\Qc\left(\sqrt{\frac{\zeta^2W}{1-\zeta}}\right)$\dots}

==> attn_model.tex <==
\section{Problem setting}
\label{sec:problem-setting}

\subsection{Motivation: Prompt-tuning}
\label{sec:motivation}
Consider a single-head self-\Attn layer
\begin{align}\label{eq:self-attn}
\Ob_\pre = 
\sft{\X\WQ\WK^\top\X^\top}\X\WV
\end{align}
with input $\X\in\R^{T\times d}$ consisting of $T$  tokens of dimension $d$ each, trainable parameters $(\WK,\WQ,\WV)$ and a softmax nonlinearity $\phi:\R^T\mapsto\R^T$, $[\phi(\vb)]_t=e^{v_t}/\sum_{t'\in[T]}e^{v_{t'}}$ that acts row-wise on matrix $T\times T$. We scalarize the output of the self-\Attn output with a trainable linear head $\bar{\Ub}$ which yields
\begin{align}\label{eq:self-attn-scalar-output}
y_\pre=\inp{\bar{\Ub}}{\Ob_\pre}=\inp{\Ub}{\sft{\X\WQ\WK^\top\X^\top}\X}
\end{align}
%for trainable $\Ub\in\R^{T\times d}$.
Note here that we implicitly subsume the value matrix $\WV$ in the linear head via $\Ub:=\bar{\Ub}\WV^\top$.

We assume that the model above is pre-trained so that $\WK,\WQ,\Ub$ are fixed. Our goal is to use the pretrained transformer on (potentially) new classification tasks. Towards this goal, we explore the use of prompt-tuning, introduced in \citet{li2021prefix, lester2021power} as an alternative to fine-tuning the existing transformer weights. 

Prompt-tuning appends a trainable prompt $\Pbb\in\R^{m\times d}$ to the input features $\X\in\R^{T\times d}$ with the goal of conditioning the transformer to solve the new classification task. Let $\Xp:=\begin{bmatrix}\Pbb\\\X\end{bmatrix}\in\R^{(T+m)\times d}$ be the new transformer input. The output of the \Attn-layer is thus is of the form
$$
\Ob=\sft{\Xp\WQ\WK^\top\X^\top}\X.
$$
Note that this is slightly different from  \eqref{eq:self-attn} in that now the layer computes a cross-\Attn between the augmented inputs $\Xp$ and the original inputs $\X$. This is also equivalent to self-attention on $\Xp$ after masking the prompt $\Pbb$ from keys. {This masking is used to cleanly isolate the residual contribution of the prompt without impacting the frozen attention output. Concretely, l}et $\W$ be the prediction head associated with the prompt tokens. As before, we scalarize the output by projecting with a linear head of size $(T+m)\times d$ as follows:%\begin{bmatrix}\W\\\Ub\end{bmatrix}
\begin{align}
y&=\inp{[\W^\top~\Ub^\top]^\top}{\sft{\Xp\WQ\WK^\top\X^\top}\X}\label{eq:prompt-output-general}
\\
&= \underbrace{\inp{\W}{\sft{\Pbb\WQ\WK^\top\X^\top}\X}}_{\text{prompt-attention $y_\new$}}+\underbrace{\inp{\Ub}{\sft{\X\WQ\WK^\top\X^\top}\X}}_{\text{frozen self-attention $y_\pre$}} \nn.
\end{align}
Here, $y_\new$ captures the additive impact of prompt-tuning on the prediction. We denote the trainable parameters in the model above as $\thetab:=(\W,\Pbb)$. Since the $y_\new$ term becomes a self-contained module and the features attend directly to the prompt vector, we will refer to it as \emph{prompt-attention}.

Our goal is understanding the expressivity, training dynamics, and generalization properties of the above model. To simplify our analysis, we consider the following setting.

\begin{enumerate}
    \item We focus our attention on the novel component $y_\new$ of the model output in \eqref{eq:prompt-output-general} so as to isolate and fully understand the capabilities of prompt-attention.
    %{\red{Add remark that can potentially take care of by blowing up $\W$ in training. Can we assume $\Ub$ is small and do perturbation argument. Add lemma if perturbation small then things don't change.}}
    \item We assume $\WK,\WQ\in\R^{d\times d}$ are full-rank.
    %and for further simplicity $\WK=\WQ=\mtx{I}_d.$\red{Really the only thing we need here is full-rank and then optimal $\Pb$ is $\WQK^{-1}\qstar$}
    \item We assume a single trainable prompt $\qb\in\R^d$ i.e.,~$m=1$.% and $\Pbb=\pb$.
\end{enumerate}

% \red{Discuss above simplifications} \red{Also potentially discuss role of prompting. Why in this model prompting can be even better than self-\Attn.}

\textbf{Prompt-attention model.} Using these assumptions and setting $\qb:=\WK\WQ^\top \Pbb^\top\in\R^d$ and $\w=\W^\top\in\R^d$, we arrive at our core \emph{prompt-attention} model
\begin{align}
    f_{\thetab}(\X) = \inp{\w}{\X^\top\phi\left(\X\qb\right)}, \quad\thetab=(\w,\qb).\label{eq:PA}%\tag{}
\end{align}
We shall see that this model exhibits exciting properties to learn rich contextual relationships within the data and can even be more expressive than a single self-attention layer.

We remark that the model above is of interest even beyond the context of prompting: the \prml model in \eqref{eq:PA} is reminiscent of  the simplified model proposed in earlier seq2seq architectures \cite{bahdanau2014neural,xu2015show,chan2015listen} preceding self-attention and \Tfs \cite{vaswani2017attention}. Indeed, in  the simplified attention mechanism of \cite{bahdanau2014neural,xu2015show,chan2015listen}, the tokens' \emph{relevance scores} and corresponding \emph{attention weights} are determined by $\ab=\phi(\X\qb)$ in which $\qb$ is a trainable vector and $\phi$ is the softmax score transformation. Note here that the trainable parameter $\qb$ corresponds exactly to the trainable prompt vector in \eqref{eq:PA}.

\subsection{Contextual data model}
\label{sec:data_model}
Consider supervised classification on IID data $(\X,y)\sim \Dc$ with features $\X\in\R^{T\times d}$ and binary label $y\in\{\pm1\}$.  

\noindent\textbf{Dataset model:} We assume the following about an example $(\X,y)$ drawn from $\Dc$: The labels $y$ are distributed as $\Pro(y=1)=1-\Pro(y=-1)=\pi$; for simplicity, we set $\pi=1/2$ so that $\E[y]=0$. The tokens $\x_t,t\in[T]$ of input example $\X:=[\x_{1},\ldots,\x_{T}]$ are split into a \emph{\ctx-relevant} set $\Rc\subset [T]$ and \emph{\ctx-irrelevant} set $\Rcc:=[T]-\Rc$. Specifically, conditioned on the labels and relevance set $\Rc$, tokens $\x_t, t\in[T]$ within $\X$ are i.i.d.~as follows 
\begin{equation}%\label{eq:CGMM-main}
\x_t | y = \begin{cases}
\qstar + y \wstar &, 
t\in\Rc
~~~~~~\text{(relevant token)}
\\
-\delq\qstar-\delw y\wstar+\z_t 
&, 
t\not\in\Rc~~~~~~\text{(\textbf{ir}relevant token)}\,.%-\qstar\qstar^\top
\end{cases}\label{eq:CGMM}\tag{DATA}
\end{equation}
In the above, $\qstar$ is a \ctx-vector that indicates token relevance and $\wstar$ is a regressor vector. $y,\del:=(\delq,\delw), (\z_t)_{t=1}^T$ are independent variables as follows: 

\noindent$\bullet$~$\del=(\delq,\delw)\in\R^2$ is a bounded random variable that obeys $\delq\geq 0$. Thus, $\del$ reflects \emph{out-of-context} information within irrelevant tokens. However, $\del$ is allowed to expose label information through $\delw$. When $\del=(0,0)$ almost surely, we call the resulting distribution \textbf{core dataset model}.  % since $\delq\geq 0$.
%\todoasr{What do you mean by ``either positive or negative''?}

\noindent$\bullet$~$\z_t$ are independent centered subgaussian and random variables with covariance $\bSi$ (see Ass. \ref{ass:noise}). When $\bSi=0$, we call the resulting distribution \textbf{discrete dataset model}.

\noindent$\bullet$~We allow the relevance set $\Rc$ to be non-stochastic. This includes $\Rc$ being adversarial to the classification model.

\noindent$\bullet$~We assume constant fraction $\zeta=|\Rc|/T\in(0,1)$ of  label-relevant tokens for each input example $\X$ drawn from $\Dc$. Thus,  $\zeta$ represents the sparsity of relevant signal tokens.

\noindent\textbf{Training dataset $\Sc:=(\X_i,y_i)_{i=1}^n$.} We draw $n$ i.i.d.~samples from $\Dc$ to form our training dataset $\Sc:=(\X_i,y_i)_{i=1}^n$. For $i$'th example $(y_i,\X_i)$, we denote the tokens by $(\xti)_{t=1}^T$, noise by $(\zti)_{t=1}^T$, relevance set by $\Rc_i$, and out-of-context variable by $\del_i=(\delq_i,\delw_i)$.


%and $\order{\|\bSi\|}$ subgaussian norm
 Ideally, for each example $i$, we would like to identify its \ctx-relevant set $\Rc_i$ and discard the rest: This would especially help when the signal-to-noise-ratio is small, i.e. $\zeta=|\Rc_i|/T\ll 1$. This is precisely the role of the \ctx-vector $\qstar$: Observe that, per our construction, relevant tokens have positive correlation with $\qstar$ whereas irrelevant tokens have non-positive correlation with $\qstar$ in expectation. Thus, by focusing attention onto tokens based on their $\qstar$ correlation, we can potentially select the relevant set.

 %\ct{Say that $\Rc$ can vary with $i$}

 \begin{remark}[Model interpretation.] \eqref{eq:CGMM} can be thought of as a simplified model for binary image classification with tokens being image patches of two types: ones revealing information about the label (set $\Rc$) and uninformative ones containing noise. Tokens in $\Rc$ contain information indicating: (i) class-membership via signed-regressor $y\wstar$ and (ii) \ctx-relevance via \ctx-vector $\qstar$. The signed-regressor differs across tokens of examples belonging to different classes $y\in\{\pm1\}$, while the \ctx-vector is common for all \ctx-relevant tokes across classes. For a concrete example, consider images each depicting multiple, say $|\Rc|$, birds of one type on label-irrelevant / noisy background. The goal is to classify images according to one of two types of birds. Here, think of ``\ctx'' as feature-information indicating corresponding pixels belong to ``bird'' (of either type) rather than ``background,'' while the ``regressor'' represents feature information useful to distinguish between two bird types. Alternatively, \eqref{eq:CGMM} may be modeling deep representations (rather than raw pixels) of the original images. Overall, simplified models similar to \eqref{eq:CGMM} have been used previously to analyze optimization and generalization dynamics of training fully-connected \cite{frei2022random} and convolutional models \cite{cao2022benign}. Specifically, \eqref{eq:CGMM} is an extension of the commonly used (sub)-Gaussian mixture model customized to the nature of \Attn: each example is tokenized and \ctx-relevant information ist described in terms of both a regressor (differing between classes) and a \ctx (common across classes).
 \end{remark}

% \begin{equation}
% \x_t | y = \begin{cases}
% \qstar^{\ell} + y \wstar & \text{w.p.}~ \zeta~~~~~~~~\text{(a.k.a.~relevant token)}
% \\
% \z_t \sim \subg{\sigma^2\Iden} & \text{w.p.}~ 1-\zeta~~~~\text{(a.k.a.~irrelevant token)}%-\qstar\qstar^\top
% \end{cases}\label{eq:CGMM}
% %\,,\qquad  \qb_{t,\star}^\perp \text{ zero-mean stochastic}
% \end{equation}

% \begin{equation}
% \x_t  = \begin{cases}
% \qstar^{\ell}+\z_t & \text{w.p.}~ \zeta~~~~~~~~\text{(a.k.a.~relevant token)}
% \\
% \z_t \sim \subg{\sigma^2\Iden} & \text{w.p.}~ 1-\zeta~~~~\text{(a.k.a.~irrelevant token)}%-\qstar\qstar^\top
% \end{cases}\label{eq:CGMM}
% \qquad y=f(\sum_{t\in\Gc}\wstar^\top\x_t)
% %\,,\qquad  \qb_{t,\star}^\perp \text{ zero-mean stochastic}
% \end{equation}



%\input{sec/insights}

% \subsection{\Prml Model}
% \label{sec:pmt-attn}

% The \Attn  mechanism  extracts the relevant information within high-dimensional features. This idea is best captured through the simplified \Attn model proposed in earlier seq2seq architectures preceding \Tfs \cite{bahdanau2014neural,xu2015show,chan2015listen}. We refer to this earlier model as \emph{\prml} to distinguish from self-\Attn \cite{?}. In the \prml model \cite{bahdanau2014neural,xu2015show,chan2015listen}the tokens' \emph{relevance scores} / \emph{attention weights} are determined by $\ab=\phi(\X\qstar)$ in which $\qstar$ is a vector that dictates label-relevance and $\phi(\cdot):\R^\top\rightarrow \R^\top$ is a score transformation. Concretely, $\sft{}:\R^\top\rightarrow\R^\top$ is the softmax nonlinearity, i.e. $[\sft{\vb}]_t=\exp(v_t)/\sum_{\tau\in[T]}{v_\tau}$ for vector for vector $\vb=[v_1,\ldots,v_T]^\top.$
%  Thus, the \prml layer $\X\in\R^{T\times d}$ outputs $\X^\top\phi(\X\qstar)=\X^\top\ab$. This output representation is then transformed to a label prediction through a prediction head. Overall, denoting trainable parameters by 
% %Let $\ab[t]$ be the $t$'th entry of a vector. Let $\sft:\R^\top\rightarrow\R^\top$ be the function that generates attention weights. We consider a simple attention model $\fat$ parameterized by query vector $\qb\in\R^d$ and prediction head $\w\in\R^d$.
% %Denote model parameters by 
% $\thetab=(\w,\qb)$, the \prml model $\fat$ predicts
% %Given tokenized features $\X$, this model predicts
% \begin{align}\label{eq:PA}
% \fat_{\thetab}(\X) &= \w^\top\X^\top\ab  =  \sum_{t\in[T]} [\ab]_t \w^\top\x_t \quad\text{where}\\
% \ab&=\sft{\X\qb}=\exp(\X\qb)/\ones^\top\exp(\X\qb).
% \end{align}
% %\textcolor{red}{MS: fixed a typo as before it was $\fat_{\thetab}(\X) = \w^\top\X\ab$}

% %\noindent\red{\textbf{Concern:} Using $\sft{|\X\wstar|}$ will solve our dataset without a need for $\qstar$. Similarly, if we motivate prompt-tuning, observe that $\WK=\WQ=\wstar$ might solve the self-attention because $\X\X^\top\sim \wstar\wstar^\top$ (i.e.~label sign doesn't matter). This hurts our fine-tuning argument as query-vector is irrelevant for self-attention model.\\
% %\textbf{Potential resolution:} The way to fix this issue is allowing $\zti \sim \subg{\sigma_i\wstar,\bSi}$ where $(y_i,\sigma_i)\in \{\pm 1,\pm \sigma\}$ with a joint distribution. Here, $\sigma_i$ can now adversarially hurt the label raising the need for query. This can also further distinguish from the other papers.}



\subsection{Baseline Models}
We compare performance of the \prml model in \eqref{eq:PA} with the following three baseline models.

\noindent\textbf{The linear model} is parameterized by $\thetab=\w$ and outputs
\begin{align}\label{eq:linear_model}
\flin(\w) = \frac{1}{T}\w^\top\X^\top\ones_T=\frac{1}{T}\sum_{t\in[T]}\w^\top\x_t.
\end{align}
Note  this corresponds to a \prml model with uniform attention weights $[\ab]_t=1/T, t\in[T].$

\noindent\textbf{The self-\attn model} model is a strict generalization of the linear model. Recalling \eqref{eq:self-attn-scalar-output}, let us merge the key-query weights $\W:=\W_Q\W_K^\top$ (without losing generality) and gather weights into $\thetab=(\Ub,\W)$. We then write it as
%and
\begin{align}\label{eq:satt_model}
\fsat(\Ub,\W) = \frac{1}{T}\li\Ub,\sft{\X\W\X^\top}\X\ri.
\end{align}
%where $\Vb\in \R^{T\times d}$. Following remarks are in place: Self-attention with a linear head can be more explicitly written as $\fsat=\frac{1}{T}\li\Vb,\sft{\X\W_Q\W_K^\top\X^\top}\X\W_V\ri$ where $\Vb$ is the linear head and $\W_K,\W_Q,\W_V$ are the key/query/value weights. Thus, above, without losing any generality, (key, query) weight matrices are merged under the weights $\W$ and the value weights are merged with the linear head. 
Rather than using a $Td$ dimensional $\Vb$, we will also consider the simpler token-pooling via $\Vb=\ones_T\vb^\top$ for $\vb\in\R^d$.

%Secondly, all tokens are pooled after inner product with $\w\in\R^d$. The reason is that the \ctx-relevant set is allowed to be adversarial which nullifies the benefit of using multiple $\w$'s for different token indices $t\in[T]$. Finally, \emph{weight matrix for the value keys} is implicitly subsumed within the linear prediction head $\ones_T\w^\top$ (without losing generality).
%Note  this corresponds to a primal-attention model with uniform attention weights $[\ab]_t=1/T, t\in[T]$.

\noindent\textbf{Linear-\attn model.} The linear-\attn model parameterized by $\thetab=(\w,\qb)$ replaces the softmax score transformation in \eqref{eq:PA}  with a linear function and outputs
\begin{align}\label{eq:linatt_model}
\flinatt(\w,\qb) = \w^\top\X^\top\X\qb/T.
\end{align}

\subsection{Training}
Given $\Sc=(\X_i,y_i)_{i=1}^n$ drawn i.i.d.~from $\Dc$, we solve square-loss empirical risk minimization to obtain $\thetah=(\wh,\qh)$ %(considered here for simplicity compared to say logistic or hinge loss) 
\begin{align}\label{eq:loss}
\thetah=\arg\min_{\thetab} \Lch_{\Sc}(\thetab):=\frac{1}{2n}\sum_{i=1}^n (y_i-f_{\thetab}(\X_i))^2.
\end{align}
Within our theoretical investigation, we are interested in the following performance criteria for models $f\in \{\fat,\flinatt,\fsat\}$:
%\begin{itemize}
%\item 
\noindent$\bullet$\textbf{Classification error}: For a model $f_{\thetah}$ this is defined as $\err(\thetah):=\Pro(y f_{\thetah}(\X)>0)$.
 \noindent$\bullet$~\textbf{Test risk:} $\Lc(\thetah)=\E_{(y,\X)\sim \Dc}[(y-f_{\thetah}(\X))^2]$,
%\item \textbf{Estimation quality:} $\corr{\qstar,\qh}, \corr{\wstar,\wh}$ where $\corr{\cdot,\cdot}$ returns the correlation coefficient.
%\end{itemize}
%Let us introduce the standard definition for 
%where we let $\thetab=(\qb,\w)$ denote the model parameters.

% We make the following assumption.
% \begin{assumption} \label{main assume}$\rho(\cdot)=\text{softmax}$ nonlinearity, $\qstar\perp\wstar$, and third moment of $\z\sim\subg{\sigma^2\Iden}$ is zero.
% \end{assumption}
% Softmax is the standard nonlinearity for attention mechanism. The orthogonality condition is useful for more tractable analysis as it helps decouple feature selection and prediction. Zero third moment is a mild condition e.g.~holds for symmetric distributions $\z\sim-\z$.


%\input{sec/baseline}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%
%%%\begin{align}
%%%\term{1} &= \frac{1}{nT}\sum_{i\in[n]}y_i\X_i^\top\X_i\w 
%%%\\
%%%&=\zeta\hat{Y}\corq \qb_\star  + \zeta\hat{Y}\corw \w_\star + \zeta\corq\w_\star + \zeta\corw\qb_\star + \frac{1}{nT}\sum_{i\in[n]}\Z_i^\top\Z_i\w, \nn
%%%\\
%%%&=\zeta(\hat{Y}\corq + \corw) \qb_\star  + \zeta(\hat{Y}\corw + \corq) \w_\star + \frac{1}{nT}\sum_{i\in[n]}\Z_i^\top\Z_i\w, \nn
%%%\end{align}
%%%
%%%
%%%\vp
%%%
%%%
%%%\begin{align*}
%%%\term{3}&=\frac{1}{nT^2}\sum_{i\in[n]}\big(\w^\top\X_i^\top\ones_T\big)\X_i^\top\X_i\w \\
%%%&= \frac{\zeta}{nT}\sum_{i\in[n]}\big(\w^\top\X_i^\top\ones_T\big)(\qb_\star+y_i\w_\star)(\qb_\star+y_i\w_\star)^\top\w 
%%%+ \frac{1}{nT}\sum_{i\in[n]}\big(\w^\top\X_i^\top\ones_T\big)\Z_i^\top\Z_i\w
%%%\\
%%%&= \frac{\zeta^2}{n}\sum_{i\in[n]}(\w^\top\qb_\star+y_i\w^\top\w_\star)^2(\qb_\star+y_i\w_\star) + 
%%%\frac{\zeta}{nT}\sum_{i\in[n]}(\w^\top\Z_i\ones)(\qb_\star^\top\w+y_i\w_\star^\top\w) (\qb_\star+y_i\w_\star)
%%%\\
%%%&\qquad+ \frac{\zeta}{nT}\sum_{i\in[n]}(\w^\top\qb_\star+y_i\w^\top\w_\star)\Z_i^\top\Z_i\w
%%%+ \frac{1}{nT^2}\sum_{i\in[n]}(\w^\top\Z_i\ones)\Z_i^\top\Z_i\w
%%%\\
%%%&= \frac{\zeta^2}{n}\sum_{i\in[n]}(\corq+y_i\corw)^2(\qb_\star+y_i\w_\star) + 
%%%\frac{\zeta}{nT}\sum_{i\in[n]}(\w^\top\Z_i\ones)(\corq+y_i\corw) (\qb_\star+y_i\w_\star)
%%%\\
%%%&\qquad+ \frac{\zeta}{nT}\sum_{i\in[n]}(\corq+y_i\corw)\Z_i^\top\Z_i\w
%%%+ \frac{1}{nT^2}\sum_{i\in[n]}(\w^\top\Z_i\ones)\Z_i^\top\Z_i\w
%%%\end{align*}
%%%
%%%\vp 
%%%\begin{align*}
%%%\term{2}&=\frac{1}{nT^2}\sum_{i\in[n]}y_i\X_i^\top\ones\ones^\top\X_i\w
%%%\\
%%%&=\frac{1}{nT^2}\sum_{i\in[n]}y_i\big(\zeta T (\qstar+y_i\wstar)+\Z_i^\top\ones\big)\big( \zeta T(\corq+y_i\corw)+\ones^\top\Z_i\w \big)
%%%\end{align*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\vspace{10pt}
%\begin{align}
%\sum_{\ell,k}\eb_\ell\eb_k^\top \E[ f(\X)_{\ell,k}\X] =
%\sum_{\ell,k}\eb_\ell\eb_k^\top \E[\partialf{f(\X)_{\ell,k}}{\X}]
%\end{align}



\subsection{Assumptions and notations}


% We make the following assumptions. 
 

 %e.g.~holds for symmetric distributions $\z\sim-\z$.

% \begin{assumption}\label{ass:noise}
% The noise vector $\z\sim\subg{\bSi}$ is centered, $K$-subgaussian with covariance $\Sigmab:=\E[\z\z^T]$. Moreover, its distribution is symmetric and zero-third moment, i.e. $\E\Big[\z\otimes \left(\z^T \z\right)\Big]=0$.
% %\ct{Decide: $\Sigmab=\sigma^2\Id$ or keep general and write everything in terms of $K$-subgaussian}
% \end{assumption}

% \let\origtheassumption\theassumption

% First, we assume that the size of the set of label-relevant tokens is constant among different data samples. This assumption is mild: it helps simplify the statements of the results and can be easily relaxed. Importantly, despite the assumption, our model \eqref{eq:CGMM} still allows for different subsets of label-relevant vs irrelevant tokens among different examples.
% \ct{We can as well subsume this to the model definition. may be cleaner}
% \begin{assumption}\label{ass:zeta constant}
%     For any example $(\X_i,y_i)\sim\Dc$ in \eqref{eq:CGMM} assume constant fraction of the set of label-relevant tokens $\zeta:=|\Rc_i|/T\in(0,1)$.
% \end{assumption}



 First, we formally state our assumptions on the noisy tokens. The more general condition is that noise is subgaussian and satisfies a mild zero third-moment condition.

\let\origtheassumption\theassumption
\edef\oldassumption{\the\numexpr\value{assumption}+1}
\setcounter{assumption}{0}
\renewcommand{\theassumption}{\oldassumption.\alph{assumption}}

\begin{assumption}\label{ass:noise}
The noise vector $\z\sim\subg{\sigma}$ is centered $\sigma$-subGaussian, i.e. $\tn{\z}_{\psi_2}=\sigma$. Moreover, its distribution is symmetric and zero-third moment, i.e. $\E\Big[\z\otimes \left(\z^\top \z\right)\Big]=0$. We denote the noise covariance  $\Sigmab:=\E[\z\z^\top].$
%\ct{Decide: $\Sigmab=\sigma^2\Id$ or keep general and write everything in terms of $K$-subgaussian}
\end{assumption}

For some of our results it will be convenient to further assume that noise is Gaussian since this allows leads to precise formulas that are easily interpretable.

\begin{assumption}\label{ass:noise Gaussian}
The noise vector $\z\sim\Nn(0,\sigma^2\Id)$ is isotropic Gaussian with variance $\sigma^2.$
\end{assumption}



 \let\theassumption\origtheassumption


\edef\oldassumption{\the\numexpr\value{assumption}+1}


\setcounter{assumption}{0}
\renewcommand{\theassumption}{\oldassumption.\alph{assumption}}



Second, a mild assumption on the correlation between the context $\qstar$ and classifier $\wstar$, which guarantees  pure signal tokens $\qstar+y\wstar$ are correctly classifier by the true regressor $\wstar,$ i.e. $y\wstar^\top\qstar+y\wstar>0$. For convenience, we denote
\[
\wnorm:=\tn{\wstar},~~~
\qnorm:=\tn{\qstar},~~~
\rho:=\frac{\qstar^\top\wstar}{\tn{\qstar}\tn{\wstar}}.
\]
\begin{assumption}\label{ass:rho general but small}
    Correlation  satisfies $\abs{\rho}<\frac{W}{Q}.$
\end{assumption}

We will also often
 consider the special case of zero correlation $\rho$ and thus state it as separate assumption below. This  orthogonality assumption, is useful for more tractable analysis as it helps decouple feature selection and prediction.
\begin{assumption}\label{ass:orthogonal}The context and classifier vectors are orthogonal, i.e. $\qstar\perp\wstar$.
\end{assumption}
% However, our analysis is general and covers non-zero correlation. For convenience, denote
% \begin{align}\label{eq:corrdef} 
% \rho:= \qstar^\top\wstar/\qnorm\wnorm.
%\end{align}


\paragraph{Notation.}
%Let $\qstarnorm=\qstar/\tn{\qstar}, \wstarnorm=\wstar/\tn{\wstar}.$ $\qnorm:=\tn{\qstar}, \wnorm:=\tn{\wstar}$
We use boldface letters for vectors and matrices. We use $\ones_m$ to denote an  $m$-dimensional vector of all ones.  For a vector $\vb$, $\tn{\vb}$ denotes its Euclidean norm and $\vb/\tn{\vb}$ its normalization. $\sft{\cdot}$ denotes the softmax transformation. $Q(\cdot)$ denotes the tail function of standard normal distribution. $\mini$ / $\maxi$ denotes the minimum / maximum of two numbers.  $\ordet{}$ and $\gtrsim$ notation suppress logarithmic dependencies. $\propto$ denotes proportionality.
%$\rho:= \qstar^\top\wstar/\qnorm\wnorm.$

% The noise covariance $\Sigmab:=\E[\z\z^\top]$

==> conclusion.tex <==
\section{Discussion}

In light of remarkable success of attention architectures, we initiate a theoretical investigation of the fundamentals of one one of its core mechanisms: prompt-tuning. For a one-layer attention model, we motivate and analyze a simplified model for prompt-tuning, which we coin prompt-attention. Although simple, prompt-attention and its analysis captures nontrivial interactions between the prompt vector and input features showing how it enables attending to context-relevant information while discarding nuisance parameters. It also shows the important role played in this process by the softmax transformation. Finally, the model allows for an interesting finding: prompt-attention can outperform fine-tuning. This theoretical finding is further supported  by and guides our experiments on real datasets. Looking ahead, there are several exciting options to extend our model and analysis. For example, we aim to relax the three simplifying assumption in Sec. \ref{sec:motivation}. Specifically, we believe that it is possible to extend our results to include the frozen self-attention part of the output $y_\text{pre}$ by introducing a deviations argument. An extension of the model to include  multiple prompt vectors perhaps in accordance with extending \eqref{eq:CGMM} to include multiple context vectors are interesting directions. We also want to investigate the role of multi-head attention in our setting. 

% \red{Discuss joint analysis of prompt-attention and self-attention}.

%  Secondly, our dataset model \eqref{eq:CGMM} will (essentially) be solvable by prompt-tuning alone and $y_\pre$ only depends on the pre-trained model and is isolated from the prompt-weights $\thetab$. Consequently, one can scale up the prompt-head $\W$ to dominate $y_\pre$ without impacting accuracy. 

==> experiments.tex <==
\section{Experiments}

First, we verify the utility of the \prml via experiments on a synthetic setting that precisely follows the contextual data model (cf.~Section~\ref{sec:data_model}). Subsequently, we explore prompt-tuning on various image-classification tasks that are motivated by the contextual data model and compare it with the standard fine-tuning method. Finally, we validate the utility of prompt vectors in distinguishing relevant tokens from irrelevant tokens via \prml under an image classification setting. %\todoasr{Add a statement about relevance/attn scores.}
Due to space constraints, we delegate our results on synthetic dataset to Appendix~\ref{append:synthetic-exp}.

% \subsection{Synthetic experiments}
% \label{append:synthetic-exp}
% \subsection{Synthetic experiments}
% \label{sec:exp-synthetic}
% Here, we generate a synthetic dataset according to the \textit{core dataset model}, i.e., we have $\delta = (\delta^q, \delta^w) = (0,0)$ for all examples in the dataset. In particular, we consider a setting with $T$ = 500, $d$=50, and $\zeta = 0.1$, i.e., each example has 500 tokens out of which 10\% tokens are relevant. As for the noisy tokens, they consists of i.i.d. $\mathcal{N}(0, \mathbf{I})$ vectors. Assuming that $\qstar \perp \wstar$ and $\sqrt{T}\wnorm = 3$, we generate $n = 10\cdot d$ training examples from the core dataset model for varying $\qnorm$. Fig.~\ref{fig:synthetic-results} showcases the performance of \prml (cf.~Section~\ref{sec:pmt-attn}) when combined with the estimates $\hat{\qb}$ and $\hat{\w}$ gradient-based algorithm in Section~\ref{sec:gradient-algo}. We also showcase the performance of the linear model (cf.~\eqref{eq:linear_model}) and two oracle methods where we assume access to true $\qstar$ and true $(\qstar, \wstar)$ while applying the \prml, respectively.

% Note that \prml achieves a vanishing classification test error in this setting whereas a natural baseline (linear model) can fail to achieve a good performance. On the other hand, the \prml enable by the gradient-based algorithm successfully achieves a high accuracy as the context energy (defined by $\qnorm$) increases, validating the utility of \prml as well as our gradient-based algorithm.

% \begin{figure}[h!]
%         \centering
%         \includegraphics[scale=0.5]{figs/normQ_ITR_20_GRID_21_ALP_10_TD_10_ZETA_0.1_mean.pdf}
%     \caption{Performance of \prml on the synthetic setting described in Section~\ref{sec:exp-synthetic}. For \prml, we employ the gradient-based algorithm from Section~\ref{sec:gradient-algo} to obtain estimates $\hat{\qb}$ and $\hat{\w}$. For the baseline linear model and two oracle settings, we have closed-form expressions for their asymptotic test error (cf.~Theorem~\ref{separate thm}), which is depicted by solid lines. On the other hand, markers show the finite sample performance of these three methods. All finite sample performances are obtained by averaging over 20 independent runs.}
%     \label{fig:synthetic-results}
% \end{figure}

\begin{figure*}[t!]
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[scale=0.17]{figs/ftiled_combined_image_3.pdf}
        \caption{{\footnotesize\ftiled}}
        \label{fig:ftiled-ex}
    \end{subfigure}%
    \quad
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[scale=0.17]{figs/ptiled_combined_image_3v2.pdf}
        \caption{{\footnotesize\ptiled}}
        \label{fig:ptiled-ex}
    \end{subfigure}%
    \quad
    \begin{subfigure}{0.35\textwidth}
        \centering
        \includegraphics[scale=0.17]{figs/embd_combined_image_3.pdf}
        \caption{{\footnotesize\embd}}
        \label{fig:embd-ex}
    \end{subfigure}
    \caption{Illustration of different CIFAR-10 based datasets utilized in image classification experiments (cf.~Section~\ref{sec:exp-image}). Note that all three variants correspond to 10-way multiclass classification tasks corresponding to 10 original classes in CIFAR-10.}
    \label{fig:dataset-examples}
\end{figure*}


\begin{figure*}[t!]
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.37]{figs/embed_imagenet_5k_.pdf}
        \caption{Full dataset}
        \label{fig:embd-res-cap100}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.37]{figs/embed_imagenet_500_.pdf}
        \caption{Capped 10\%}
        \label{fig:embd-res-cap10}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.37]{figs/embed_imagenet_100_.pdf}
        \caption{Capped 2\%}
        \label{fig:embd-res-cap2}
    \end{subfigure}
    \caption{Performance of fine-tuning vs. prompt-tuning on 10-way classification tasks defined by \embd dataset. Full dataset has 50K training examples. Capped 10\% and 2\% correspond to sub-sampled \textit{train} sets where we select exactly 500 and 100 examples per class from the full dataset. Note that number of prompt vectors equal to 0 corresponds to \textit{zero-shot} performance.}
    \label{fig:embd-results}
\end{figure*}

% \begin{figure*}[t!]
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_5k_.pdf}
%         \caption{Full dataset}
%         \label{fig:ptiled-res-cap100}
%     \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_500_.pdf}
%         \caption{Capped 10\%}
%         \label{fig:ptiled-res-cap10}
%     \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_100_.pdf}
%         \caption{Capped 2\%}
%         \label{fig:ptiled-res-cap2}
%     \end{subfigure}
%     \caption{Performance of fine-tuning vs. prompt-tuning on 10-way classification tasks defined by \ptiled dataset. Full dataset has 50K training examples. Capped 10\% and 2\% correspond to sub-sampled \textit{train} sets where we select exactly 500 and 100 examples per class from the full dataset. Note that number of prompt vectors equal to 0 corresponds to \textit{zero-shot} performance.}
%     \label{fig:ptiled-results}
% \end{figure*}

\subsection{Image classification experiments}
\label{sec:exp-image}

% \subsubsection{Experimental setup}
% \label{sec:setup-image}

\textbf{Dataset.} Motivated by our contextual data model (cf.~Section~\ref{sec:data_model}), we construct multiple datasets based on the CIFAR-10 dataset~\citep{krizhevsky2009learning} to conduct our evaluation. We construct three such datasets (see Fig.~\ref{fig:dataset-examples} for examples). Due to spaces constraints, we defer the additional details regarding datasets to Appendix~\ref{append:image-experiments}. We also refer the reader to Appendix~\ref{append:image-experiments} for details regarding the model architecture and training procedure.

% \begin{itemize}
% \item {\ftiled.}~For this dataset, each examples consists of a 64x64 images obtained by arranging a 32x32 image from the original CIFAR-10 dataset a tiling pattern with four tiles (cf.~Fig.~\ref{fig:ftiled-ex}).
% \item {\ptiled.}~This is dataset is similar to \ftiled with the exception that each image has at-least $T$ out of 4 tiles replaced by a patch of i.i.d. random Gaussian noise with mean zero and variance 0.2. Note that $T \in \{1, 2, 3\}$ is a random number as well as the location of the noisy tiles for each image in the dataset (cf.~Fig.~\ref{fig:ptiled-ex}).  
% \item {\embd.}~In this dataset~\citep{karp2021neurips}, we construct an example by simply embedding a 32 x 32 image from CIFAR-10 at a random location in a 64 x 64 background corresponding to a randomly selected image from ImageNet~\cite{ILSVRC15}. We also add a i.i.d. random Gaussian noise with mean zero and variance 0.2 to the background (cf.~Fig.~\ref{fig:embd-ex}).
% \end{itemize}
% By construction, each dataset has 50,000 train and 10,000 test examples corresponding to train and test set of CIFAR-10. We also considered data-limited setting where we keep the test set intact but reduce the size of train set by sampling a fixed number of images for each class from the original train set. Note that all three datasets define 10-way multiclass classification tasks with CIFAR-10 classes as potential labels.

% \textbf{Model architecture.}~We utilize a tiny variant of the Vision transformer model~\cite{dosovitskiy2021vit} for all of our experiments in this subsection. This variant has 12 transformer layers with it hidden dimension, MLP intermediate dimension, and number of heads per attention layer being equal to 192, 768, and 3, respectively. The patch size in our study is set to be 4x4. The model itself (without counting the trainable parameters/weights during prompt-tuning) has approximately 5.44M parameters. We rely on the CLS token to obtain the classification logits.

% \textbf{Training.}~We rely on Scenic library~\citep{dehghani2021scenic}\footnote{\url{https://github.com/google-research/scenic}} to conduct our experiments on image classification. Following the default settings in the library along with a coarse grid search, we employ Adam optimizer~\citep{kingma2014adam} with $\beta_1$ = 0.9,  $\beta_2$ = 0.999, weight decay = 0.1, and batch size = 128 while training a \textit{randomly initialized} model. Furthermore, we employ a linear warm-up of learning rate followed cosine learning rate schedule with base learning rate 3e-3. As for the fine-tuning and prompt-tuning experiments that (partially) initialize from a \textit{pre-trained} model, we rely on SGD with momentum parameter 0.9 and batch size = 128 to update trainable parameters. Again, we utilize a linear warm-up of learning rate followed cosine learning rate schedule. Throughout our experiments, the base learning rates for fine-tuning and prompt-tuning are 1e-3 and 0.1, respectively.

\textbf{Methods.}~In our fine-tuning experiments, we update all pre-trained model parameters. %of a pre-trained model. 
As for prompt-tuning, we only update newly introduced (prompt) variables and keep the pre-trained network frozen. We consider three variants of prompt-tuning: 1) \promptt~\citep{lester2021power}, where we add trainable vector between CLS token embedding and first image (patch) embeddings only at the input; 2) \prefixt~\citep{li2021prefix}, where we add the \textit{same} trainable vectors between the CLS embedding and the first image embedding at the input of every transformer layer; and 3) \prefixtfull, where we add \textit{different} trainable vectors between the CLS embedding and the first image patch embedding at the input of every transformer layer. Note that the number of trainable parameters in \promptt and \prefixt do not scale with the number of layers whereas we have linear scaling with number of layers in % the trainable parameters in 
\prefixtfull. %linearly scales with the number of transformer layers in the model. 
Interestingly, all three prompt-tuning variant are identical when the number of layers is 1, which corresponds to the setup we theoretically analyzed in the paper. However, they exhibit remarkably different behavior for a multi-layer transformer model, as we show in the next subsection. 

% \subsubsection{Results}
\noindent{\textbf{Results.}}~Here, the main goal of our exploration is to highlight the different behavior of fine-tuning and prompt-tuning. Towards this, we utilize a model trained on \ftiled dataset as the pre-trained model. This model achieves top-1 (in-domain) accuracy of 80.43 on \ftiled test set. In contrast, it achieves \textit{zero-shot} top-1 accuracy of 56.35 and 17.97 on \ptiled and \embd, respectively. This alludes to the fact that \embd corresponds to a larger distribution shift from the pre-training distribution (\ftiled), as compared to \ptiled.

Fig.~\ref{fig:embd-results} and Fig.~\ref{fig:ptiled-results} (cf.~Appendix~\ref{append:additional-image-results}) showcase the performance of fine-tuning and prompt-tuning approaches on \embd and \ptiled, respectively.  %It is evident from the figures
Note that fine-tuning outperforms prompt-tuning in a data-rich setting (cf.~Fig.~\ref{fig:embd-res-cap100} and \ref{fig:ptiled-res-cap100}). This is due to fine-tuning having the ability to update a large number of model parameters (5.4M in our case). In contrast, with $2000$ prompt vectors, \prefixtfull (the most expensive prompt-tuning method out of all three) only updates 460.8K parameters.

Interestingly, in the data-limited regimes, prompt-tuning becomes more competitive with fine-tuning. In fact, the best performing prompt-tuning method outperforms the fine-tuning (cf.~Fig.~\ref{fig:embd-res-cap10} and \ref{fig:embd-res-cap2}) on \embd, where fine-tuning can easily overfit as it cannot leverage the benefits of the pre-training data due to a large distribution-shift between \ftiled and \embd. 

As for the varying performance among different prompt-tuning approaches, part of the performance gap between \prefixtfull and \prefixt can be attributed to the larger number of trainable parameters available to \prefixtfull. Even more interestingly, \prefixt consistently outperforms \promptt, even with the same number of trainable parameters. This alludes to the fact that optimization and architecture choices play a major role beyond just the number of trainable parameters. As mentioned earlier, our theoretical treatment for a single-layer model cannot distinguish among these different prompt-tuning approaches. As a result, we believe that our empirical observations point to multiple interesting avenues for future work.

\subsection{Attention weights for prompt vectors}
\label{sec:relevance-prompt-vecs}

Finally, we explore what role \prml, i.e., the attention weights with prompt vectors as keys and image patches/tokens as values, plays towards underlying task. In Fig.~\ref{fig:image_and_attn_maps}~(cf.~Appendix~\ref{append:additional-image-results}), we illustrate one representative example. The figures shows how average attention weights from prompt vectors to image tokens/patches evolve across transformer layers, when we employ \prefixtfull. Indeed, the figure verifies that \prml helps locate the relevant tokens/patches from the irrelevant patches, validating our starting hypothesis in Section~\ref{sec:motivation} and \ref{sec:data_model}.

%Although simple, prompt-attention and its analysis captures nontrivial interactions between the prompt vector and input features showing how it enables attending to context-relevant information while discarding nuisance parameters. 
\vspace{-6pt}
\section*{Discussion}\vspace{-3pt}
In light of remarkable success of attention architectures, we initiate a theoretical investigation of one of its core mechanisms: prompt-tuning. For a one-layer attention model, we motivate and analyze a simplified model for prompt-tuning, which we coin prompt-attention. Through our model, we developed new statistical foundations for gradient-based prompt-tuning, characterized its optimization and generalization dynamics and how it facilitates attending to context-relevant information. We also showed that under \eqref{eq:CGMM} model one-layer softmax-prompt-tuning can provably be superior to alternatives including one layer self-attention. Thorough experiments support our theory on how prompt-tuning attends to the context and how it can potentially outperform full fine-tuning. Our results also suggest many interesting future directions including (1) extension to deeper architectures by characterizing the role of softmax-attention in individual layers, (2) developing a stronger theoretical and empirical understanding of when/if promp-tuning is superior to fine-tuning, (3) extending our model to include multiple prompt vectors (and perhaps extending \eqref{eq:CGMM} to include multiple context vectors), and (4) investigating the role of multiple attention heads in prompt-tuning.

%(3) we believe that it is possible to extend our results to include the frozen self-attention part of the output $y_\text{pre}$ by introducing a perturbation argument. An extension of the model

%Specifically, we believe that it is possible to extend our results to include the frozen self-attention part of the output $y_\text{pre}$ by introducing a deviations argument. An extension of the model to include  multiple prompt vectors perhaps in accordance with extending \eqref{eq:CGMM} to include multiple context vectors are interesting directions. We also want to investigate the role of multi-head attention in our setting.

% \todo{Put the figure in the right section in the appendix, when everything else is finalized.}

% \begin{figure*}
%   \vspace{-2mm}
%   \hspace{15mm}
%     \begin{subfigure}[b]{0.25\linewidth}
%       \centering
%       \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0},clip]{attn_imgs/embed_imagenet_image_16.pdf}
%       \caption{Input image}
%       \label{fig:image1}
%     \end{subfigure}
%   \hfill
%   \begin{minipage}[b]{.7\linewidth}
%   \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_0.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_3.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_7.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_11.pdf}
%     \caption{Average attention weights from prompts (keys) to image patches (values).}
%     \label{fig:attn_maps1}
%   \end{subfigure}
%   \end{minipage}%
%   \caption{Illustration of how attention weights progressive change from first layer (Fig.~\ref{fig:attn_maps1}-top) to last layer (Fig.~\ref{fig:attn_maps1}-bottom) in the transformer model for a given input image (Fig.~\ref{fig:image1}) when we employ \prefixtfull. We plot average attention weights from 50 prompt vectors (keys) to 256 image patches (values). The attention weights for each attention head are naturally arranged in a 16 x 16 grid corresponding to original locations of the patches in the image. Note that the attention weights in the early layer have the tiling pattern similar to that in \ftiled -- the dataset utilized by the pre-trained model. However, as we progress deeper in the transformer, attention weights begin to capture the relevant patch locations in the dataset of interest, i.e., \embd.}
%   \label{fig:image_and_attn_maps}
% \end{figure*}

==> experiments_camera_ready.tex <==
\section{Experiments}

First, we verify the utility of \prml via experiments on a synthetic setting that precisely follows the contextual data model from Section~\ref{sec:data_model}. Subsequently, we explore prompt-tuning on various image classification tasks that are motivated by the contextual data model and compare it with the standard fine-tuning method. Finally, we validate the utility of prompt vectors in distinguishing relevant tokens from irrelevant tokens via \prml under an image classification setting. 
% Due to space constraints, we delegate our results on synthetic dataset to Appendix~\ref{append:synthetic-exp}.

\subsection{Synthetic experiments}
\label{sec:exp-synthetic}
Here, we generate a synthetic dataset according to the \textit{core dataset model}, i.e. we have $\delta = (\delta^q, \delta^w) = (0,0)$ for all examples in the dataset. In particular, we consider a setting with $T = 500$, $d = 50$, and $\zeta = 0.1$, i.e. each example has 500 tokens out of which 10\% tokens are relevant. As for the noisy tokens, they consists of i.i.d. $\mathcal{N}(0, \mathbf{I})$ vectors. Assuming that $\qstar \perp \wstar$ and $\sqrt{T}\wnorm = 3$, we generate $n = 10\cdot d$ training examples from the core dataset model for varying $\qnorm$. Fig.~\ref{fig:synthetic-results} showcases the performance of \prml (cf.~\eqref{eq:PA}) when combined with the estimates $\hat{\qb}$ and $\hat{\w}$ produced by gradient-based algorithm in \eqref{eq:algo}. We also showcase the performance of the linear model (cf.~\eqref{eq:linear_model}) and two oracle methods where we assume access to true $\qstar$ and true $(\qstar, \wstar)$, respectively, while applying the \prml. Note that \prml achieves a vanishing classification test error in this setting whereas a natural baseline (linear model) can fail to achieve a good performance. On the other hand, the \prml enabled by \eqref{eq:algo} successfully achieves a high accuracy as the context energy (defined by $\qnorm$) increases, validating the utility of \prml as well as our gradient-based algorithm in \eqref{eq:algo}.
{Finally, we also consider a stochastic $\delta = (\delta^q, \delta^w) \neq (0, 0)$ to validate Theorem~\ref{separate thm} as described in Fig.~\ref{fig:thm1-verification}.}

\begin{figure}[t!]
        \centering
        \includegraphics[scale=0.4]{figs/normQ_ITR_20_GRID_21_ALP_10_TD_10_ZETA_0.1_mean.pdf}
        \vspace{-2mm}
    \caption{Performance of \prml on the synthetic setting described in Section~\ref{sec:exp-synthetic}. For \prml, we employ the algorithm in \eqref{eq:algo} to obtain $\hat{\qb}$ and $\hat{\w}$. For the baseline linear model and two oracle settings, we have closed-form expressions for their asymptotic test error (cf.~Theorem~\ref{separate thm}), which are depicted by solid lines. On the other hand, markers show the finite sample performance of these three methods. All finite sample performances are obtained by averaging over 20 independent runs.}
    \label{fig:synthetic-results}
    \vspace{-4mm}
\end{figure}

% First, we verify the utility of the \prml via experiments on a synthetic setting that precisely follows the contextual data model (cf.~Section~\ref{sec:data_model}). Subsequently, we explore prompt-tuning on various image-classification tasks that are motivated by the contextual data model and compare it with the standard fine-tuning method. Finally, we validate the utility of prompt vectors in distinguishing relevant tokens from irrelevant tokens via \prml under an image classification setting. %\todoasr{Add a statement about relevance/attn scores.}
% Due to space constraints, we delegate our results on synthetic dataset to Appendix~\ref{append:synthetic-exp}.

% \subsection{Synthetic experiments}
% \label{append:synthetic-exp}
% \subsection{Synthetic experiments}
% \label{sec:exp-synthetic}
% Here, we generate a synthetic dataset according to the \textit{core dataset model}, i.e., we have $\delta = (\delta^q, \delta^w) = (0,0)$ for all examples in the dataset. In particular, we consider a setting with $T$ = 500, $d$=50, and $\zeta = 0.1$, i.e., each example has 500 tokens out of which 10\% tokens are relevant. As for the noisy tokens, they consists of i.i.d. $\mathcal{N}(0, \mathbf{I})$ vectors. Assuming that $\qstar \perp \wstar$ and $\sqrt{T}\wnorm = 3$, we generate $n = 10\cdot d$ training examples from the core dataset model for varying $\qnorm$. Fig.~\ref{fig:synthetic-results} showcases the performance of \prml (cf.~Section~\ref{sec:pmt-attn}) when combined with the estimates $\hat{\qb}$ and $\hat{\w}$ gradient-based algorithm in Section~\ref{sec:gradient-algo}. We also showcase the performance of the linear model (cf.~\eqref{eq:linear_model}) and two oracle methods where we assume access to true $\qstar$ and true $(\qstar, \wstar)$ while applying the \prml, respectively.

% Note that \prml achieves a vanishing classification test error in this setting whereas a natural baseline (linear model) can fail to achieve a good performance. On the other hand, the \prml enable by the gradient-based algorithm successfully achieves a high accuracy as the context energy (defined by $\qnorm$) increases, validating the utility of \prml as well as our gradient-based algorithm.

% \begin{figure}[h!]
%         \centering
%         \includegraphics[scale=0.5]{figs/normQ_ITR_20_GRID_21_ALP_10_TD_10_ZETA_0.1_mean.pdf}
%     \caption{Performance of \prml on the synthetic setting described in Section~\ref{sec:exp-synthetic}. For \prml, we employ the gradient-based algorithm from Section~\ref{sec:gradient-algo} to obtain estimates $\hat{\qb}$ and $\hat{\w}$. For the baseline linear model and two oracle settings, we have closed-form expressions for their asymptotic test error (cf.~Theorem~\ref{separate thm}), which is depicted by solid lines. On the other hand, markers show the finite sample performance of these three methods. All finite sample performances are obtained by averaging over 20 independent runs.}
%     \label{fig:synthetic-results}
% \end{figure}

% \begin{figure*}[t!]
%     \begin{subfigure}{0.32\textwidth}
%         \centering
%         \includegraphics[scale=0.17]{figs/ftiled_combined_image_3.pdf}
%         \caption{{\footnotesize\ftiled}}
%         \label{fig:ftiled-ex}
%     \end{subfigure}%
%     \quad
%     \begin{subfigure}{0.32\textwidth}
%         \centering
%         \includegraphics[scale=0.17]{figs/ptiled_combined_image_3v2.pdf}
%         \caption{{\footnotesize\ptiled}}
%         \label{fig:ptiled-ex}
%     \end{subfigure}%
%     \quad
%     \begin{subfigure}{0.35\textwidth}
%         \centering
%         \includegraphics[scale=0.17]{figs/embd_combined_image_3.pdf}
%         \caption{{\footnotesize\embd}}
%         \label{fig:embd-ex}
%     \end{subfigure}
%     \caption{Illustration of different CIFAR-10 based datasets utilized in image classification experiments (cf.~Section~\ref{sec:exp-image}). Note that all three variants correspond to 10-way multiclass classification tasks corresponding to 10 original classes in CIFAR-10.}
%     \label{fig:dataset-examples}
% \end{figure*}

\begin{figure*}[t!]
    \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[scale=0.15]{figs/ftiled_combined_image_3.pdf}
        \caption{{\footnotesize\ftiled}}
        \label{fig:ftiled-ex}
    \end{subfigure}%
    \quad
    \begin{subfigure}{0.31\textwidth}
        \centering
        \includegraphics[scale=0.15]{figs/ptiled_combined_image_3v2.pdf}
        \caption{{\footnotesize\ptiled}}
        \label{fig:ptiled-ex}
    \end{subfigure}%
    \quad
    \begin{subfigure}{0.36\textwidth}
        \centering
        \includegraphics[scale=0.15]{figs/embd_combined_image_3.pdf}
        \caption{{\footnotesize\embd}}
        \label{fig:embd-ex}
    \end{subfigure}
    \caption{Illustration of different CIFAR-10 based datasets utilized in image classification experiments (cf.~Section~\ref{sec:exp-image}). Note that all three variants correspond to 10-way multiclass classification tasks corresponding to 10 original classes in CIFAR-10.}
    \label{fig:dataset-examples}
\end{figure*}


\begin{figure*}[t!]
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.35]{figs/embed_imagenet_5k_.pdf}
        \caption{Full dataset}
        \label{fig:embd-res-cap100}
    \end{subfigure}~%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.35]{figs/embed_imagenet_500_.pdf}
        \caption{Capped 10\%}
        \label{fig:embd-res-cap10}
    \end{subfigure}~%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[scale=0.35]{figs/embed_imagenet_100_.pdf}
        \caption{Capped 2\%}
        \label{fig:embd-res-cap2}
    \end{subfigure}
    \caption{Performance of fine-tuning vs. prompt-tuning on 10-way classification tasks defined by \embd dataset. Full dataset has 50K training examples. Capped 10\% and 2\% correspond to sub-sampled \textit{train} sets where we select exactly 500 and 100 examples per class from the full dataset. Note that number of prompt vectors equal to 0 corresponds to \textit{zero-shot} performance.}
    \label{fig:embd-results}
\end{figure*}

% \begin{figure*}[t!]
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_5k_.pdf}
%         \caption{Full dataset}
%         \label{fig:ptiled-res-cap100}
%     \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_500_.pdf}
%         \caption{Capped 10\%}
%         \label{fig:ptiled-res-cap10}
%     \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/ptiled_100_.pdf}
%         \caption{Capped 2\%}
%         \label{fig:ptiled-res-cap2}
%     \end{subfigure}
%     \caption{Performance of fine-tuning vs. prompt-tuning on 10-way classification tasks defined by \ptiled dataset. Full dataset has 50K training examples. Capped 10\% and 2\% correspond to sub-sampled \textit{train} sets where we select exactly 500 and 100 examples per class from the full dataset. Note that number of prompt vectors equal to 0 corresponds to \textit{zero-shot} performance.}
%     \label{fig:ptiled-results}
% \end{figure*}

\subsection{Image classification experiments}
\label{sec:exp-image}

% \subsubsection{Experimental setup}
% \label{sec:setup-image}

\textbf{Dataset.} Motivated by our contextual data model, we construct three datasets based on CIFAR-10~\citep{krizhevsky2009learning} to conduct our evaluation %. We construct three such datasets 
(see Fig.~\ref{fig:dataset-examples} for examples). Due to spaces constraints, we defer the additional details regarding datasets to Appendix~\ref{append:image-experiments}. We also refer the reader to Appendix~\ref{append:image-experiments} for details regarding the model architecture and training procedure.

% \begin{itemize}
% \item {\ftiled.}~For this dataset, each examples consists of a 64x64 images obtained by arranging a 32x32 image from the original CIFAR-10 dataset a tiling pattern with four tiles (cf.~Fig.~\ref{fig:ftiled-ex}).
% \item {\ptiled.}~This is dataset is similar to \ftiled with the exception that each image has at-least $T$ out of 4 tiles replaced by a patch of i.i.d. random Gaussian noise with mean zero and variance 0.2. Note that $T \in \{1, 2, 3\}$ is a random number as well as the location of the noisy tiles for each image in the dataset (cf.~Fig.~\ref{fig:ptiled-ex}).  
% \item {\embd.}~In this dataset~\citep{karp2021neurips}, we construct an example by simply embedding a 32 x 32 image from CIFAR-10 at a random location in a 64 x 64 background corresponding to a randomly selected image from ImageNet~\cite{ILSVRC15}. We also add a i.i.d. random Gaussian noise with mean zero and variance 0.2 to the background (cf.~Fig.~\ref{fig:embd-ex}).
% \end{itemize}
% By construction, each dataset has 50,000 train and 10,000 test examples corresponding to train and test set of CIFAR-10. We also considered data-limited setting where we keep the test set intact but reduce the size of train set by sampling a fixed number of images for each class from the original train set. Note that all three datasets define 10-way multiclass classification tasks with CIFAR-10 classes as potential labels.

% \textbf{Model architecture.}~We utilize a tiny variant of the Vision transformer model~\cite{dosovitskiy2021vit} for all of our experiments in this subsection. This variant has 12 transformer layers with it hidden dimension, MLP intermediate dimension, and number of heads per attention layer being equal to 192, 768, and 3, respectively. The patch size in our study is set to be 4x4. The model itself (without counting the trainable parameters/weights during prompt-tuning) has approximately 5.44M parameters. We rely on the CLS token to obtain the classification logits.

% \textbf{Training.}~We rely on Scenic library~\citep{dehghani2021scenic}\footnote{\url{https://github.com/google-research/scenic}} to conduct our experiments on image classification. Following the default settings in the library along with a coarse grid search, we employ Adam optimizer~\citep{kingma2014adam} with $\beta_1$ = 0.9,  $\beta_2$ = 0.999, weight decay = 0.1, and batch size = 128 while training a \textit{randomly initialized} model. Furthermore, we employ a linear warm-up of learning rate followed cosine learning rate schedule with base learning rate 3e-3. As for the fine-tuning and prompt-tuning experiments that (partially) initialize from a \textit{pre-trained} model, we rely on SGD with momentum parameter 0.9 and batch size = 128 to update trainable parameters. Again, we utilize a linear warm-up of learning rate followed cosine learning rate schedule. Throughout our experiments, the base learning rates for fine-tuning and prompt-tuning are 1e-3 and 0.1, respectively.

\noindent\textbf{Methods.}~In our fine-tuning experiments, we update all pre-trained model parameters. %of a pre-trained model. 
As for prompt-tuning, we only update newly introduced (prompt) variables and keep the pre-trained network frozen. We consider three variants of prompt-tuning: 1) \promptt~\citep{lester2021power}, where we add trainable vector between CLS token embedding and first image (patch) embeddings only at the input; 2) \prefixt~\citep{li2021prefix}, where we add the \textit{same} trainable vectors between the CLS embedding and the first image embedding at the input of every transformer layer; and 3) \prefixtfull, where we add \textit{different} trainable vectors between the CLS embedding and the first image patch embedding at the input of every transformer layer. Note that the number of trainable parameters in \promptt and \prefixt do not scale with the number of layers whereas we have linear scaling with number of layers in % the trainable parameters in 
\prefixtfull. %linearly scales with the number of transformer layers in the model. 
Interestingly, all three prompt-tuning variant are identical when the number of layers is 1, which corresponds to the setup we theoretically analyzed in the paper. However, they exhibit remarkably different behavior for a multi-layer transformer model, as we show next. (In Appendix~\ref{append:additional-image-results}, we also compare prompt-tuning with fine-tuning only first layer self-attention parameters for the underlying ViT model as per the single-layer nature of our theoretical results.)

% \textbf{Methods.}~In our fine-tuning experiments, we update all pre-trained model parameters. %of a pre-trained model. 
% As for prompt-tuning, we only update newly introduced (prompt) variables and keep the pre-trained network frozen. We consider three variants of prompt-tuning: 1) \promptt~\citep{lester2021power}, where we add trainable vector between CLS token embedding and first image (patch) embeddings only at the input; 2) \prefixt~\citep{li2021prefix}, where we add the \textit{same} trainable vectors between the CLS embedding and the first image embedding at the input of every transformer layer; and 3) \prefixtfull, where we add \textit{different} trainable vectors between the CLS embedding and the first image patch embedding at the input of every transformer layer. Note that the number of trainable parameters in \promptt and \prefixt do not scale with the number of layers whereas we have linear scaling with number of layers in % the trainable parameters in 
% \prefixtfull. %linearly scales with the number of transformer layers in the model. 
% Interestingly, all three prompt-tuning variant are identical when the number of layers is 1, which corresponds to the setup we theoretically analyzed in the paper. However, they exhibit remarkably different behavior for a multi-layer transformer model, as we show in the next subsection. 

% \subsubsection{Results}
\noindent{\textbf{Results.}}~Here, the main goal of our exploration is to highlight the different behavior of fine-tuning and prompt-tuning. We utilize a model trained on \ftiled dataset as the pre-trained model. This model achieves top-1 (in-domain) accuracy of 80.43 on \ftiled test set. In contrast, it achieves \textit{zero-shot} top-1 test accuracy of 56.35 and 17.97 on \ptiled and \embd, respectively. This alludes to the fact that \embd corresponds to a larger distribution shift from the pre-training distribution (\ftiled), as compared to \ptiled.

% \noindent{\textbf{Results.}}~Here, the main goal of our exploration is to highlight the different behavior of fine-tuning and prompt-tuning. Towards this, we utilize a model trained on \ftiled dataset as the pre-trained model. This model achieves top-1 (in-domain) accuracy of 80.43 on \ftiled test set. In contrast, it achieves \textit{zero-shot} top-1 accuracy of 56.35 and 17.97 on \ptiled and \embd, respectively. This alludes to the fact that \embd corresponds to a larger distribution shift from the pre-training distribution (\ftiled), as compared to \ptiled.

Fig.~\ref{fig:embd-results} and Fig.~\ref{fig:ptiled-results} (cf.~Appendix~\ref{append:additional-image-results}) 
showcase the performance of fine-tuning and prompt-tuning approaches on \embd and \ptiled, respectively.  %It is evident from the figures
Note that fine-tuning outperforms prompt-tuning in a data-rich setting (cf.~Fig.~\ref{fig:embd-res-cap100} and \ref{fig:ptiled-res-cap100}). This is due to fine-tuning having the ability to update a large number of model parameters (5.4M in our case). In contrast, with $2000$ prompt vectors, \prefixtfull (the most expensive prompt-tuning method out of all three) only updates 460.8K parameters.

% Fig.~\ref{fig:embd-results} and Fig.~\ref{fig:ptiled-results} (cf.~Appendix~\ref{append:additional-image-results}) showcase the performance of fine-tuning and prompt-tuning approaches on \embd and \ptiled, respectively.  %It is evident from the figures
% Note that fine-tuning outperforms prompt-tuning in a data-rich setting (cf.~Fig.~\ref{fig:embd-res-cap100} and \ref{fig:ptiled-res-cap100}). This is due to fine-tuning having the ability to update a large number of model parameters (5.4M in our case). In contrast, with $2000$ prompt vectors, \prefixtfull (the most expensive prompt-tuning method out of all three) only updates 460.8K parameters.

Interestingly, in the data-limited regimes, prompt-tuning becomes more competitive.~% with fine-tuning. 
In fact, the best performing prompt-tuning method outperforms the fine-tuning (cf.~Fig.~\ref{fig:embd-res-cap10} and \ref{fig:embd-res-cap2}) on \embd, where fine-tuning can easily overfit as it cannot leverage the benefits of the pre-training data due to a large distribution-shift between \ftiled and \embd. 

%As for the varying performance among different prompt-tuning approaches, part 
Part of the performance gap between \prefixtfull and \prefixt can be attributed to the larger number of trainable parameters available to \prefixtfull. % Even more interestingly, 
Note that \prefixt consistently outperforms \promptt, even with the same number of trainable parameters. This alludes to the fact that optimization and architecture choices play a major role beyond just the number of trainable parameters. As mentioned earlier, our theoretical treatment for a single-layer model cannot distinguish among these different prompt-tuning approaches. As a result, we believe that our empirical observations point to multiple interesting avenues for future work.

% Interestingly, in the data-limited regimes, prompt-tuning becomes more competitive with fine-tuning. In fact, the best performing prompt-tuning method outperforms the fine-tuning (cf.~Fig.~\ref{fig:embd-res-cap10} and \ref{fig:embd-res-cap2}) on \embd, where fine-tuning can easily overfit as it cannot leverage the benefits of the pre-training data due to a large distribution-shift between \ftiled and \embd. 

% As for the varying performance among different prompt-tuning approaches, part of the performance gap between \prefixtfull and \prefixt can be attributed to the larger number of trainable parameters available to \prefixtfull. Even more interestingly, \prefixt consistently outperforms \promptt, even with the same number of trainable parameters. This alludes to the fact that optimization and architecture choices play a major role beyond just the number of trainable parameters. As mentioned earlier, our theoretical treatment for a single-layer model cannot distinguish among these different prompt-tuning approaches. As a result, we believe that our empirical observations point to multiple interesting avenues for future work.

\vspace{-6pt}
\subsection{Attention weights for prompt vectors}
\label{sec:relevance-prompt-vecs}

Finally, we explore what role \prml, i.e. the attention weights with prompt vectors as keys and image patches/tokens as values, plays towards underlying task. In Fig.~\ref{fig:image_and_attn_maps}~(cf.~Appendix~\ref{append:additional-image-results}), we illustrate one representative example. The figure shows how average attention weights from prompt vectors to image tokens/patches evolve across transformer layers, when we employ \prefixtfull. Indeed, the figure verifies that \prml helps distinguish the relevant tokens/patches from the irrelevant patches, validating our starting hypothesis in Section~\ref{sec:motivation} and \ref{sec:data_model}.

%Although simple, prompt-attention and its analysis captures nontrivial interactions between the prompt vector and input features showing how it enables attending to context-relevant information while discarding nuisance parameters. 
\vspace{-6pt}
\section{Discussion}\vspace{-3pt}
In light of remarkable success of attention architectures, we initiate a theoretical investigation of one of its core mechanisms: prompt-tuning. For a one-layer attention model, we motivate and analyze a simplified model for prompt-tuning, which we coin \prml. Through this model, we developed new statistical foundations for gradient-based prompt-tuning, characterized its optimization and generalization dynamics, and explored how it facilitates attending to context-relevant information. We also showed that under \eqref{eq:CGMM} one-layer softmax-prompt-tuning can provably be superior to alternatives including one layer self-attention. Thorough experiments support our theory on how prompt-tuning attends to the context and how it can potentially outperform full fine-tuning. Our results also suggest many interesting future directions including 1) extension to deeper architectures by characterizing the role of softmax-attention in individual layers, 2) developing a stronger theoretical and empirical understanding of when/if prompt-tuning is superior to fine-tuning, 3) extending our model to include multiple prompt vectors (and perhaps extending \eqref{eq:CGMM} to include multiple context vectors), and 4) investigating the role of multi-head attention in prompt-tuning.

%(3) we believe that it is possible to extend our results to include the frozen self-attention part of the output $y_\text{pre}$ by introducing a perturbation argument. An extension of the model

%Specifically, we believe that it is possible to extend our results to include the frozen self-attention part of the output $y_\text{pre}$ by introducing a deviations argument. An extension of the model to include  multiple prompt vectors perhaps in accordance with extending \eqref{eq:CGMM} to include multiple context vectors are interesting directions. We also want to investigate the role of multi-head attention in our setting.

% \todo{Put the figure in the right section in the appendix, when everything else is finalized.}

% \begin{figure*}
%   \vspace{-2mm}
%   \hspace{15mm}
%     \begin{subfigure}[b]{0.25\linewidth}
%       \centering
%       \includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0},clip]{attn_imgs/embed_imagenet_image_16.pdf}
%       \caption{Input image}
%       \label{fig:image1}
%     \end{subfigure}
%   \hfill
%   \begin{minipage}[b]{.7\linewidth}
%   \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_0.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_3.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_7.pdf}
%     % \caption{xyz}
%     % \label{fig:attn_maps}
%   \end{subfigure}
%     \begin{subfigure}[b]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{attn_imgs/embed_imagenet_image_16_layer_11.pdf}
%     \caption{Average attention weights from prompts (keys) to image patches (values).}
%     \label{fig:attn_maps1}
%   \end{subfigure}
%   \end{minipage}%
%   \caption{Illustration of how attention weights progressive change from first layer (Fig.~\ref{fig:attn_maps1}-top) to last layer (Fig.~\ref{fig:attn_maps1}-bottom) in the transformer model for a given input image (Fig.~\ref{fig:image1}) when we employ \prefixtfull. We plot average attention weights from 50 prompt vectors (keys) to 256 image patches (values). The attention weights for each attention head are naturally arranged in a 16 x 16 grid corresponding to original locations of the patches in the image. Note that the attention weights in the early layer have the tiling pattern similar to that in \ftiled -- the dataset utilized by the pre-trained model. However, as we progress deeper in the transformer, attention weights begin to capture the relevant patch locations in the dataset of interest, i.e., \embd.}
%   \label{fig:image_and_attn_maps}
% \end{figure*}

==> extensions_and_previous_discussions.tex <==
\section{Extensions}

\paragraph{Discriminative model}


\begin{equation}
\x_t  = \begin{cases}
\qstar^{\ell}+\z_t & \text{w.p.}~ \zeta~~~~~~~~\text{(a.k.a.~relevant token)}
\\
\z_t \sim \subg{\sigma^2\Iden} & \text{w.p.}~ 1-\zeta~~~~\text{(a.k.a.~irrelevant token)}%-\qstar\qstar^\top
\end{cases}\label{eq:CGMM discriminative}
\qquad y=f(\sum_{t\in\Gc}\wstar^T\x_t)
%\,,\qquad  \qb_{t,\star}^\perp \text{ zero-mean stochastic}
\end{equation}

\paragraph{Multiple contexts}
\begin{align}\label{eq:primal_attn_multi}
\fat_{\thetab}(\X) = \inp{\ones\w^T}{\rho(\Q\X^T)\X}
\end{align}
$\W,\Q\in\R^{m\times d}$


\begin{equation}
\x_t | y = \begin{cases}
\qstar^{\ell} + y \wstar & \text{w.p.}~ \zeta~~~~~~~~\text{(a.k.a.~relevant token)}
\\
\z_t \sim \subg{\sigma^2\Iden} & \text{w.p.}~ 1-\zeta~~~~\text{(a.k.a.~irrelevant token)}%-\qstar\qstar^\top
\end{cases}\label{eq:CGMM_multi_context}
%\,,\qquad  \qb_{t,\star}^\perp \text{ zero-mean stochastic}
\end{equation}


\section{Previous discussions}
\gray{\paragraph{Previous discussion:}
Message: Impact of prompt at any layer is impact of primal \Attn.
\[
\text{before}:~y=\inp{\W}{\sft{\X^\top \X}\X>}\qquad\text{after}:~y=\inp{[\w~\W]}{\sft{\X_p^\top  \X}\X}=\text{before}+\w^\top \X\sft{\pb^\top \X}
\]

\begin{align}
&\text{before}:~y=\inp{\W}{\sft{\X^\top \X}\X}
\\
&\text{after}:~ \mathbf{O}=\sft{\X_{\pb}\X^\top}\X,\quad y=\inp{\w}{\mathbf{o}_{T+1}}=\inp{\w}{\sft{\pb^\top  \X}\X}
\end{align}

\begin{align}
\mathbf{O}=\sft{\X_{\pb}\X_{\pb}^\top}\X_{\pb}
\end{align}
The last output token is
\begin{align}
    \mathbf{o}_{T+1} = \sum_{t=1}^{T}[\sft{\X_{\pb}\pb}]_t\x_t + [\sft{\X_{\pb}\pb}]_{T+1}\pb
\end{align}
and the output label is
\begin{align}\label{eq:CLS_label}
    \hat{y}=\inp{\w}{\mathbf{o}_{T+1}} = \sum_{t=1}^{T}[\sft{\X_{\pb}\pb}]_t\inp{\w}{\x_t} + [\sft{\X_{\pb}\pb}]_{T+1}\inp{\w}{\pb}.
\end{align}

\textbf{Goal:} Show that when data $\X$ comes from our GMM parameterized by some $\qstar,\wstar$ then training $\pb$ and $\w$ in \eqref{eq:CLS_label} achieves good generalization.
}

==> gradient_analysis_backup_Feb2023.tex <==
\section{Proofs for finite-sample Gradient Analysis in Section \ref{sec:finite analysis}}\label{sec:proofs grad finite}




% \subsection{Finite-sample Analysis}
In this section, we focus on finite-sample analysis of Algorithm \ref{eq:algo}. Introduce the following shorthand notation analogous to the population counterparts in Section \ref{sec:population analysis main}:
\begin{align}
&\widehat\G_\qb(\qb,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) = \frac{1}{n}\sum_{i\in[n]} (y_i-f_{\thetab}(\X_i)) \X_i^\top\sftd{\X_i\qb}\,\X_i \w \nn
\\
&\widehat\G_\w(\qb,\w):=-\nabla_{\w}\Lch_{\Dc}(\thetab) = \frac{1}{n}\sum_{i\in[n]} (y_i-f_{\thetab}(\X_i)) \X_i^\top\sft{(\X_i\qb)} .
\end{align}


\subsection{Gradient Calculations}
We begin with the gradient calculations for the first two steps of the algorithm.

For convenience, we make use of the following shorthands
\begin{subequations}\label{eq:gradient_term_notations}
\begin{align*}
\corq&:=\corqarg{\w}:=\w^\top\qb_\star,
\qquad\corw:=\corwarg{\w}:=\w^\top\w_\star,\qquad\alpha_i:=\alpha(\w,y_i):=\corq+y_i\corw, \\
\gammab_i&:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\qquad
\beta_i:=\beta(\Z_i;\w)=\gammab_i^T\w, \qquad
\hat\Sigmab_i:=\frac{1}{T}\Z_i^T\Z_i.
\end{align*}
\end{subequations}
for $\Z_i\in\R^{(1-\zeta)T \times d}$ is the matrix of irrelevant tokens $\zti, t\in\Rcc$ for sample $i\in[n].$

\begin{lemma}\label{lem:w_der_finite}
 Under dataset model \eqref{eq:CGMM} and Assumption \ref{ass:noise}, we have
\begin{align}
\Ghat_\w(0,0)
&=  \zeta \w_\star + \zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ \frac{1}{n}\sum_{i}y_i\gammab_i.
\end{align}
% where $\hat{Y}:=\frac{1}{n}\sum_{i\in[n]}y_i$ and $\Z_{i}\in\R^{(1-\zeta)T\times d}$ is the matrix of noisy tokens for sample $i\in[n]$. 
% That is, 
% \begin{align}
% \Ghat_\w(0,0)\,|\,\y\sim \subg{ \zeta \hat{Y} \qb_\star + \zeta \w_\star, \sigma^2(1-\zeta)\Iden}.
%\end{align}
\end{lemma}



\begin{lemma}\label{lem:q_der_finite} Under dataset model \eqref{eq:CGMM} and Assumption \ref{ass:noise}, we have that
%for $\w=\mu\w_\star+\tau\qb_\star+\etab$, $\etab\sim\subg{\alpha^2\Id}$, we have that 
\begin{align}\label{eq:q_der_finite}
\Ghat_\qb(0,\w):=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)\left(\qstar + y_i\wstar\right)
+ \hat\Sigmab_i\w
- (\zeta\alpha_i+\beta_i)\gammab_i
\right]\,.
\end{align}
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:w_der_finite}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By direct computation,
\begin{align}
\hat\G_\w(0,0):=-\nabla_{\w}\Lch_{\Dc}(\thetab) 
&= \frac{1}{nT}\sum_{i\in[n]}y_i\X_i^T\ones_T = \frac{1}{nT}\sum_{i\in[n]}\sum_{t\in[T]}y_i\x_{i,t} \nn
\\
&=\frac{1}{n}\big(\sum_{i\in[n]}\zeta_iy_i\big) \qb_\star
+\frac{1}{n}\big(\sum_{i\in[n]}\zeta_i\big) \w_\star
+\frac{1}{n}\sum_{i\in[n]}y_i \zai \nn
\end{align}
where $\zeta_i$ is the fraction of relevant tokens in the $i$-th sample and $\zai=\frac{1}{T}\sum_{t=1}^{T}\z_{i,t}$ where we again set noise $\z_t=0$ for relevant tokens. %The desired follows by recognizing that $y_i\z_{i,t}\sim\subg{\sigma^2\Id}$ for irrelevant tokens and using simplifying Assumption \ref{ass:zeta}.


% \subsection{Proof of New Lemma 4}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recall that $\phi^\prime(Xq)=\text{diag}\left(\phi'(\X\qb)\right)-\phi'(\X\qb)\phi'(\X\qb)^T$; hence, for $\thetab=(\qb,\w)$:
% \begin{align*} 
% \hat\G_\qb(\qb,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) 
% &= \frac{1}{n}\sum_{i\in[n]} \underbrace{(y_i-f_{\thetab}(\X_i)) \X_i^\top\text{diag}\left(\phi'(\X_i\qb)\right)\X_i\w}_{\term{1,i}} \\
% &\quad\quad- \frac{1}{n}\sum_{i\in[n]} \underbrace{{(y_i-f_{\thetab}(\X_i)) \X_i^\top\phi'(\X_i\qb)\phi'(\X_i\qb)^T\X_i \w}}_{\term{2,i}}.
% \end{align*}
% Moreover, note that, 
% \begin{align}
% f_{\thetab}(\X_i)&=\w^T\X_i^T\phi\left(\X_i\qb\right), \nn \\
% \X_i^\top\X_i &= \zeta T(\qb_\star + y_i \w_\star) (\qb_\star + y \w_\star)^\top + \Z_i^\top\Z_i,\nn\\
% \X_i^\top\ones &= \zeta T (\qb_\star + y_i \w_\star) + \Z_i^\top\ones.\nn
% \end{align}
% where recall the notation in Lemma \ref{lem:w_der_finite} for $\Z_i.$ Hence, using the lemma's notation (repeated here for convenience)
% \begin{align*}
% \alpha_i&:=\corq+y_i\corw, \\
% \beta_i&:=\beta(\Z_i;\w):=\frac{1}{T}\ones^T\Z_i\w, \\
% \gammab_i&:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\\
% \hat\Sigmab_i&:=\frac{1}{T}\Z_i^T\Z_i.
% \end{align*}
% we find that
% \begin{align}
% y_i-f_{\thetab}(\X_i) &= y_i - \zeta \alpha_i-\beta_i
% \\
% \frac{1}{T}\X_i\X_i^\top\w&=\zeta \alpha_i\qstar + \zeta y_i \alpha_i \wstar+\hat\Sigmab_i\w
% \\
% \frac{1}{T^2}{\X_i^\top\ones\ones^\top\X_i\w}&=\zeta\left(\zeta  \alpha_i+\beta_i\right) \qstar + \zeta\left(\zeta  \alpha_i+\beta_i\right) y_i \wstar 
% +\left(\zeta  \alpha_i+\beta_i\right)\gammab_i.
% \end{align}


% With the above, each one of the two terms becomes:

% \begin{align}
% \term{1,i}= \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta \alpha_i \qstar + 
% \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta  \alpha_i y_i \wstar + \left(y_i - \zeta \alpha_i-\beta_i\right)\hat\Sigmab_i\w
% \end{align}

% \begin{align}
% \term{2,i}= \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\qstar + 
% \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right) y_i\wstar + \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\gammab_i
% \end{align}

% Combining the above:

% \begin{align}
% {\term{1,i}-\term{2,i}}=\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
% \zeta\left((1-\zeta)\alpha_i-\beta_i\right)\left(\qstar + y_i\wstar\right)
% + \hat\Sigmab_i\w
% - (\zeta\alpha_i+\beta_i)\gammab_i
% \right]
% \end{align}


%\subsubsection{Remarks}

% \begin{remark}
% Lemma \ref{lem:q_der_pop} follows by Lemma \ref{lem:q_der_finite} by choosing $\w=\alpha\wstar$ and letting $n\rightarrow\infty$. To see this note that for this choise of $\w$, $\alpha_i=y_i\alpha\|\wstar\|^2$. Hence, recalling the shorthand $B:=\alpha\|\wstar\|^2$ the $\qstar$ direction in \eqref{eq:q_der_finite} is
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B)-\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \qstar
% \end{align*}
% Let $n\rightarrow\infty$ and apply law of large numbers with recalling that $$\E[y]=0, ~~\E[y\beta]=0,~~ \E[y^2]=1 ~~\text{and}~~ \E[\beta^2]=\frac{1}{T^2}\alpha^2\E[(\wstar^T\Z_i^T\ones)^2]=\frac{\alpha\sigma^2(1-\zeta)B}{T}.$$ This evaluates the coefficient of $\qstar$ above to:
% \begin{align}
% (1-\zeta B) (\zeta-\zeta^2) B +\frac{\alpha\sigma^2(\zeta-\zeta^2)B}{T} = \left[ \left(\zeta-\zeta^2\right)(1+\alpha\sigma^2/T)-\left(\zeta^2-\zeta^3\right)B \right] B.
% \end{align}

% Similarly, it can be shown that the $\wstar$ direction in \eqref{eq:q_der_finite}, i.e.
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left((1 - \zeta B)-y_i\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \wstar
% \end{align*}
% is zero. This is because $\E[y]=0$, $\E[\beta]=0$ and $y,\beta$ are independent.

% Next, take the $\hat\Sigmab_i\w$ direction:
% \begin{align}\label{eq:q_der_finite}
% \frac{\alpha}{n}\sum_{i=1}^{n}\left(y_i (1- \zeta B)-\beta_i\right)  \hat\Sigmab_i\w_\star
% \end{align}
% The first term is asymptotically zero by independence of $y_i,\hat\Sigmab_i$ and by $\E[y]=0$. The second term involves
% $$
% \E\left[(\w_\star^T\Z^T\ones)\Z^T\Z\w_\star\right]=0
% $$
% which is zero by assumption on third moments of $\Z$ being zero.

% Finally, consider the $\gammab_i$ direction:
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B) - \beta_i\right) 
% (\zeta y_i B+\beta_i)\gammab_i 
% \end{align*}
% The only term that survives zero-mean assumption of $y$, zero mean of $\gammab$ and independence of $y,\gammab_i$ is the term:
% $$
% \E\left[\beta^2\gammab\right] = \frac{1}{T^3}\E\left[\left(\w_\star^T\Z^T\ones\right)^2\Z^T\ones\right],
% $$
% which is again zero because of third moment of $\Z$ being zero.

% \end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:q_der_finite}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recall that $\phi^\prime(0)=\frac{1}{T}\Id-\frac{1}{T^2}\ones\ones^T$; hence, for $\thetab=(0,\w)$:
\begin{align*} 
\hat\G_\qb(0,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) 
&= \frac{1}{n}\sum_{i\in[n]} \underbrace{\frac{1}{T}(y_i-f_{\thetab}(\X_i)) \X_i^\top\X_i\w}_{\term{1,i}} - \frac{1}{n}\sum_{i\in[n]} \underbrace{{\frac{1}{T^2}(y_i-f_{\thetab}(\X_i)) \X_i^\top\ones\ones^\top\X_i \w}}_{\term{2,i}}.
\end{align*}
Moreover, note that, 
\begin{align}
f_{\thetab}(\X_i)&=\frac{1}{T}\w^T\X_i^T\ones, \nn \\
\X_i^\top\X_i &= \zeta T(\qb_\star + y_i \w_\star) (\qb_\star + y_i \w_\star)^\top + \Z_i^\top\Z_i,\nn\\
\X_i^\top\ones &= \zeta T (\qb_\star + y_i \w_\star) + \Z_i^\top\ones.\nn
\end{align}
where recall the notation in Lemma \ref{lem:w_der_finite} for $\Z_i.$ Hence, using the lemma's notation (repeated here for convenience)
\begin{align*}
\alpha_i&:=\corq+y_i\corw, \quad
\beta_i:=\beta(\Z_i;\w):=\frac{1}{T}\ones^T\Z_i\w, \quad
\gammab_i:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\quad
\hat\Sigmab_i:=\frac{1}{T}\Z_i^T\Z_i.
\end{align*}
we find that
\begin{align}
y_i-f_{\thetab}(\X_i) &= y_i - \zeta \alpha_i-\beta_i
\\
\frac{1}{T}\X_i\X_i^\top\w&=\zeta \alpha_i\qstar + \zeta y_i \alpha_i \wstar+\hat\Sigmab_i\w
\\
\frac{1}{T^2}{\X_i^\top\ones\ones^\top\X_i\w}&=\zeta\left(\zeta  \alpha_i+\beta_i\right) \qstar + \zeta\left(\zeta  \alpha_i+\beta_i\right) y_i \wstar 
+\left(\zeta  \alpha_i+\beta_i\right)\gammab_i.
\end{align}


With the above, each one of the two terms becomes:

\begin{align}
\term{1,i}= \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta \alpha_i \qstar + 
\left(y_i - \zeta \alpha_i-\beta_i\right)\zeta  \alpha_i y_i \wstar + \left(y_i - \zeta \alpha_i-\beta_i\right)\hat\Sigmab_i\w
\end{align}

\begin{align}
\term{2,i}= \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\qstar + 
\zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right) y_i\wstar + \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\gammab_i
\end{align}

Combining the above:

\begin{align}
{\term{1,i}-\term{2,i}}=\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
\zeta\left((1-\zeta)\alpha_i-\beta_i\right)\left(\qstar + y_i\wstar\right)
+ \hat\Sigmab_i\w
- (\zeta\alpha_i+\beta_i)\gammab_i
\right]
\end{align}


%\subsubsection{Remarks}

% \begin{remark}
% Lemma \ref{lem:q_der_pop} follows by Lemma \ref{lem:q_der_finite} by choosing $\w=\alpha\wstar$ and letting $n\rightarrow\infty$. To see this note that for this choise of $\w$, $\alpha_i=y_i\alpha\|\wstar\|^2$. Hence, recalling the shorthand $B:=\alpha\|\wstar\|^2$ the $\qstar$ direction in \eqref{eq:q_der_finite} is
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B)-\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \qstar
% \end{align*}
% Let $n\rightarrow\infty$ and apply law of large numbers with recalling that $$\E[y]=0, ~~\E[y\beta]=0,~~ \E[y^2]=1 ~~\text{and}~~ \E[\beta^2]=\frac{1}{T^2}\alpha^2\E[(\wstar^T\Z_i^T\ones)^2]=\frac{\alpha\sigma^2(1-\zeta)B}{T}.$$ This evaluates the coefficient of $\qstar$ above to:
% \begin{align}
% (1-\zeta B) (\zeta-\zeta^2) B +\frac{\alpha\sigma^2(\zeta-\zeta^2)B}{T} = \left[ \left(\zeta-\zeta^2\right)(1+\alpha\sigma^2/T)-\left(\zeta^2-\zeta^3\right)B \right] B.
% \end{align}

% Similarly, it can be shown that the $\wstar$ direction in \eqref{eq:q_der_finite}, i.e.
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left((1 - \zeta B)-y_i\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \wstar
% \end{align*}
% is zero. This is because $\E[y]=0$, $\E[\beta]=0$ and $y,\beta$ are independent.

% Next, take the $\hat\Sigmab_i\w$ direction:
% \begin{align}\label{eq:q_der_finite}
% \frac{\alpha}{n}\sum_{i=1}^{n}\left(y_i (1- \zeta B)-\beta_i\right)  \hat\Sigmab_i\w_\star
% \end{align}
% The first term is asymptotically zero by independence of $y_i,\hat\Sigmab_i$ and by $\E[y]=0$. The second term involves
% $$
% \E\left[(\w_\star^T\Z^T\ones)\Z^T\Z\w_\star\right]=0
% $$
% which is zero by assumption on third moments of $\Z$ being zero.

% Finally, consider the $\gammab_i$ direction:
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B) - \beta_i\right) 
% (\zeta y_i B+\beta_i)\gammab_i 
% \end{align*}
% The only term that survives zero-mean assumption of $y$, zero mean of $\gammab$ and independence of $y,\gammab_i$ is the term:
% $$
% \E\left[\beta^2\gammab\right] = \frac{1}{T^3}\E\left[\left(\w_\star^T\Z^T\ones\right)^2\Z^T\ones\right],
% $$
% which is again zero because of third moment of $\Z$ being zero.

% \end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Concentration of Gradient \texorpdfstring{$\Ghat_\qb{(0,\w)}$}{} in the \texorpdfstring{$\qb$}{context} direction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main result of this section is the following lemma about concentration of gradient with respect to $\qb$.

\begin{lemma}[Concentration of $\Ghat_\qb(0,\w)$]\label{lem:conc_grad_q}
Fix any vectors $\vb,\w\in\R^d$. For convenience define $\corqv:=\vb^T\qstar$ and $\corwv:=\vb^T\wstar$ and recall $\corw,\corq$ notations from Lemma \ref{lem:q_der_finite}. Then, we can decompose
\[
\vb^T\Ghat_\qb(0,\w) =\vb^T\G_\qb(0,\w) + \vb^T\Gtilde_\qb(0,\w),
\]
where the expectation term is given by 
    \begin{align}
\vb^T\G_\qb(0,\w):=\E\left[\vb^T\Ghat_\qb(0,\w)\right] 
&= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
\\ 
&
+\left(\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \right)\,\corqw -\left(\left(1+{2}/{T}\right)(\zeta-\zeta^2)\corq\right)\vb^T\Sigmab\w
\label{eq:mean_one_step_grad_q}
\end{align}
and the deviation term obeys
\begin{align}
\vb^T\Gtilde_\qb(0,\w) 
&=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
\\
&\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
\\
&\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad
+\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
\\
&\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
\\
&\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
\\
&\qquad\qquad\qquad- 
\zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
\\
&\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
\\
&\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
\\
&\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right).\label{eq:Ghat full}
\end{align}
Moreover, all random terms in \eqref{eq:Ghat full} are zero-mean and concentrate as prescribed by
Lemma \ref{lem:psi} below
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Main concentration lemma]\label{lem:psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $y_i, i\in[n]$ be iid Rademacher random variables. Let $\Z_i\in\R^{(1-\zeta)T \times d}, i\in[n]$ be iid copies of a random matrix $\Z$. Each row  $\z_t, t\in[(1-\zeta)T]$ of $\Z$ is an iid copy of a random vector $\z$ satisfying Assumption \ref{ass:noise}. For convenience denote $\gammab_i:=\Z_i^T\ones/T$ and $\hat\Sigmab_i:=\Z_i^T\Z_i/T$. Then, the following statements are true for all vectors $\w,\vb\in\R^{d}$.
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}y_i}{2}&\leq \frac{C}{\sqrt{n}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\gammab_i^T\w}{2} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\gammab_i^T\w}{2} &\leq \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2}{\sqrt{nT}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right) - \frac{1-\zeta}{T}\vb^T\Sigmab\w}{1} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)}{1} &\leq \frac{C\sigma^2(1-\zeta)\|\w\|_2\|\vb\|_2}{T\sqrt{n}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\w^T\hat\Sigmab_i\vb-{(1-\zeta)}\w^T\Sigmab\vb}{1} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\w^T\hat\Sigmab_i\vb  }{1}&\leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\left(\gammab_i^T\w\right)^2-\frac{1-\zeta}{T}{\w^T\Sigmab\w}\right)\gammab_i^T\vb}{2/3}&\leq \frac{C\sigma^3(1-\zeta)^{3/2}\|\w\|_2^2\|\vb\|_2}{T^{3/2}\sqrt{n}}\log n
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3} &\leq \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T\sqrt{n}}}\log n
\end{align*}
Also, all the random variables that appear above are zero mean.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsubsection{Proof of Lemma \ref{lem:conc_grad_q}}

We split \eqref{eq:q_der_finite} in four terms and handle each of them separately.

\noindent\textbf{$\bullet$~~ $\term{I}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)\qstar$}\\
We first focus on
\begin{align*}
\term{I}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i(1-\zeta\corw) -\beta_i- \zeta \corq\right) 
\left(y_i(\zeta-\zeta^2)\corw-\zeta\beta_i+(\zeta-\zeta^2)\corq\right)\qstar=:A\qstar.
\end{align*}
We we can express $A$ above conveniently as follows (recall $y_i^2=1$):
\begin{align*}
A&:=-\zeta(\zeta-\zeta^2)\corq^2+(1-\zeta\corw)(\zeta-\zeta^2)\corw +\left((1-\zeta\corw)(\zeta-\zeta^2)\corq-\zeta(\zeta-\zeta^2)\corw\corq\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right)
\\
&\qquad\qquad+\left(-(\zeta-\zeta^2)\corq+\zeta^2\corq\right)\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\left(-(1-\zeta\corw)\zeta-(\zeta-\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\beta_i\right)
+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2\right)
\\
&=(\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right)
\\
&\qquad\qquad+\left(-\zeta+2\zeta^2\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\beta_i\right)
\\
&\qquad\qquad+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)+\frac{(\zeta-\zeta^2)}{T}\w^T\Sigmab\w.
\end{align*}
From Lemma \ref{lem:psi}, all random terms above are zero mean. Hence,
\begin{align}
\E[A]&=-(\zeta^2-\zeta^3)\corq^2+(1-\zeta\corw)(\zeta-\zeta^2)\corw+(\zeta-\zeta^2)\frac{\w^T\Sigmab\w}{T} \nn
\\
&=-(\zeta^2-\zeta^3)\corq^2+(\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\corw^2 \nn
\\
&=(\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right).\label{eq:Exp_term1}
\end{align}
%We will show that for all $0<t<\sqrt{n}$:
%\begin{align}
%\Pr\left(|A-\E[A]|\leq \frac{C\sigma\|\w\|_2 t}{\sqrt{n}} \right)\geq 1-2e^{-t^2}.
%\end{align}
%Indeed, 


\vp
\noindent\textbf{$\bullet$~~$\term{II}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)y_i\wstar$}\\
\begin{align*}
\term{II}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i(1-\zeta\corw) -\beta_i- \zeta \corq\right) 
\left(y_i(\zeta-\zeta^2)\corw-\zeta\beta_i+(\zeta-\zeta^2)\corq\right)y_i\wstar=B\wstar.
\end{align*}
We we can express $B$ above conveniently as:
\begin{align*}
B&:=\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\left(\frac{1}{n}\sum_{i\in[n]}y_i\right)  +\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq
\\
&\qquad\qquad+\left(-\zeta+2\zeta^2\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}\beta_iy_i\right)
+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2y_i\right).
\end{align*}
%where we also used that $y_i^2=1$.
All the random terms above are zero-mean. Hence,
\begin{align}
\E[B]&=\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\,.
\label{eq:Exp_term2}
\end{align}


% Clearly this is a zero-mean random variable since $\beta_i,y_i$ are independent and $\E[y_i]=0$. Further note that 
% \begin{align}
% \beta_i^2y_i = (1-\zeta)^2\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}y_i\z_{t,i}^T\w\right)\widesim{D} (1-\zeta)^2\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\wt\z_{t,i}^T\w\right),
% \end{align} 
% where $\wt\z_{i,t}\widesim{D}\z_{i,t}$ and $\wt\z_{i,t}$ are independent for all $t$. Hence,
% \begin{align}
% \|\beta_i^2y_i\|_{\psi_1}\leq (1-\zeta)^2\|\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\|_{\psi_2}\|\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\wt\z_{t,i}^T\w\right)\|_{\psi_2}\leq C(1-\zeta) K^2\|\w\|_2^2/T
% \end{align}
% Thus,
% \begin{align}
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\beta_i^2\big| \leq  \frac{C\sigma^2(1-\zeta)\|\w\|_2^2}{T\sqrt{n}} t
% \right)&\geq 1-2{e^{-c\min\{{t^2,t\sqrt{n}}\}}}
% \end{align}

\vp
\noindent\textbf{$\bullet$~~ $\term{III}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
 \hat\Sigmab_i\w$}\\

Fix any vector $\vb:$

\begin{align*}
\vb^T\{\term{III}\} &= \left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) - \zeta \left(\corq+y_i\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w\right)-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\vb^T\hat\Sigmab_i\w\right)\\
&= \left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) - \zeta \corq\left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w\right)-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\vb^T\hat\Sigmab_i\w\right)
\\
&= \left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) 
-
\zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right)-
 (\zeta-\zeta^2)\corq \vb^T\Sigmab\w
\\ &\qquad\qquad-
\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)+(1-\zeta)(\w^T\Sigmab\vb)\frac{1}{n}\sum_{i=1}^{n}(\gammab_i^T\w)
\end{align*}

From Lemma \ref{lem:psi} all random terms above are zero mean. Hence,
\begin{align}
\E\left[\vb^T\{\term{III}\}\right] = -(\zeta-\zeta^2)\corq \w^T\Sigmab\vb .\label{eq:Exp_term3}
%- (1-\zeta)\w^T\Sigmab\vb 
\end{align}
Moreover, from Lemma \ref{lem:psi} we have the following:

%\ct{We need a reference for the penultimate inequality in the above display: How it follows from last statement of Lemma \ref{lem:psi}}

\vp
\noindent\textbf{$\bullet$~~ $\term{IV}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)\gammab_i$}\\

For fixed vector $\vb$, $
    \vb^T\{\term{IV}\} = \frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)\vb^T\gammab_i.
$
Reorganizing, note that
\begin{align*}
\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)  &= \zeta y_i (\corq+y_i\corw) - \zeta^2(\corq^2+\corw^2+2y_i\corq\corw)-2\zeta\corq\beta_i-2\zeta\corw y_i\beta_i+y_i\beta_i-\beta_i^2\\
&= \left(\zeta\corq -2 \zeta^2\corq\corw\right) y_i + \left(\zeta\corw - \zeta^2(\corq^2+\corw^2)\right) -\left(2\zeta\corq\right)\beta_i+\left(1-2\zeta\corw\right) y_i\beta_i-\beta_i^2
\end{align*}

Overall,
\begin{align*}
    \vb^T\{\term{IV}\} &=\left(\zeta\corw - \zeta^2(\corq^2+\corw^2)\right) \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right)+\left(\zeta\corq -2 \zeta^2\corq\corw\right)\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right)
    \\
    &+\left(1-2\zeta\corw\right) \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right)
    \\
    &-\left(2\zeta\corq\right)\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right)-\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
    \\
    &- \frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)
+\frac{(1-\zeta)}{T}\w^T\Sigmab\w \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\right)
\end{align*}
According to Lemma \ref{lem:psi} all random terms above are zero mean. Thus,
\begin{align}
\E\left[\vb^T\{\term{IV}\}\right] &= -2\zeta\corq\frac{1-\zeta}{T}\w^T\Sigmab\vb
\label{eq:Exp_term4}
\end{align}


\vp
\noindent\textbf{$\bullet$~~ Combined} \\
The desired identities \eqref{eq:mean_one_step_grad_q} and \eqref{eq:Ghat full} follow by combining all the terms above. 


% We now combine all the above. For convenience define $\corqv:=\vb^T\qstar$ and $\corwv:=\vb^T\wstar$. Then, we have shown:
% \[
% \vb^T\Ghat_\qb(0,\w) =\vb^T\G_\qb(0,\w) + \vb^T\Gtilde_\qb(0,\w),
% \]
% where
% \begin{align}
%     \vb^T\G_\qb(0,\w) 
% &:=\E\left[\vb^T\Ghat_\qb(0,\w)\right] \nn \\
% &=\Big[\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corqv + \left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corwv  \nn
% \\&\qquad\qquad+{(\zeta-\zeta^2)\corqv}\left(\w^T\Sigmab\w/T\right)
% -(\zeta-\zeta^2)\corq \vb^T\Sigmab\w
% -\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
% \Big] \nn
% \\
% &= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
% \\&\qquad\qquad+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \,\corwv-(\zeta-\zeta^2)\corq \w^T\Sigmab\vb -2\zeta\corq\frac{1-\zeta}{T}\w^T\Sigmab\vb\nn
% \\
% &= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
% \\ 
% &\qquad\qquad 
% +\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \,\corwv
%  -\left(1+\frac{2}{T}\right)(\zeta-\zeta^2)\corq\vb^T\Sigmab\w
%  \label{eq:gradient_mesh}
% \end{align}

% and 
% \begin{align}
% \vb^T\Gtilde_\qb(0,\w) 
% &=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
% \\
% &\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad
% +\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
% \\
% &\qquad\qquad\qquad- 
% \zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
% \\
% &\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right) \label{eq:Ghat full}
% \end{align}

% \begin{align}
% \vb^T\Ghat_\qb(0,\w) 
% &=\Big[\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corqv + \left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corwv  \nn
% \\&\qquad\qquad\qquad+{(\zeta-\zeta^2)\corqv}\left(\w^T\Sigmab\w/T\right)
% -(\zeta-\zeta^2)\corq \vb^T\Sigmab\w
% -\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
% \Big] \nn
% \\
% &\qquad+\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
% \\
% &\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad
% +\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
% \\
% &\qquad\qquad\qquad- 
% \zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
% \\
% &\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right) \label{eq:Ghat full}
% \end{align}



%%%%%%%%%%% CHRISTOS CONCENTRATION
% \begin{align*}
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\big| \leq \frac{C}{\sqrt{n}}u\right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)\big| \leq \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2 }{\sqrt{nT}} u
% \right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\left(\gammab_i^T\w\right)\big| \leq C \frac{\sqrt{(1-\zeta)}K\|\w\|_2}{\sqrt{n T}} u
% \right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\big| \leq C \frac{{(1-\zeta)}K^2\|\w\|_2^2}{{T\sqrt{n}}} u
% \right)&\geq 1-2{e^{-c\min\{u^2,u\sqrt{n}\}}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)^2y_i| \leq C \frac{{(1-\zeta)}K^2\|\w\|_2^2}{{T\sqrt{n}}} u
% \right)&\geq 1-2{e^{-c\min\{u^2,u\sqrt{n}\}}}
% \\
% \Pr\left(
%     |\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w| \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}} u
%     \right) &\geq 1-2e^{-c\min\{u^2,u\sqrt{n}\}}
% \\
%     \Pr\left(
%     |\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w - (1-\zeta)\w^T\Sigmab\vb| \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}} u
%     \right) &\geq 1-2e^{-c\min\{u^2,u\sqrt{n}\}}
% \\
%     \Pr\left(
%     \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)} \leq u\,\frac{C\sigma^3(1-\zeta)\|\w\|_2^2\|\vb\|_2}{T\sqrt{n}}\log{n}\, 
%     \right) &\geq 1-c'e^{-cu^{2/3}}
% \end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:psi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}
% ~

\vp
\noindent\underline{First bound:} Obvious by boundedness (hence, sub-gaussianity) of $y_i$ and Fact \ref{fact:psi_additive}.

\vp
\noindent\underline{Second bound:} For convenience set $\wt T=(1-\zeta)T$ and assume wlog that $\Rcc=[\wt T].$  Recall that $$\beta_i=\frac{1}{T}\sum_{t=1}^{\wt T} \z_{i,t}^T\w=\frac{1-\zeta}{\wt T} \sum_{t=1}^{\wt T}\z_{i,t}^T\w.
$$
Also
for all $t$: $\psinorm{\z_{i,t}^T\w}{2}\leq K\|\w\|_2$. Thus, from Fact \ref{fact:psi_additive}:
\begin{align}\label{eq:beta_psi2}
\psinorm{\beta_i}{2} \leq \frac{C\sigma(1-\zeta)\|\w\|_2}{\sqrt{\wt T}} = \frac{C\sigma\sqrt{(1-\zeta)}\|\w\|_2}{\sqrt{ T}}
\end{align}
The bound then follows by applying Fact \ref{fact:psi_additive} once more.  

For the second term in this bound  recall that $y_i\in\{\pm{1}\}$ and $\beta_i=\sum_t \z_{i,t}^T\w/T$. Also, for all $i\in[n]$: $y_i,\{\z_{i,t}\}_{t}$ are zero-mean and independent. Thus (i) $\E[y_i\beta_i]=0$, and (ii)  {$\{y_i\z_{i,t}\widesim{D} \z_{i,t} \text{ and } y_i\z_{i,t} \perp y_i\z_{i,t'} \} \implies y_i\beta_i\widesim{D} \beta_i$.} Thus, the same bound as the first term holds.

\vp
\noindent\underline{Third bound:} It is easy to compute 
\begin{align}\label{eq:beta2_expectation}
\E[\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]=\frac{1}{T^2}\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\w^T\z_{i,t}\z_{i,t'}\vb] = \frac{1-\zeta}{T}\vb^T\Sigmab\w,
\end{align} 
and, using \eqref{eq:beta_psi2}
\begin{align}\label{eq:beta2_psi1}
\psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)-\E[\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]}{1} \leq C \psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)}{1} \leq  C \psinorm{\gammab_i^T\w}{2}\psinorm{\gammab_i^T\vb}{2} = \frac{C\sigma^2{(1-\zeta)}\|\w\|_2\|\vb\|_2}{{T}}.
\end{align}
Since $\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right), i\in[n]$ are independent, the desired bound on the first term follows from Fact \ref{fact:psi_additive}.

Consider now the second term. By independence of $y_i, \gammab_i$ it holds that $\E[y_i\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]=0$. Arguing as we did above for the second bound, $y_i\gammab_i^T\w\widesim{D} \gammab_i^T\w$. Hence, the subexponential bound is the same as for the first term.


\vp
\noindent\underline{Fourth bound:} First, it is easy to compute that for all $i\in[n]$:
$$
\E[\w^T\Sigmab_i\vb]=\frac{1}{T}\E[\w^T\Z_i^T\Z_i\vb] = \frac{1}{T}\sum_{t=1}^{\wt T}\E[\w^T\z_{i,t}^T\z_{i,t}\vb] = \frac{\wt T}{T}\w^T\Sigmab\vb = (1-\zeta)\w^T\Sigmab\vb.
$$
Thus,
\begin{align*}
\w^T\hat\Sigmab_i\vb-\E[\w^T\hat\Sigmab_i\vb]=\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb
%=\frac{1}{T}\w^T\Z_i^T\Z_i\vb-(1-\zeta)\w^T\Sigma \vb
=\frac{1}{T}\sum_{t=1}^{\wt T}\Big((\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\Big)
\end{align*}
and so
\begin{align*}
\frac{1}{n}\sum_{i=1}^{n}\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb
%=\frac{1}{T}\w^T\Z_i^T\Z_i\vb-(1-\zeta)\w^T\Sigma \vb
=\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^{\wt T}\Big((\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\Big).
\end{align*}
Now, each random variable in the double sum above is independent and such that
\begin{align}\label{eq:wSv}
\|(\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\|_{\psi_1}\le 2\|(\z_{i,t}^T\w)(\z_{i,t}^T\vb)\|_{\psi_1}\le 2\|\z_{i,t}^T\w\|_{\psi_2}\|\z_{i,t}^T\vb\|_{\psi_2}\le C\sigma^2\|\w\|_2\|\vb\|_2.
\end{align}
Hence, from Fact \ref{fact:psi_additive},
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i=1}^{n}\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb}{1}\leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}}
\end{align*}


The bound for the second term follows along the same lines. The two key observations are that (i) $\E[y_i\w^T\hat\Sigmab_i\vb]=0$ because $y_i$ and $\z_{i,t}$ are independent, and, (ii) 
\begin{align*}
y_i\w^T\hat\Sigmab_i\vb=
\frac{1}{T}\w^Ty_i\Z_i^T\Z_i\vb \widesim{D} \frac{1}{T}\w^T\wt\Z_i^T\Z_i\vb
=\frac{1}{T}\sum_{t=1}^{\wt T}(\wt\z_{i,t}^T\w)(\z_{i,t}^T\vb)
\end{align*}
where $\wt\Z_i$ is an independent copy of $\Z_i$.

\vp
\noindent\underline{Fifth bound:}From \eqref{eq:beta2_psi1} and \eqref{eq:beta2_expectation}, we have for all $i\in[n]$ that
\begin{align*}\label{eq:beta2_psi1}
\psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)-\frac{1-\zeta}{T}\w^T\Sigmab\w}{1} \leq \frac{C\sigma^2{(1-\zeta)}\|\w\|_2^2}{{T}}.
\end{align*}
Moreover, recall from Eq. \eqref{eq:beta_psi2} that
$$
\psinorm{\gammab_i^T\vb}{2}\leq  \frac{C\sigma\sqrt{1-\zeta}\|\vb\|_2}{\sqrt{ T}}.
$$
Combining the above two displays and applying Fact \ref{fact:orlitz_inequality} we find for all $i\in[n]$ that
\begin{align}
\psinorm{\left(\left(\gammab_i^T\w\right)^2-\frac{1-\zeta}{T}{\w^T\Sigmab\w}\right)\gammab_i^T\vb}{2/3}&\leq \frac{C\sigma^3(1-\zeta)^{3/2}\|\w\|_2^2\|\vb\|_2}{T^{3/2}}.
\end{align}
The desired bound follows from the above after using Fact \ref{fact:psi_heavy_Talagrand}.


\vp
\noindent\underline{Sixth bound:}
From Eq. \eqref{eq:wSv}:
$$
\psinorm{\w^T\hat\Sigmab_i\vb - (1-\zeta)\w^T\Sigmab\vb}{1} \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{T}}
$$
and from Eq. \eqref{eq:beta_psi2}
$$
\psinorm{\gammab_i^T\w}{2}\leq  \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2}{\sqrt{ T}}.
$$
Next we use Fact \ref{fact:orlitz_inequality} with $\alpha=2$ and $\beta=1$ to find that 
\begin{align*}
\psinorm{\left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3} \leq 
 \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T}}
\end{align*}
Next we use Fact \ref{fact:psi_heavy_Talagrand} which allows us to conclude that 
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3}\le  \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T\sqrt{n}}}\log n
\end{align*}
Finally, the zero-mean property follows since
\begin{align*}
\E[\left(\ones^T\Z_i\w\right)\left(\w^T\Z_i\Z_i^T\vb\right)] &= 
\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\left(\z_{i,t}^T\w\right)\left(\w^T\z_{i,t'}\z_{i,t'}^T\vb\right)]
= 
\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\w^T\z_{i,t}\tr\left({\z_{i,t'}\z_{i,t'}^T\vb\w^T}\right)]
\\
&=
\wt T^2\E[\tr\left(\z^T\w\right)\tr\left({\z\z^T\vb\w^T}\right)] = \wt T^2\E[\tr\left( (\z^T\w) \otimes (\z\z^T\vb\w^T)\right)]
\\
&=
\wt T^2\tr\left( \E[(\z^T\otimes \z\z^T)] (\w\otimes\vb\w^T)\right) = 0
\end{align*}
where the last equality follows by the zero third moment property in Assumption \ref{ass:noise}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finite-sample analysis: First and second gradient steps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The lemma below studies the deviation of the first-step of GD $\what_1$ with respect to its population counterpart $\w_1$.  Provided that $n$ and $n\zeta T /d$ are larger than appropriate functions of other problem parameters, then the deviations are of small multiplicative order. We remark that the constants below have not been optimized (eg. the factor $1/2$ in \eqref{eq:w1hat corr} is arbitrary and can be replaced by and small positive constant by appropriately increasing the constant $C$ in \eqref{eq:large n lemma}).
\begin{lemma}[First gradient step]\label{lem:1st gradient step}
Consider the one-step population and finite updates $\w_1=\eta\G_\w(0,0)$ and $\what_1=\eta\Ghat_\w(0,0)$, respectively. For convenience denote $\corw=\w_1^T\wstar, \corq=\w_1^T\qstar$ and $\hcorw=\what_1^T\wstar, \hcorq=\what_1^T\qstar$ their finite-sample counterparts.
Suppose for large enough absolute constant $C>0$ and any $u>0$,
\begin{align}\label{eq:large n lemma}
    \sqrt{n}&\geq C u 
    \qnorm/\wnorm
    %\left(1\maxi \abs{\rho}\qnorm/\wnorm \right)
    \qquad\text{and}\qquad
    \sqrt{n\zeta T}\geq C u \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}\, 
\end{align}
Then, for absolute constants $c,c'>0$ with probability at least $1-c'e^{-cu^2}$
    \begin{align}\label{eq:w1hat corr}
        \abs{\hcorw-\corw}\leq \corw/2\qquad\text{and}\qquad\abs{\hcorq-\corq}\leq \eta \zeta \,\qnorm\wnorm/2
    \end{align}
    Additionally, if 
    \begin{align}
    \sqrt{n}&\geq Cu\qnorm/\wnorm
    \qquad\text{and}\qquad
    \sqrt{n\zeta T}\geq Cu \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}  \sqrt{d}
\end{align}
then with the same probability 
\begin{align}\label{eq:w1hat norm}
    \abs{\tn{\what_1}-\tn{\w_1}}\leq\tn{\w_1}/2.
\end{align}
\end{lemma}
\begin{proof}
Note that the conclusions of the lemma are all homogeneous in $\eta$. Hence, without loss of generality, set $\eta=1$.

    By Lemma \ref{lem:w_der_finite},
    \begin{align}\label{eq:what_1 first eq}
\what_1=\Ghat_\w(0,0)
&=  \zeta \w_\star + \zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ 
\frac{1}{n}\sum_{i}y_i\gammab_i.
\end{align}
and recall $\w_1=\G_\w(0,0)=\zeta\wstar$ (thus, $\corw=\zeta\wnorm^2$).
From these, and also using Lemma \ref{lem:psi} , for any $u>0$ with probability at least $1-2e^{-cu^2}$
\begin{align}
\abs{\hcorw-\corw}&=\abs{\wstar^T(\what_1-\w_1)}\leq \zeta  \abs{\rho}\wnorm\qnorm \abs{\frac{1}{n}\sum_{i\in[n]}y_i}+ 
\abs{\frac{1}{n}\sum_{i}y_i\gammab_i^T\wstar}\leq  \frac{Cu\zeta   \abs{\rho}\wnorm\qnorm}{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\wnorm}{\sqrt{n\zeta T}}\nn
\\
&\leq \frac{\zeta \wnorm^2}{2}=\frac{\corw}{2}.\nn
\end{align}
where the last inequality follows by assuming $n,\zeta T$ large enough as in the condition of the lemma.
Similarly,  
\begin{align*}
\abs{\hcorq-\corq}=\abs{\qstar^T(\what_1-\w_1)}&\leq \zeta  \qnorm^2 \abs{\frac{1}{n}\sum_{i\in[n]}y_i}+ 
\abs{\frac{1}{n}\sum_{i}y_i\gammab_i^T\qstar}
\leq  \frac{Cu\zeta  \qnorm^2}{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\qnorm}{\sqrt{n\zeta T}}\nn\leq 
\frac{\zeta\qnorm\wnorm}{2}
%\red{\eps\zeta\qnorm(\qnorm+\wnorm)}
\end{align*}
for sufficiently large $n$ as in \eqref{eq:large n lemma}.

Finally, 
\begin{align}
    \tn{\what_1}-\tn{\w_1}\leq \tn{\what_1-\w_1}\leq \frac{Cu\zeta\qnorm }{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\sqrt{d}}{\sqrt{n\zeta T}}\leq \frac{\zeta\wnorm}{2}=\frac{\tn{\w_1}}{2} \label{eq:w1 norm diff}
\end{align}
where, again, the last inequality follows by assuming $n,\zeta T$ large enough as stated in the lemma. In the second inequality, we used from Lemma \ref{lem:psi} that $\sum_{i\in[n]}y_i\gammab_i/n$ is $C\sigma\sqrt{1-\zeta}/\sqrt{nT}$-subGaussian and applied Fact \ref{fact:norm subg} to get a high-probability bound on its euclidean norm.
\end{proof}



Next, we move on to the second gradient update in the direction of $\Ghat_\qb(0,\what_1).$ Recall our goal of controlling the relevance scores of signal and noisy tokens. The first lemma below takes a step in this direction by computing the signal and noise relevance scores assuming access to the population gradient $\G_\qb(0,\what_1):=\E\left[\Ghat_\qb(0,\what_1)\right].$
%
\begin{lemma}[$\Ghat_\qb(0,\cdot)$ control: Expectation term]\label{lem:finite q1 expectation}Let $\G_\qb(0,\w_1)=\E\left[\Ghat_\qb(0,\w_1)\right]$ be the expectation of a step in the $\qb$-gradient evaluated at $(0,\what_1)$ and recall that $\what_1=\eta\Ghat_\w(0,0)$ for $\eta>0.$ Suppose $\what_1$ satisfies \eqref{eq:w1hat corr} and \eqref{eq:w1hat norm}.
Further assume that the step-size $\eta$ satisfies the following for sufficiently small absolute constant $c_\eta>0$:
    \begin{align}\label{eq:eta small deviation}
    \eta<c_\eta \left(\wnorm^{-2}\maxi\qnorm^{-2}\maxi \sigma^{-2}\right)
    \end{align}
Then, for $y\in\{\pm1\}$ it holds that
\begin{align}
\left(\qstar+y\wstar\right)^T\G_\qb(0,\hat\w_1) &\geq  \eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(15-8\rho^2-6\abs{\rho}\right)\qnorm - \left(210\abs{\rho}+33\right)\wnorm \right)/64\,
   \label{eq:finite signal exp}
\end{align}
Moreover, for fresh noise variables $\z_t, t\in\Rcc$ satisfying Assumption \ref{ass:noise}, it holds that
\begin{align}
\z_t^T\G_\qb(0,\hat\w_1)\eqd\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \,\sigma\sqrt{3}\sqrt{(3/2)^4+2\left((1+1/(4\cdot 16^2))\rho^2+1/4\right)} \cdot G_t,\quad G_t\sim\subg{1} 
\label{eq:finite noise exp}
\end{align}
\end{lemma}

\begin{proof}
Fix any $\vb$ and recall the notation of Lemma \ref{lem:1st gradient step}. With these, we have from Lemma \ref{lem:conc_grad_q} that
\begin{align}
    \vb^T\G_\qb(0,\what_1)&=\left((\zeta-\zeta^2)\left(\hcorw+{\sigma^2\tn{\what_1}^2}/{T}\right)-(\zeta^2-\zeta^3)\left(\hcorw^2 + \hcorq^2\right)\right)\,\vb^T\qstar\nn
\\ 
&\qquad\qquad 
+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\hcorw\right)\hcorq \,\vb^T\wstar\nn
-\sigma^2\left(1+{2}/{T}\right)(\zeta-\zeta^2)\hcorq\vb^T\what_1
\\
&=(\zeta-\zeta^2)\hcorw\left(1+{\sigma^2\tn{\what_1}^2}/({T}\hcorw)-\zeta\left(\hcorw + \hcorq^2/\hcorw\right)\right)\,\vb^T\qstar\nn
\\ 
&\qquad\qquad 
+(\zeta-\zeta^2)\hcorq \,\left(1-2\zeta\hcorw\right)\,\vb^T\wstar\nn
-\sigma^2\left(1+{2}/{T}\right)(\zeta-\zeta^2)\hcorq\vb^T\what_1
\\
&=(\zeta-\zeta^2)\hcorw\underbrace{\left(1+{\sigma^2\tn{\what_1}^2}/({T}\hcorw)-\zeta\left(\hcorw + \hcorq^2/\hcorw\right)\right)}_{:=\Chat_1}\,\vb^T\qstar\nn
\\ 
&\qquad
+(\zeta-\zeta^2)\hcorq \,\underbrace{\left(1-2\zeta\hcorw-\eta\zeta\sigma^2\left(1+{2}/{T}\right)\right)}_{:=\Chat_2}\,\vb^T\wstar -\underbrace{\eta\sigma^2\left(1+{2}/{T}\right)}_{:=\Chat_3}(\zeta-\zeta^2)\hcorq\vb^T\deltab_1\nn
%\label{eq:q1hat exp}
% \\
% &=:(\zeta-\zeta^2)\left(A\,\vb^T\qstar+B\,\vb^T\wstar +D\,\vb^T\deltab_1\right)\label{eq:q1hat exp}
\end{align}
where we used \eqref{eq:what_1 first eq} and set $\deltab_1:=(\what_1-\w_1)/\eta=\zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ 
\frac{1}{n}\sum_{i}y_i\gammab_i.$

Recall that $\corw/2\leq \hcorw\leq 3\corw/2$, ${\corq}-\eta\zeta\qnorm\wnorm/2\leq \hcorq\leq {\corq}+\eta\zeta\qnorm\wnorm/2$ and $\tn{\w_1}/2\leq \tn{\what_1}\leq 3\tn{\w_1}/2$. Also, $\corw=\eta\zeta\wnorm^2$ $\corq=\eta\zeta\rho\wnorm\qnorm$ and $\tn{\w_1}=\eta\zeta\wnorm$. With these, we can set step size $\eta$  small enough such that 
$\Chat_1\in[1/2,3/2]$, $\Chat_2\in[-1/8,1]$ and $\Chat_3\in[0,1/(16 \zeta)]$.  
Also, recall from \eqref{eq:w1 norm diff}
$
\tn{\deltab_1}\leq \zeta\wnorm/2;
$
thus, 
\[
\Chat_3\abs{\hcorq}\tn{\deltab_1}\leq \frac{1}{16\zeta}\eta\zeta\qnorm\wnorm\left(\abs{\rho}+1/2\right)\frac{\zeta\wnorm}{2}=\eta\zeta\,\frac{(\abs{\rho}+1/2)\qnorm\wnorm^2}{32}\,.
\]
With these, we arrive at the following:
\begin{align}
    \qstar^T\G_\qb(0,\hat\w_1)\geq \eta\zeta(\zeta-\zeta^2)\left(\wnorm^2\qnorm^2/4-\abs{\rho}(\abs{\rho}+1/2)\qnorm^2\wnorm^2/8-(\abs{\rho}+1/2)\qnorm^2\wnorm^2/32\right)
    \geq  \eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm^2\left(15-8\rho^2-6\abs{\rho}\right)/64\nn
\end{align}
and for $y\in\{\pm1\}$
\begin{align}
\abs{y\wstar^T\G_\qb(0,\hat\w_1)}\leq \eta\zeta\left(\zeta-\zeta^2\right)\wnorm^3\qnorm\left(\abs{\rho}\left(9/4+1+1/32\right)+\left(1/2+1/64\right)\right)=\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^3\qnorm\left(\abs{\rho}\left(105/32\right)+33/64\right)\,.\nn
\end{align}
The above two displays put together yield \eqref{eq:finite signal exp}.

To see \eqref{eq:finite noise exp}, note that
% \[
% \z_t^T\G_\qb(0,\hat\w_1)\Big/(\zeta-\zeta)^2=\left(\Chat_1\hcorw\qb+\Chat_2\hcorq+\Chat_3\deltab_1\right)^T\z_t
% \]
$\z_t^T\wstar\sim\subg{\sigma\wnorm},$ $\z_t^T\qstar\sim\subg{\sigma\qnorm}$ and $\z_t^T\deltab_1\sim\subg{\sigma\tn{\deltab_1}}.$ Thus,  the noise relevant scores are \iid subgaussian random variables with sub-gaussian constant $\sigmahat$ upper bounded as follows
\begin{align}
\z_t^T\G_\qb(0,\hat\w_1)=\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \,\sigmahat \cdot G_t,~ G_t\sim\subg{1} \quad\text{and}\quad \sigmahat\leq \sigma\sqrt{3}\sqrt{(3/2)^4+2\left((1+1/(4\cdot 16^2))\rho^2+1/4\right)}\,.
\label{eq:finite noise exp precise}
\end{align}
\end{proof}


The next lemma controls the effect on the relevance scores of the deviation  term $\Gtilde_\qb(0,\what)=\Ghat_\qb(0,\what)-\G_\qb(0,\what).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[$\Ghat_\qb(0,\cdot)$ control: Deviation term]
    \label{lem:finite q1 deviation}Let $\Gtilde_\qb(0,\what_1):=\Ghat_\qb(0,\what_1)-\G_\qb(0,\what_1)$ and suppose $\what_1$ satisfies \eqref{eq:w1hat corr} and \eqref{eq:w1hat norm}.
    %Further assume that the step-size $\eta$ satisfies \eqref{eq:eta small deviation} small absolute constant $c_\eta>0$. 
    Fix any $u>0$ and any small constant $c_1>0$. 
    Then, there exists small enough constant $c_\eta$ (dependent on $c_1$) such that if step-size $\eta$ is small enough as per \eqref{eq:eta small deviation} the  following statements hold.

    
    First, for signal tokens, there exist positive constants $C,c',c$ such that with probability at least $1-c'e^{-cu^{2/3}}$
\begin{align}    
\abs{(\qstar+y\wstar)^T\Gtilde_\qb(0,\what_1)}\leq u\, C\,c_1\,(\wnorm^2\maxi \qnorm^2)\left(1\maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}},\,\quad y\in\{\pm1\}\label{eq:finite signal dev}
\end{align}
Second, for fresh noise variables $\z_t, t\in\Rcc$ satisfying Assumption \ref{ass:noise}, it holds that
\begin{align}
\z_t^T\G_\qb(0,\hat\w_1)\sim\subg{\sigmatilde}\quad\text{where w.p. $\geq1-c'd\,e^{-cu^{2/3}}$}\quad 
\label{eq:finite noise dev}
\sigmatilde\leq u\,\sigma\, C\,c_1\,\left(\wnorm\maxi\qnorm \maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}}\,.
\end{align}

\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
     We study each one of the terms of $\Gtilde_\qb(0,\what_1)$ in \eqref{eq:Ghat full} separately. We repeat the terms here for convenience, also noting the substitutions $\corw\leftarrow\hcorw=\what_1^T\wstar$ and $\corq\leftarrow\hcorq=\what_1^T\qstar.$
\begin{align} 
    \vb^T\Gtilde_\qb(0,\what_1)&=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\hcorw\right)\hcorq\corqv+\left((\zeta-\zeta^2)\hcorw-(\zeta^2-\zeta^3)\left(\hcorw^2+\hcorq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
\\
&\qquad+\left[\left(-\zeta+2\zeta^2\right)\hcorq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\hcorw\right)\corwv+(1-\zeta)\what_1^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\hcorw - \zeta^2(\hcorq^2+\hcorw^2)+ \frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
\\
&\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\hcorw\right)\corqv+\left(-\zeta+2\zeta^2\right)\hcorq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\what_1\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\hcorq -2 \zeta^2\hcorq\hcorw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad
+\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right) \nn
\\
&\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2y_i\right) \nn
\\
&\qquad\qquad\qquad+\left[1-2\zeta\hcorw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad+\left(1-\zeta\hcorw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\what_1 \right) \nn
\\
&\qquad\qquad\qquad- 
\zeta \hcorq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\vb^T\Sigmab\what_1\right) \nn
\\
&\qquad-\left[2\zeta\hcorq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\what_1\right) \nn
\\
&\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\what_1^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right)\right) \nn 
\\
&\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\left(\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\what_1^T\Sigmab\vb\right)\right) \,.\label{eq:Ghat full what}
\end{align}
Recall from the lemma assumption that \eqref{eq:w1hat corr} holds and from $\corw=\eta\zeta\wnorm^2$ and $\corq=\eta\zeta\rho\wnorm\qnorm$, that 
$1/2 \eta\zeta\wnorm^2\leq \hcorw\leq 3/2 \eta\zeta\wnorm^2$ and $\eta\zeta(\rho-1/2)\wnorm\qnorm\leq \abs{\hcorq}\leq \eta\zeta(\rho+1/2)\wnorm\qnorm$. The observation is that we can choose step-size $\eta$ small enough (as stated in \eqref{eq:eta small deviation}) to bound (in absolute value) all the coefficients in \eqref{eq:Ghat full what} (aka all terms in square brackets) that include  $\hcorw,\hcorq$.  Therefore, for any small positive constant $c_1>0$ it can be checked that there is sufficiently small constant $c_\eta$ that determines step-size $\eta$ in \eqref{eq:eta small deviation} such that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}    
\abs{\vb^T\Gtilde_\qb(0,\what_1)}&\leq c_1\left[\abs{\corqv}+\abs{\corwv}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i} \nn
\\
&\qquad+\left[c_1\abs{\corqv}+c_1\abs{\corwv}+(1-\zeta)\sigma^2\abs{\what_1^T\vb}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)}\nn
\\
&\qquad\qquad\qquad+\left[c_1+ \frac{(1-\zeta)}{T}\sigma^2\tn{\what_1}^2\right] \abs{\frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i} \nn
\\
&\qquad\qquad\qquad+\left[c_1\abs{\corqv}+c_1\abs{\corwv}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\what_1\right)} \nn
\\
&\qquad\qquad\qquad+\left[c_1\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)}\nn
\\
&\qquad
+\zeta\abs{\corqv} \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1} \nn
\\
&\qquad\qquad\qquad+\zeta\abs{\corwv} \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2y_i} \nn
\\
&\qquad\qquad\qquad+\left[1+c_1\right] \abs{ \frac{1}{n}\sum_{i=1}^{n}y_i\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)} \nn
\\
&\qquad+\left[1+c_1\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\what_1}\nn
\\
&\qquad\qquad\qquad + c_1\abs{\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\vb^T\Sigmab\what_1}\nn
\\
&\qquad+\left[c_1\right]\abs{ \frac{1}{n}\sum_{i=1}^{n}\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\what_1} \nn
\\
&\qquad + \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\what_1^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right)} \nn 
\\
&\qquad+\abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\left(\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\what_1^T\Sigmab\vb\right)}\,.\label{eq:Ghat full what simple}
\end{align}
Now, we use successively Lemma \ref{lem:conc_grad_q} to bound the random terms. Also note that $\abs{\corqv}\leq \qnorm\tn{\vb}$, $\abs{\corwv}\leq \wnorm\tn{\vb}$ and $\tn{\what_1}\leq (3/2) \tn{\w_1}=(3/2)\eta\zeta\wnorm.$ For any $u>0$, with  probability at least $1-c'e^{-cu^{2/3}}$ we have

\begin{align}    
&\abs{\vb^T\Gtilde_\qb(0,\what_1)}\leq u\cdot\frac{C}{\sqrt{n}}\,\tn{\vb}\,c_1\left(\wnorm+\qnorm\right) \nn
\\
&+u\cdot\frac{C\sigma\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,\left( c_1\left(2\wnorm+2\qnorm+\eta\zeta(1-\zeta)\sigma^2\wnorm\right)\eta\zeta W + \left(2c_1 + \sigma^2(1-\zeta)\eta^2\zeta^2W^2/T\right) \right) \nn
\\
% %
% &\frac{C c_1\tn{\vb}\left(\wnorm+\qnorm+\eta\zeta(1-\zeta)\sigma^2\wnorm\right) \sigma\sqrt{1-\zeta}\eta\zeta\wnorm}{\sqrt{nT}}u\nn
% +\frac{C \left(c_1 + \sigma^2(1-\zeta)\eta^2\zeta^2W^2/T\right) \sigma\sqrt{1-\zeta}\tn{\vb}}{\sqrt{nT}}u\nn
% +\frac{C  c_1 \left(\wnorm+\qnorm\right)\tn{\vb}\sigma\sqrt{1-\zeta}\eta\zeta\wnorm}{\sqrt{nT}}u\nn
% \\
% &\qquad\qquad\qquad+\frac{C c_1 \sigma\sqrt{1-\zeta} \tn{\vb}}{\sqrt{nT}}u\nn
% \\
&+u\cdot\frac{C\sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,\left(\eta^2\zeta^3\wnorm^2\qnorm + \eta^2\zeta^3\wnorm^3+(1+c_1)\eta\zeta\wnorm\right) \nn
% \\
% &
% +\frac{C (1-\zeta)\sigma^2\zeta\tn{\vb}\qnorm\eta^2\zeta^2\wnorm^2}{T\sqrt{n}}u \nn
% +\frac{C(1-\zeta)\sigma^2\zeta\tn{\vb}\wnorm\eta^2\zeta^2\wnorm^2}{T\sqrt{n}}u
%  \nn
% +
% \frac{C(1+c_1)(1-\zeta)\sigma^2\eta\zeta\wnorm\tn{\vb}}{T\sqrt{n}}u
%  \nn
\\
&+u\cdot\frac{C\sigma^2\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,\left((1+2c_1)\eta\zeta\wnorm\right)\nn
% \\
% &+\frac{C(1+c_1)\sigma^2\sqrt{1-\zeta}\eta\zeta\wnorm\tn{\vb}}{\sqrt{nT}}u\nn
% + \frac{C c_1 \sigma^2\sqrt{1-\zeta}\eta\zeta\wnorm\tn{\vb}}{\sqrt{nT}}u
\\
&+u\,\frac{C \sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,\left(c_1\eta\zeta\wnorm\right) \nn
\\
&+
u\,\frac{C\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}\,\tn{\vb}\,\left( \eta^2\zeta^2\wnorm^2\right)
 \nn 
\\
&+
u\,\frac{C\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}\,\tn{\vb}\,\eta^2\zeta^2\wnorm^2
\,.\label{eq:Ghat full what simple with concentration}
\end{align}

Now, again  using small step size $\eta$ as per \eqref{eq:eta small deviation}, this can be further simplified to the following (here the value of constant $c_1$ might be different from \eqref{eq:Ghat full what simple with concentration})
\begin{align}    
\abs{\vb^T\Gtilde_\qb(0,\what_1)}&\leq u\cdot\frac{C}{\sqrt{n}}\,\tn{\vb}\,c_1\left(\wnorm+\qnorm\right)
+u\cdot\frac{C\sigma\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,c_1\left(1+\wnorm+\qnorm\right) \nn
+u\cdot\frac{C\sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,c_1 \nn
\\
&\quad+u\cdot\frac{C\sigma^2\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,c_1
+
u\,\frac{C\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}\,\tn{\vb}\,c_1
 \nn 
+
u\,\frac{C\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}\,\tn{\vb}\,c_1
\,
\\
&\leq u\cdot\tn{\vb}\cdot \frac{C}{\sqrt{n}} \cdot c_1 \left(\wnorm\maxi\qnorm\maxi\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^2}{T}\maxi\frac{\sigma^3\log(n)}{T^{3/2}}\maxi\frac{\sigma^3\log(n)}{T}\right) \nn
\\
&\leq u\cdot\tn{\vb}\cdot \frac{C\,\log(n)}{\sqrt{n}} \cdot c_1 \left(\wnorm\maxi\qnorm\maxi\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right) \label{eq:Ghat full what simple with concentration very simple to use}
\end{align}

%.\label{eq:Ghat full what simple with concentration very simple}
% \begin{align}    
% \frac{\abs{\vb^T\Gtilde_\qb(0,\what_1)}}{\tn{\vb}}&\leq \frac{C c_1\left(\wnorm+\qnorm\right)}{\sqrt{n}}u \nn
% +\frac{C c_1\sigma\sqrt{1-\zeta}}{\sqrt{nT}}u\nn
% +\frac{C c_1 (1-\zeta)\sigma^2\zeta}{T\sqrt{n}}u \nn
% + \frac{C c_1 \sigma\sqrt{1-\zeta}}{\sqrt{nT}}u
% \\
% &\qquad\qquad\qquad\qquad+
% \frac{Cc_1\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}u
% +
% \frac{Cc_1\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}u
% \\
% &\leq \frac{Cc_1(\wnorm+\qnorm)\poly{\sigma}\log(n)}{\sqrt{n}}u
% \,.\label{eq:Gtilde full what simple with concentration}
% \end{align}


Now, we can compute the deviation of the relevance scores. For signal tokens we have for both $y\in\{\pm1\}$, and all $u>0$ with probability at least $1-c'e^{-cu^{2/3}}$, there exist constant $C>0$ such that
\begin{align}    
\abs{(\qstar+y\wstar)^T\Gtilde_\qb(0,\what_1)}\leq u\, C(\wnorm^2\maxi \qnorm^2)\left(1\maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}} \label{eq:finite signal dev 2}
\end{align}

For a noisy token $\z_t,t\in\Rcc$ note that $ \z_t^T\Gtilde_\qb(0,\what_1)\sim\subg{\sigma\tn{\Gtilde_\qb(0,\what_1)}}$. We can bound $\tn{\Gtilde_\qb(0,\what_1)}$ applying \eqref{eq:Ghat full what simple with concentration very simple to use} for all standard basis vectors $\vb=\eb_j, j\in[n]$ and union bounding. This gives for all $u>0$ with probability at least $1-c'de^{-cu^{2/3}},$
\[
\tn{\Gtilde_\qb(0,\what_1)}\leq u\, C\left(\wnorm\maxi\qnorm \maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}}\,.
\]

% for all $t\in\Rcc$ and all $u>0$ with probability at least $1-c'de^{-cu^{2/3}},$
% \begin{align}
%     \z_t^T\Gtilde_\qb(0,\what_1)\sim \subg{\sigmatilde}\qquad \sigmatilde\leq Cc_1(\wnorm+\qnorm)\sigma\poly{\sigma}\frac{\log(n)}{\sqrt{n}}u
%     \label{eq:finite noise dev}
% \end{align}
% where to bound $\tn{\Gtilde_\qb(0,\what_1)}$, we applied union bound.
\end{proof}

With lemmas \ref{lem:finite q1 expectation} and \ref{lem:finite q1 deviation} at hand, we are now ready to put things together stating our final bounds for relevance scores. The finding is presented as a stand-alone lemma below.
\begin{lemma}[Put things together]\label{putogether1}
    Consider the finite-sample gradient step
    $\qhat_1=\Ghat_\qb(0,\what_1)$, where recall that $\what_1=\eta\Ghat_\w(0,0).$
    Fix any $u_0,u_1,u_2,u_3>0$ and any small constant $\wt{c}_1>0$.
    Suppose step-size $\eta$ of first gradient step satisfies \eqref{eq:eta small deviation} for sufficiently small constant $c_\eta>0$ (dependent on $\wt{c}_1$) and further assume
\begin{align}
    \sqrt{n}&\geq u_0\cdot C_0  \frac{\qnorm}{\wnorm}
    \qquad\text{and}\qquad
    \sqrt{\frac{n\zeta T}{d}}\geq   u_0 \cdot C_0  \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}.
\end{align}
for some large enough  constant $C_0>0$. Finally, assume for simplicity that
\begin{align}\label{eq:strignent for convenience}
\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T} \leq \wnorm\maxi\qnorm 
\end{align}
Consider a fresh dataset $(\X_i,y_i)_{i\in[n]}$ and consider the signal and noise relevance scores $\rhat_{i,t}:=r_{i,0}:=\left(\qstar+y_i\wstar\right)^T\qhat_1, t\in\Rc$ and $\rhat_{i,t}:=\z_{i,t}^T\qhat_1, t\in\Rcc$, respectively.  
Then, there exist positive absolute constants $C,c_i,c_i',i=0,1,2,3$ such that the following statements hold
\begin{itemize}
    \item With probability at least $1-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}},$ the signal relevance scores satisfy
    \begin{align}
    \label{eqcomb1}
        \min_{i\in[n]} r_{i,0} \geq  \eta\zeta
        (\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(15-8\rho^2-6\abs{\rho}\right)\qnorm - \left(210\abs{\rho}+33\right)\wnorm \right)/64
        %(\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(8-6\rho^2-\abs{\rho}\right)\qnorm - 121\abs{\rho}\wnorm \right)/32\ 
        - 
        u_1\, C\,\wt{c}_1\,(\wnorm^2\maxi \qnorm^2)\frac{\log(n)}{\sqrt{n}}=:B(u_1)
        %u_1 \cdot C_1(\wnorm+\qnorm)^2\poly{\sigma}\log(n) /\sqrt{n}
    \end{align}
    \item With probability at least $1-c_0'e^{-c_0u_0^2}-c_2'n(1-\zeta)Te^{-c_2u_2^2}-c_3'dn(1-\zeta)Te^{c_3u_3^{2/3}},$ the noise relevance scores satisfy
    \begin{align}
    \label{eqcomb2}
        \max_{i\in[n],t\in\Rcc}r_{i,t} \leq  u_2\,\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \,\sigma\,C  + u_3\,\sigma\, C\,\wt{c}_1\,\left(\wnorm\maxi\qnorm \right)\frac{\log(n)}{\sqrt{n}}=:M(u_2,u_3)
    \end{align}
\end{itemize}

\end{lemma}
\begin{proof} The lemma follows by collecting \eqref{eq:finite signal exp}, \eqref{eq:finite signal dev}, \eqref{eq:finite noise exp}, \eqref{eq:finite noise dev}, and applying union bound for the noise terms over $i\in[n],t\in\Rcc$.
%we arrive at the following. There exist absolute constants $C,C_1,C_2$ such that the following hold for all $u>0$ with probability at least $1-c'e^{-cu^{2/3}}$:
% \begin{align}
%         r_{i,0} \geq  \eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(8-6\rho^2-\abs{\rho}\right)\qnorm - 121\abs{\rho}\wnorm \right)/32\ - 
%         u_1\, C\,c_1\,(\wnorm^2\maxi \qnorm^2)\frac{\log(n)}{\sqrt{n}}
% \end{align}
% and \eqref{eqcomb1} follows because $\eta$ is small enough as per \eqref{eq:eta small deviation}. Also,
%  with probability at least $1-c'dn(1-\zeta)Te^{-cu^{2/3}}$:
% \begin{align}
% \max_{i\in[n],t\in\Rcc}\z_{i,t}^T\Ghat_\qb(0,\what_1) \leq 
% u_2\,\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \,\sigma\,C
% + C_2(\wnorm+\qnorm)\sigma\poly{\sigma}\log(n) u /\sqrt{n}
% \end{align}
% % Thus, with 
\end{proof}

==> gradient_analysis_backup_March2023.tex <==
\section{Proofs for finite-sample Gradient Analysis in Section \ref{sec:finite analysis}}\label{sec:proofs grad finite}




% \subsection{Finite-sample Analysis}
In this section, we focus on finite-sample analysis of Algorithm \ref{eq:algo}. Introduce the following shorthand notation analogous to the population counterparts in Section \ref{sec:population analysis main}:
\begin{align}
&\widehat\G_\qb(\qb,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) = \frac{1}{n}\sum_{i\in[n]} (y_i-f_{\thetab}(\X_i)) \X_i^\top\sftd{\X_i\qb}\,\X_i \w \nn
\\
&\widehat\G_\w(\qb,\w):=-\nabla_{\w}\Lch_{\Dc}(\thetab) = \frac{1}{n}\sum_{i\in[n]} (y_i-f_{\thetab}(\X_i)) \X_i^\top\sft{(\X_i\qb)} .
\end{align}


\subsection{Gradient Calculations}
We begin with the gradient calculations for the first two steps of the algorithm.

For convenience, we make use of the following shorthands
\begin{subequations}\label{eq:gradient_term_notations}
\begin{align*}
\corq&:=\corqarg{\w}:=\w^\top\qb_\star,
\qquad\corw:=\corwarg{\w}:=\w^\top\w_\star,\qquad\alpha_i:=\alpha(\w,y_i):=\corq+y_i\corw, \\
\gammab_i&:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\qquad
\beta_i:=\beta(\Z_i;\w)=\gammab_i^T\w, \qquad
\hat\Sigmab_i:=\frac{1}{T}\Z_i^T\Z_i.
\end{align*}
\end{subequations}
for $\Z_i\in\R^{(1-\zeta)T \times d}$ is the matrix of irrelevant tokens $\zti, t\in\Rcc$ for sample $i\in[n].$

\begin{lemma}\label{lem:w_der_finite}
 Under dataset model \eqref{eq:CGMM} and Assumption \ref{ass:noise}, we have
\begin{align}
\Ghat_\w(0,0)
&=  \zeta \w_\star + \zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ \frac{1}{n}\sum_{i}y_i\gammab_i.
\end{align}
% where $\hat{Y}:=\frac{1}{n}\sum_{i\in[n]}y_i$ and $\Z_{i}\in\R^{(1-\zeta)T\times d}$ is the matrix of noisy tokens for sample $i\in[n]$. 
% That is, 
% \begin{align}
% \Ghat_\w(0,0)\,|\,\y\sim \subg{ \zeta \hat{Y} \qb_\star + \zeta \w_\star, \sigma^2(1-\zeta)\Iden}.
%\end{align}
\end{lemma}



\begin{lemma}\label{lem:q_der_finite} Under dataset model \eqref{eq:CGMM} and Assumption \ref{ass:noise}, we have that
%for $\w=\mu\w_\star+\tau\qb_\star+\etab$, $\etab\sim\subg{\alpha^2\Id}$, we have that 
\begin{align}\label{eq:q_der_finite}
\Ghat_\qb(0,\w):=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)\left(\qstar + y_i\wstar\right)
+ \hat\Sigmab_i\w
- (\zeta\alpha_i+\beta_i)\gammab_i
\right]\,.
\end{align}
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:w_der_finite}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By direct computation,
\begin{align}
\hat\G_\w(0,0):=-\nabla_{\w}\Lch_{\Dc}(\thetab) 
&= \frac{1}{nT}\sum_{i\in[n]}y_i\X_i^T\ones_T = \frac{1}{nT}\sum_{i\in[n]}\sum_{t\in[T]}y_i\x_{i,t} \nn
\\
&=\frac{1}{n}\big(\sum_{i\in[n]}\zeta_iy_i\big) \qb_\star
+\frac{1}{n}\big(\sum_{i\in[n]}\zeta_i\big) \w_\star
+\frac{1}{n}\sum_{i\in[n]}y_i \zai \nn
\end{align}
where $\zeta_i$ is the fraction of relevant tokens in the $i$-th sample and $\zai=\frac{1}{T}\sum_{t=1}^{T}\z_{i,t}$ where we again set noise $\z_t=0$ for relevant tokens. %The desired follows by recognizing that $y_i\z_{i,t}\sim\subg{\sigma^2\Id}$ for irrelevant tokens and using simplifying Assumption \ref{ass:zeta}.


% \subsection{Proof of New Lemma 4}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recall that $\phi^\prime(Xq)=\text{diag}\left(\phi'(\X\qb)\right)-\phi'(\X\qb)\phi'(\X\qb)^T$; hence, for $\thetab=(\qb,\w)$:
% \begin{align*} 
% \hat\G_\qb(\qb,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) 
% &= \frac{1}{n}\sum_{i\in[n]} \underbrace{(y_i-f_{\thetab}(\X_i)) \X_i^\top\text{diag}\left(\phi'(\X_i\qb)\right)\X_i\w}_{\term{1,i}} \\
% &\quad\quad- \frac{1}{n}\sum_{i\in[n]} \underbrace{{(y_i-f_{\thetab}(\X_i)) \X_i^\top\phi'(\X_i\qb)\phi'(\X_i\qb)^T\X_i \w}}_{\term{2,i}}.
% \end{align*}
% Moreover, note that, 
% \begin{align}
% f_{\thetab}(\X_i)&=\w^T\X_i^T\phi\left(\X_i\qb\right), \nn \\
% \X_i^\top\X_i &= \zeta T(\qb_\star + y_i \w_\star) (\qb_\star + y \w_\star)^\top + \Z_i^\top\Z_i,\nn\\
% \X_i^\top\ones &= \zeta T (\qb_\star + y_i \w_\star) + \Z_i^\top\ones.\nn
% \end{align}
% where recall the notation in Lemma \ref{lem:w_der_finite} for $\Z_i.$ Hence, using the lemma's notation (repeated here for convenience)
% \begin{align*}
% \alpha_i&:=\corq+y_i\corw, \\
% \beta_i&:=\beta(\Z_i;\w):=\frac{1}{T}\ones^T\Z_i\w, \\
% \gammab_i&:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\\
% \hat\Sigmab_i&:=\frac{1}{T}\Z_i^T\Z_i.
% \end{align*}
% we find that
% \begin{align}
% y_i-f_{\thetab}(\X_i) &= y_i - \zeta \alpha_i-\beta_i
% \\
% \frac{1}{T}\X_i\X_i^\top\w&=\zeta \alpha_i\qstar + \zeta y_i \alpha_i \wstar+\hat\Sigmab_i\w
% \\
% \frac{1}{T^2}{\X_i^\top\ones\ones^\top\X_i\w}&=\zeta\left(\zeta  \alpha_i+\beta_i\right) \qstar + \zeta\left(\zeta  \alpha_i+\beta_i\right) y_i \wstar 
% +\left(\zeta  \alpha_i+\beta_i\right)\gammab_i.
% \end{align}


% With the above, each one of the two terms becomes:

% \begin{align}
% \term{1,i}= \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta \alpha_i \qstar + 
% \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta  \alpha_i y_i \wstar + \left(y_i - \zeta \alpha_i-\beta_i\right)\hat\Sigmab_i\w
% \end{align}

% \begin{align}
% \term{2,i}= \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\qstar + 
% \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right) y_i\wstar + \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\gammab_i
% \end{align}

% Combining the above:

% \begin{align}
% {\term{1,i}-\term{2,i}}=\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
% \zeta\left((1-\zeta)\alpha_i-\beta_i\right)\left(\qstar + y_i\wstar\right)
% + \hat\Sigmab_i\w
% - (\zeta\alpha_i+\beta_i)\gammab_i
% \right]
% \end{align}


%\subsubsection{Remarks}

% \begin{remark}
% Lemma \ref{lem:q_der_pop} follows by Lemma \ref{lem:q_der_finite} by choosing $\w=\alpha\wstar$ and letting $n\rightarrow\infty$. To see this note that for this choise of $\w$, $\alpha_i=y_i\alpha\|\wstar\|^2$. Hence, recalling the shorthand $B:=\alpha\|\wstar\|^2$ the $\qstar$ direction in \eqref{eq:q_der_finite} is
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B)-\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \qstar
% \end{align*}
% Let $n\rightarrow\infty$ and apply law of large numbers with recalling that $$\E[y]=0, ~~\E[y\beta]=0,~~ \E[y^2]=1 ~~\text{and}~~ \E[\beta^2]=\frac{1}{T^2}\alpha^2\E[(\wstar^T\Z_i^T\ones)^2]=\frac{\alpha\sigma^2(1-\zeta)B}{T}.$$ This evaluates the coefficient of $\qstar$ above to:
% \begin{align}
% (1-\zeta B) (\zeta-\zeta^2) B +\frac{\alpha\sigma^2(\zeta-\zeta^2)B}{T} = \left[ \left(\zeta-\zeta^2\right)(1+\alpha\sigma^2/T)-\left(\zeta^2-\zeta^3\right)B \right] B.
% \end{align}

% Similarly, it can be shown that the $\wstar$ direction in \eqref{eq:q_der_finite}, i.e.
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left((1 - \zeta B)-y_i\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \wstar
% \end{align*}
% is zero. This is because $\E[y]=0$, $\E[\beta]=0$ and $y,\beta$ are independent.

% Next, take the $\hat\Sigmab_i\w$ direction:
% \begin{align}\label{eq:q_der_finite}
% \frac{\alpha}{n}\sum_{i=1}^{n}\left(y_i (1- \zeta B)-\beta_i\right)  \hat\Sigmab_i\w_\star
% \end{align}
% The first term is asymptotically zero by independence of $y_i,\hat\Sigmab_i$ and by $\E[y]=0$. The second term involves
% $$
% \E\left[(\w_\star^T\Z^T\ones)\Z^T\Z\w_\star\right]=0
% $$
% which is zero by assumption on third moments of $\Z$ being zero.

% Finally, consider the $\gammab_i$ direction:
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B) - \beta_i\right) 
% (\zeta y_i B+\beta_i)\gammab_i 
% \end{align*}
% The only term that survives zero-mean assumption of $y$, zero mean of $\gammab$ and independence of $y,\gammab_i$ is the term:
% $$
% \E\left[\beta^2\gammab\right] = \frac{1}{T^3}\E\left[\left(\w_\star^T\Z^T\ones\right)^2\Z^T\ones\right],
% $$
% which is again zero because of third moment of $\Z$ being zero.

% \end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:q_der_finite}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recall that $\phi^\prime(0)=\frac{1}{T}\Id-\frac{1}{T^2}\ones\ones^T$; hence, for $\thetab=(0,\w)$:
\begin{align*} 
\hat\G_\qb(0,\w):=-\nabla_{\qb}\Lch_{\Dc}(\thetab) 
&= \frac{1}{n}\sum_{i\in[n]} \underbrace{\frac{1}{T}(y_i-f_{\thetab}(\X_i)) \X_i^\top\X_i\w}_{\term{1,i}} - \frac{1}{n}\sum_{i\in[n]} \underbrace{{\frac{1}{T^2}(y_i-f_{\thetab}(\X_i)) \X_i^\top\ones\ones^\top\X_i \w}}_{\term{2,i}}.
\end{align*}
Moreover, note that, 
\begin{align}
f_{\thetab}(\X_i)&=\frac{1}{T}\w^T\X_i^T\ones, \nn \\
\X_i^\top\X_i &= \zeta T(\qb_\star + y_i \w_\star) (\qb_\star + y_i \w_\star)^\top + \Z_i^\top\Z_i,\nn\\
\X_i^\top\ones &= \zeta T (\qb_\star + y_i \w_\star) + \Z_i^\top\ones.\nn
\end{align}
where recall the notation in Lemma \ref{lem:w_der_finite} for $\Z_i.$ Hence, using the lemma's notation (repeated here for convenience)
\begin{align*}
\alpha_i&:=\corq+y_i\corw, \quad
\beta_i:=\beta(\Z_i;\w):=\frac{1}{T}\ones^T\Z_i\w, \quad
\gammab_i:=\gammab(\Z_i)=\frac{1}{T}\Z_i^T\ones,\quad
\hat\Sigmab_i:=\frac{1}{T}\Z_i^T\Z_i.
\end{align*}
we find that
\begin{align}
y_i-f_{\thetab}(\X_i) &= y_i - \zeta \alpha_i-\beta_i
\\
\frac{1}{T}\X_i\X_i^\top\w&=\zeta \alpha_i\qstar + \zeta y_i \alpha_i \wstar+\hat\Sigmab_i\w
\\
\frac{1}{T^2}{\X_i^\top\ones\ones^\top\X_i\w}&=\zeta\left(\zeta  \alpha_i+\beta_i\right) \qstar + \zeta\left(\zeta  \alpha_i+\beta_i\right) y_i \wstar 
+\left(\zeta  \alpha_i+\beta_i\right)\gammab_i.
\end{align}


With the above, each one of the two terms becomes:

\begin{align}
\term{1,i}= \left(y_i - \zeta \alpha_i-\beta_i\right)\zeta \alpha_i \qstar + 
\left(y_i - \zeta \alpha_i-\beta_i\right)\zeta  \alpha_i y_i \wstar + \left(y_i - \zeta \alpha_i-\beta_i\right)\hat\Sigmab_i\w
\end{align}

\begin{align}
\term{2,i}= \zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\qstar + 
\zeta \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right) y_i\wstar + \left(y_i - \zeta \alpha_i-\beta_i\right) \left(\zeta\alpha_i+\beta_i\right)\gammab_i
\end{align}

Combining the above:

\begin{align}
{\term{1,i}-\term{2,i}}=\left(y_i - \zeta \alpha_i-\beta_i\right) \left[
\zeta\left((1-\zeta)\alpha_i-\beta_i\right)\left(\qstar + y_i\wstar\right)
+ \hat\Sigmab_i\w
- (\zeta\alpha_i+\beta_i)\gammab_i
\right]
\end{align}


%\subsubsection{Remarks}

% \begin{remark}
% Lemma \ref{lem:q_der_pop} follows by Lemma \ref{lem:q_der_finite} by choosing $\w=\alpha\wstar$ and letting $n\rightarrow\infty$. To see this note that for this choise of $\w$, $\alpha_i=y_i\alpha\|\wstar\|^2$. Hence, recalling the shorthand $B:=\alpha\|\wstar\|^2$ the $\qstar$ direction in \eqref{eq:q_der_finite} is
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B)-\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \qstar
% \end{align*}
% Let $n\rightarrow\infty$ and apply law of large numbers with recalling that $$\E[y]=0, ~~\E[y\beta]=0,~~ \E[y^2]=1 ~~\text{and}~~ \E[\beta^2]=\frac{1}{T^2}\alpha^2\E[(\wstar^T\Z_i^T\ones)^2]=\frac{\alpha\sigma^2(1-\zeta)B}{T}.$$ This evaluates the coefficient of $\qstar$ above to:
% \begin{align}
% (1-\zeta B) (\zeta-\zeta^2) B +\frac{\alpha\sigma^2(\zeta-\zeta^2)B}{T} = \left[ \left(\zeta-\zeta^2\right)(1+\alpha\sigma^2/T)-\left(\zeta^2-\zeta^3\right)B \right] B.
% \end{align}

% Similarly, it can be shown that the $\wstar$ direction in \eqref{eq:q_der_finite}, i.e.
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left((1 - \zeta B)-y_i\beta_i\right)
% \left((\zeta-\zeta^2)y_iB-\zeta\beta_i\right)
% \wstar
% \end{align*}
% is zero. This is because $\E[y]=0$, $\E[\beta]=0$ and $y,\beta$ are independent.

% Next, take the $\hat\Sigmab_i\w$ direction:
% \begin{align}\label{eq:q_der_finite}
% \frac{\alpha}{n}\sum_{i=1}^{n}\left(y_i (1- \zeta B)-\beta_i\right)  \hat\Sigmab_i\w_\star
% \end{align}
% The first term is asymptotically zero by independence of $y_i,\hat\Sigmab_i$ and by $\E[y]=0$. The second term involves
% $$
% \E\left[(\w_\star^T\Z^T\ones)\Z^T\Z\w_\star\right]=0
% $$
% which is zero by assumption on third moments of $\Z$ being zero.

% Finally, consider the $\gammab_i$ direction:
% \begin{align*}
% \frac{1}{n}\sum_{i=1}^{n}\left(y_i (1 - \zeta B) - \beta_i\right) 
% (\zeta y_i B+\beta_i)\gammab_i 
% \end{align*}
% The only term that survives zero-mean assumption of $y$, zero mean of $\gammab$ and independence of $y,\gammab_i$ is the term:
% $$
% \E\left[\beta^2\gammab\right] = \frac{1}{T^3}\E\left[\left(\w_\star^T\Z^T\ones\right)^2\Z^T\ones\right],
% $$
% which is again zero because of third moment of $\Z$ being zero.

% \end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Concentration of Gradient \texorpdfstring{$\Ghat_\qb{(0,\w)}$}{} in the \texorpdfstring{$\qb$}{context} direction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main result of this section is the following lemma about concentration of gradient with respect to $\qb$.

\begin{lemma}[Concentration of $\Ghat_\qb(0,\w)$]\label{lem:conc_grad_q}
Fix any vectors $\vb,\w\in\R^d$. For convenience define $\corqv:=\vb^T\qstar$ and $\corwv:=\vb^T\wstar$ and recall $\corw,\corq$ notations from Lemma \ref{lem:q_der_finite}. Then, we can decompose
\[
\vb^T\Ghat_\qb(0,\w) =\vb^T\G_\qb(0,\w) + \vb^T\Gtilde_\qb(0,\w),
\]
where the expectation term is given by 
    \begin{align}
\vb^T\G_\qb(0,\w):=\E\left[\vb^T\Ghat_\qb(0,\w)\right] 
&= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
\\ 
&
+\left(\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \right)\,\corqw -\left(\left(1+{2}/{T}\right)(\zeta-\zeta^2)\corq\right)\vb^T\Sigmab\w
\label{eq:mean_one_step_grad_q}
\end{align}
and the deviation term obeys
\begin{align}
\vb^T\Gtilde_\qb(0,\w) 
&=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
\\
&\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
\\
&\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad
+\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
\\
&\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
\\
&\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
\\
&\qquad\qquad\qquad- 
\zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
\\
&\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
\\
&\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
\\
&\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right).\label{eq:Ghat full}
\end{align}
Moreover, all random terms in \eqref{eq:Ghat full} are zero-mean and concentrate as prescribed by
Lemma \ref{lem:psi} below
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Main concentration lemma]\label{lem:psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $y_i, i\in[n]$ be iid Rademacher random variables. Let $\Z_i\in\R^{(1-\zeta)T \times d}, i\in[n]$ be iid copies of a random matrix $\Z$. Each row  $\z_t, t\in[(1-\zeta)T]$ of $\Z$ is an iid copy of a random vector $\z$ satisfying Assumption \ref{ass:noise}. For convenience denote $\gammab_i:=\Z_i^T\ones/T$ and $\hat\Sigmab_i:=\Z_i^T\Z_i/T$. Then, the following statements are true for all vectors $\w,\vb\in\R^{d}$.
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}y_i}{2}&\leq \frac{C}{\sqrt{n}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\gammab_i^T\w}{2} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\gammab_i^T\w}{2} &\leq \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2}{\sqrt{nT}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right) - \frac{1-\zeta}{T}\vb^T\Sigmab\w}{1} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)}{1} &\leq \frac{C\sigma^2(1-\zeta)\|\w\|_2\|\vb\|_2}{T\sqrt{n}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\w^T\hat\Sigmab_i\vb-{(1-\zeta)}\w^T\Sigmab\vb}{1} \vee \psinorm{\frac{1}{n}\sum_{i\in[n]}y_i\w^T\hat\Sigmab_i\vb  }{1}&\leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}}
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\left(\gammab_i^T\w\right)^2-\frac{1-\zeta}{T}{\w^T\Sigmab\w}\right)\gammab_i^T\vb}{2/3}&\leq \frac{C\sigma^3(1-\zeta)^{3/2}\|\w\|_2^2\|\vb\|_2}{T^{3/2}\sqrt{n}}\log n
\end{align*}
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i\in[n]}\left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3} &\leq \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T\sqrt{n}}}\log n
\end{align*}
Also, all the random variables that appear above are zero mean.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsubsection{Proof of Lemma \ref{lem:conc_grad_q}}

We split \eqref{eq:q_der_finite} in four terms and handle each of them separately.

\noindent\textbf{$\bullet$~~ $\term{I}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)\qstar$}\\
We first focus on
\begin{align*}
\term{I}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i(1-\zeta\corw) -\beta_i- \zeta \corq\right) 
\left(y_i(\zeta-\zeta^2)\corw-\zeta\beta_i+(\zeta-\zeta^2)\corq\right)\qstar=:A\qstar.
\end{align*}
We we can express $A$ above conveniently as follows (recall $y_i^2=1$):
\begin{align*}
A&:=-\zeta(\zeta-\zeta^2)\corq^2+(1-\zeta\corw)(\zeta-\zeta^2)\corw +\left((1-\zeta\corw)(\zeta-\zeta^2)\corq-\zeta(\zeta-\zeta^2)\corw\corq\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right)
\\
&\qquad\qquad+\left(-(\zeta-\zeta^2)\corq+\zeta^2\corq\right)\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\left(-(1-\zeta\corw)\zeta-(\zeta-\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\beta_i\right)
+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2\right)
\\
&=(\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right)
\\
&\qquad\qquad+\left(-\zeta+2\zeta^2\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\beta_i\right)
\\
&\qquad\qquad+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)+\frac{(\zeta-\zeta^2)}{T}\w^T\Sigmab\w.
\end{align*}
From Lemma \ref{lem:psi}, all random terms above are zero mean. Hence,
\begin{align}
\E[A]&=-(\zeta^2-\zeta^3)\corq^2+(1-\zeta\corw)(\zeta-\zeta^2)\corw+(\zeta-\zeta^2)\frac{\w^T\Sigmab\w}{T} \nn
\\
&=-(\zeta^2-\zeta^3)\corq^2+(\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\corw^2 \nn
\\
&=(\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right).\label{eq:Exp_term1}
\end{align}
%We will show that for all $0<t<\sqrt{n}$:
%\begin{align}
%\Pr\left(|A-\E[A]|\leq \frac{C\sigma\|\w\|_2 t}{\sqrt{n}} \right)\geq 1-2e^{-t^2}.
%\end{align}
%Indeed, 


\vp
\noindent\textbf{$\bullet$~~$\term{II}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
\left((\zeta-\zeta^2)\alpha_i-\zeta\beta_i\right)y_i\wstar$}\\
\begin{align*}
\term{II}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i(1-\zeta\corw) -\beta_i- \zeta \corq\right) 
\left(y_i(\zeta-\zeta^2)\corw-\zeta\beta_i+(\zeta-\zeta^2)\corq\right)y_i\wstar=B\wstar.
\end{align*}
We we can express $B$ above conveniently as:
\begin{align*}
B&:=\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\left(\frac{1}{n}\sum_{i\in[n]}y_i\right)  +\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq
\\
&\qquad\qquad+\left(-\zeta+2\zeta^2\right)\corq\left(\frac{1}{n}\sum_{i=1}^{n}\beta_iy_i\right)
+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}\beta_i\right)
+\zeta \left(\frac{1}{n}\sum_{i=1}^{n}\beta_i^2y_i\right).
\end{align*}
%where we also used that $y_i^2=1$.
All the random terms above are zero-mean. Hence,
\begin{align}
\E[B]&=\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\,.
\label{eq:Exp_term2}
\end{align}


% Clearly this is a zero-mean random variable since $\beta_i,y_i$ are independent and $\E[y_i]=0$. Further note that 
% \begin{align}
% \beta_i^2y_i = (1-\zeta)^2\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}y_i\z_{t,i}^T\w\right)\widesim{D} (1-\zeta)^2\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\wt\z_{t,i}^T\w\right),
% \end{align} 
% where $\wt\z_{i,t}\widesim{D}\z_{i,t}$ and $\wt\z_{i,t}$ are independent for all $t$. Hence,
% \begin{align}
% \|\beta_i^2y_i\|_{\psi_1}\leq (1-\zeta)^2\|\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\z_{t,i}^T\w\right)\|_{\psi_2}\|\left(\frac{1}{\wt T}\sum_{t=1}^{\wt T}\wt\z_{t,i}^T\w\right)\|_{\psi_2}\leq C(1-\zeta) K^2\|\w\|_2^2/T
% \end{align}
% Thus,
% \begin{align}
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\beta_i^2\big| \leq  \frac{C\sigma^2(1-\zeta)\|\w\|_2^2}{T\sqrt{n}} t
% \right)&\geq 1-2{e^{-c\min\{{t^2,t\sqrt{n}}\}}}
% \end{align}

\vp
\noindent\textbf{$\bullet$~~ $\term{III}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right) 
 \hat\Sigmab_i\w$}\\

Fix any vector $\vb:$

\begin{align*}
\vb^T\{\term{III}\} &= \left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) - \zeta \left(\corq+y_i\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w\right)-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\vb^T\hat\Sigmab_i\w\right)\\
&= \left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) - \zeta \corq\left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w\right)-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\vb^T\hat\Sigmab_i\w\right)
\\
&= \left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w\right) 
-
\zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right)-
 (\zeta-\zeta^2)\corq \vb^T\Sigmab\w
\\ &\qquad\qquad-
\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)+(1-\zeta)(\w^T\Sigmab\vb)\frac{1}{n}\sum_{i=1}^{n}(\gammab_i^T\w)
\end{align*}

From Lemma \ref{lem:psi} all random terms above are zero mean. Hence,
\begin{align}
\E\left[\vb^T\{\term{III}\}\right] = -(\zeta-\zeta^2)\corq \w^T\Sigmab\vb .\label{eq:Exp_term3}
%- (1-\zeta)\w^T\Sigmab\vb 
\end{align}
Moreover, from Lemma \ref{lem:psi} we have the following:

%\ct{We need a reference for the penultimate inequality in the above display: How it follows from last statement of Lemma \ref{lem:psi}}

\vp
\noindent\textbf{$\bullet$~~ $\term{IV}=\frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)\gammab_i$}\\

For fixed vector $\vb$, $
    \vb^T\{\term{IV}\} = \frac{1}{n}\sum_{i=1}^{n}\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)\vb^T\gammab_i.
$
Reorganizing, note that
\begin{align*}
\left(y_i - \zeta \alpha_i-\beta_i\right)  (\zeta\alpha_i+\beta_i)  &= \zeta y_i (\corq+y_i\corw) - \zeta^2(\corq^2+\corw^2+2y_i\corq\corw)-2\zeta\corq\beta_i-2\zeta\corw y_i\beta_i+y_i\beta_i-\beta_i^2\\
&= \left(\zeta\corq -2 \zeta^2\corq\corw\right) y_i + \left(\zeta\corw - \zeta^2(\corq^2+\corw^2)\right) -\left(2\zeta\corq\right)\beta_i+\left(1-2\zeta\corw\right) y_i\beta_i-\beta_i^2
\end{align*}

Overall,
\begin{align*}
    \vb^T\{\term{IV}\} &=\left(\zeta\corw - \zeta^2(\corq^2+\corw^2)\right) \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right)+\left(\zeta\corq -2 \zeta^2\corq\corw\right)\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right)
    \\
    &+\left(1-2\zeta\corw\right) \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right)
    \\
    &-\left(2\zeta\corq\right)\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right)-\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
    \\
    &- \frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)
+\frac{(1-\zeta)}{T}\w^T\Sigmab\w \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\right)
\end{align*}
According to Lemma \ref{lem:psi} all random terms above are zero mean. Thus,
\begin{align}
\E\left[\vb^T\{\term{IV}\}\right] &= -2\zeta\corq\frac{1-\zeta}{T}\w^T\Sigmab\vb
\label{eq:Exp_term4}
\end{align}


\vp
\noindent\textbf{$\bullet$~~ Combined} \\
The desired identities \eqref{eq:mean_one_step_grad_q} and \eqref{eq:Ghat full} follow by combining all the terms above. 


% We now combine all the above. For convenience define $\corqv:=\vb^T\qstar$ and $\corwv:=\vb^T\wstar$. Then, we have shown:
% \[
% \vb^T\Ghat_\qb(0,\w) =\vb^T\G_\qb(0,\w) + \vb^T\Gtilde_\qb(0,\w),
% \]
% where
% \begin{align}
%     \vb^T\G_\qb(0,\w) 
% &:=\E\left[\vb^T\Ghat_\qb(0,\w)\right] \nn \\
% &=\Big[\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corqv + \left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corwv  \nn
% \\&\qquad\qquad+{(\zeta-\zeta^2)\corqv}\left(\w^T\Sigmab\w/T\right)
% -(\zeta-\zeta^2)\corq \vb^T\Sigmab\w
% -\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
% \Big] \nn
% \\
% &= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
% \\&\qquad\qquad+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \,\corwv-(\zeta-\zeta^2)\corq \w^T\Sigmab\vb -2\zeta\corq\frac{1-\zeta}{T}\w^T\Sigmab\vb\nn
% \\
% &= \left((\zeta-\zeta^2)\left(\corw+{\w^T\Sigmab\w}/{T}\right)-(\zeta^2-\zeta^3)\left(\corw^2 + \corq^2\right)\right)\,\corqv\nn
% \\ 
% &\qquad\qquad 
% +\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq \,\corwv
%  -\left(1+\frac{2}{T}\right)(\zeta-\zeta^2)\corq\vb^T\Sigmab\w
%  \label{eq:gradient_mesh}
% \end{align}

% and 
% \begin{align}
% \vb^T\Gtilde_\qb(0,\w) 
% &=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
% \\
% &\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad
% +\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
% \\
% &\qquad\qquad\qquad- 
% \zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
% \\
% &\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right) \label{eq:Ghat full}
% \end{align}

% \begin{align}
% \vb^T\Ghat_\qb(0,\w) 
% &=\Big[\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corqv + \left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corwv  \nn
% \\&\qquad\qquad\qquad+{(\zeta-\zeta^2)\corqv}\left(\w^T\Sigmab\w/T\right)
% -(\zeta-\zeta^2)\corq \vb^T\Sigmab\w
% -\left(2\zeta\corq\right)\frac{1-\zeta}{T}\vb^T\Sigmab\w
% \Big] \nn
% \\
% &\qquad+\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\corw\right)\corq\corqv+\left((\zeta-\zeta^2)\corw-(\zeta^2-\zeta^3)\left(\corw^2+\corq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
% \\
% &\qquad+\left[\left(-\zeta+2\zeta^2\right)\corq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corwv+(1-\zeta)\w^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corw - \zeta^2(\corq^2+\corw^2)+ \frac{(1-\zeta)}{T}\w^T\Sigmab\w\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\corw\right)\corqv+\left(-\zeta+2\zeta^2\right)\corq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\w\right)\right) \nn
% \\
% &\qquad\qquad\qquad+\left[\zeta\corq -2 \zeta^2\corq\corw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad
% +\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)^2y_i\right) \nn
% \\
% &\qquad\qquad\qquad+\left[1-2\zeta\corw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
% \\
% &\qquad+\left(1-\zeta\corw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w \right) \nn
% \\
% &\qquad\qquad\qquad- 
% \zeta \corq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w-(1-\zeta)\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad-\left[2\zeta\corq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\w^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\w\right) \nn
% \\
% &\qquad\qquad\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\w^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\right)\right) \nn 
% \\
% &\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)\right) \label{eq:Ghat full}
% \end{align}



%%%%%%%%%%% CHRISTOS CONCENTRATION
% \begin{align*}
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\big| \leq \frac{C}{\sqrt{n}}u\right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)\big| \leq \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2 }{\sqrt{nT}} u
% \right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n y_i\left(\gammab_i^T\w\right)\big| \leq C \frac{\sqrt{(1-\zeta)}K\|\w\|_2}{\sqrt{n T}} u
% \right)&\geq 1-2{e^{-c u^2}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)^2-\frac{(1-\zeta)}{T}\w^T\Sigmab\w\big| \leq C \frac{{(1-\zeta)}K^2\|\w\|_2^2}{{T\sqrt{n}}} u
% \right)&\geq 1-2{e^{-c\min\{u^2,u\sqrt{n}\}}}
% \\
% \Pr\left(\big|\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)^2y_i| \leq C \frac{{(1-\zeta)}K^2\|\w\|_2^2}{{T\sqrt{n}}} u
% \right)&\geq 1-2{e^{-c\min\{u^2,u\sqrt{n}\}}}
% \\
% \Pr\left(
%     |\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\w| \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}} u
%     \right) &\geq 1-2e^{-c\min\{u^2,u\sqrt{n}\}}
% \\
%     \Pr\left(
%     |\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\w - (1-\zeta)\w^T\Sigmab\vb| \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}} u
%     \right) &\geq 1-2e^{-c\min\{u^2,u\sqrt{n}\}}
% \\
%     \Pr\left(
%     \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\w\right)\left(\vb^T\hat\Sigmab_i\w-(1-\zeta)\w^T\Sigmab\vb\right)} \leq u\,\frac{C\sigma^3(1-\zeta)\|\w\|_2^2\|\vb\|_2}{T\sqrt{n}}\log{n}\, 
%     \right) &\geq 1-c'e^{-cu^{2/3}}
% \end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lem:psi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}
% ~

\vp
\noindent\underline{First bound:} Obvious by boundedness (hence, sub-gaussianity) of $y_i$ and Fact \ref{fact:psi_additive}.

\vp
\noindent\underline{Second bound:} For convenience set $\wt T=(1-\zeta)T$ and assume wlog that $\Rcc=[\wt T].$  Recall that $$\beta_i=\frac{1}{T}\sum_{t=1}^{\wt T} \z_{i,t}^T\w=\frac{1-\zeta}{\wt T} \sum_{t=1}^{\wt T}\z_{i,t}^T\w.
$$
Also
for all $t$: $\psinorm{\z_{i,t}^T\w}{2}\leq K\|\w\|_2$. Thus, from Fact \ref{fact:psi_additive}:
\begin{align}\label{eq:beta_psi2}
\psinorm{\beta_i}{2} \leq \frac{C\sigma(1-\zeta)\|\w\|_2}{\sqrt{\wt T}} = \frac{C\sigma\sqrt{(1-\zeta)}\|\w\|_2}{\sqrt{ T}}
\end{align}
The bound then follows by applying Fact \ref{fact:psi_additive} once more.  

For the second term in this bound  recall that $y_i\in\{\pm{1}\}$ and $\beta_i=\sum_t \z_{i,t}^T\w/T$. Also, for all $i\in[n]$: $y_i,\{\z_{i,t}\}_{t}$ are zero-mean and independent. Thus (i) $\E[y_i\beta_i]=0$, and (ii)  {$\{y_i\z_{i,t}\widesim{D} \z_{i,t} \text{ and } y_i\z_{i,t} \perp y_i\z_{i,t'} \} \implies y_i\beta_i\widesim{D} \beta_i$.} Thus, the same bound as the first term holds.

\vp
\noindent\underline{Third bound:} It is easy to compute 
\begin{align}\label{eq:beta2_expectation}
\E[\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]=\frac{1}{T^2}\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\w^T\z_{i,t}\z_{i,t'}\vb] = \frac{1-\zeta}{T}\vb^T\Sigmab\w,
\end{align} 
and, using \eqref{eq:beta_psi2}
\begin{align}\label{eq:beta2_psi1}
\psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)-\E[\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]}{1} \leq C \psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)}{1} \leq  C \psinorm{\gammab_i^T\w}{2}\psinorm{\gammab_i^T\vb}{2} = \frac{C\sigma^2{(1-\zeta)}\|\w\|_2\|\vb\|_2}{{T}}.
\end{align}
Since $\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right), i\in[n]$ are independent, the desired bound on the first term follows from Fact \ref{fact:psi_additive}.

Consider now the second term. By independence of $y_i, \gammab_i$ it holds that $\E[y_i\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)]=0$. Arguing as we did above for the second bound, $y_i\gammab_i^T\w\widesim{D} \gammab_i^T\w$. Hence, the subexponential bound is the same as for the first term.


\vp
\noindent\underline{Fourth bound:} First, it is easy to compute that for all $i\in[n]$:
$$
\E[\w^T\Sigmab_i\vb]=\frac{1}{T}\E[\w^T\Z_i^T\Z_i\vb] = \frac{1}{T}\sum_{t=1}^{\wt T}\E[\w^T\z_{i,t}^T\z_{i,t}\vb] = \frac{\wt T}{T}\w^T\Sigmab\vb = (1-\zeta)\w^T\Sigmab\vb.
$$
Thus,
\begin{align*}
\w^T\hat\Sigmab_i\vb-\E[\w^T\hat\Sigmab_i\vb]=\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb
%=\frac{1}{T}\w^T\Z_i^T\Z_i\vb-(1-\zeta)\w^T\Sigma \vb
=\frac{1}{T}\sum_{t=1}^{\wt T}\Big((\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\Big)
\end{align*}
and so
\begin{align*}
\frac{1}{n}\sum_{i=1}^{n}\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb
%=\frac{1}{T}\w^T\Z_i^T\Z_i\vb-(1-\zeta)\w^T\Sigma \vb
=\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^{\wt T}\Big((\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\Big).
\end{align*}
Now, each random variable in the double sum above is independent and such that
\begin{align}\label{eq:wSv}
\|(\z_{i,t}^T\w)(\z_{i,t}^T\vb)-\w^T\Sigmab \vb\|_{\psi_1}\le 2\|(\z_{i,t}^T\w)(\z_{i,t}^T\vb)\|_{\psi_1}\le 2\|\z_{i,t}^T\w\|_{\psi_2}\|\z_{i,t}^T\vb\|_{\psi_2}\le C\sigma^2\|\w\|_2\|\vb\|_2.
\end{align}
Hence, from Fact \ref{fact:psi_additive},
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i=1}^{n}\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab \vb}{1}\leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{nT}}
\end{align*}


The bound for the second term follows along the same lines. The two key observations are that (i) $\E[y_i\w^T\hat\Sigmab_i\vb]=0$ because $y_i$ and $\z_{i,t}$ are independent, and, (ii) 
\begin{align*}
y_i\w^T\hat\Sigmab_i\vb=
\frac{1}{T}\w^Ty_i\Z_i^T\Z_i\vb \widesim{D} \frac{1}{T}\w^T\wt\Z_i^T\Z_i\vb
=\frac{1}{T}\sum_{t=1}^{\wt T}(\wt\z_{i,t}^T\w)(\z_{i,t}^T\vb)
\end{align*}
where $\wt\Z_i$ is an independent copy of $\Z_i$.

\vp
\noindent\underline{Fifth bound:}From \eqref{eq:beta2_psi1} and \eqref{eq:beta2_expectation}, we have for all $i\in[n]$ that
\begin{align*}\label{eq:beta2_psi1}
\psinorm{\left(\gammab_i^T\w\right)\left(\gammab_i^T\vb\right)-\frac{1-\zeta}{T}\w^T\Sigmab\w}{1} \leq \frac{C\sigma^2{(1-\zeta)}\|\w\|_2^2}{{T}}.
\end{align*}
Moreover, recall from Eq. \eqref{eq:beta_psi2} that
$$
\psinorm{\gammab_i^T\vb}{2}\leq  \frac{C\sigma\sqrt{1-\zeta}\|\vb\|_2}{\sqrt{ T}}.
$$
Combining the above two displays and applying Fact \ref{fact:orlitz_inequality} we find for all $i\in[n]$ that
\begin{align}
\psinorm{\left(\left(\gammab_i^T\w\right)^2-\frac{1-\zeta}{T}{\w^T\Sigmab\w}\right)\gammab_i^T\vb}{2/3}&\leq \frac{C\sigma^3(1-\zeta)^{3/2}\|\w\|_2^2\|\vb\|_2}{T^{3/2}}.
\end{align}
The desired bound follows from the above after using Fact \ref{fact:psi_heavy_Talagrand}.


\vp
\noindent\underline{Sixth bound:}
From Eq. \eqref{eq:wSv}:
$$
\psinorm{\w^T\hat\Sigmab_i\vb - (1-\zeta)\w^T\Sigmab\vb}{1} \leq \frac{C\sigma^2\sqrt{1-\zeta}\|\w\|_2\|\vb\|_2}{\sqrt{T}}
$$
and from Eq. \eqref{eq:beta_psi2}
$$
\psinorm{\gammab_i^T\w}{2}\leq  \frac{C\sigma\sqrt{1-\zeta}\|\w\|_2}{\sqrt{ T}}.
$$
Next we use Fact \ref{fact:orlitz_inequality} with $\alpha=2$ and $\beta=1$ to find that 
\begin{align*}
\psinorm{\left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3} \leq 
 \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T}}
\end{align*}
Next we use Fact \ref{fact:psi_heavy_Talagrand} which allows us to conclude that 
\begin{align*}
\psinorm{\frac{1}{n}\sum_{i=1}^n \left(\gammab_i^T\w\right)\left(\w^T\hat\Sigmab_i\vb-(1-\zeta)\w^T\Sigmab\vb\right)}{2/3}\le  \frac{ C K^3({1-\zeta})\|\w\|_2^2\|\vb\|_2}{{T\sqrt{n}}}\log n
\end{align*}
Finally, the zero-mean property follows since
\begin{align*}
\E[\left(\ones^T\Z_i\w\right)\left(\w^T\Z_i\Z_i^T\vb\right)] &= 
\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\left(\z_{i,t}^T\w\right)\left(\w^T\z_{i,t'}\z_{i,t'}^T\vb\right)]
= 
\sum_{t=1}^{\wt T}\sum_{t'=1}^{\wt T}\E[\w^T\z_{i,t}\tr\left({\z_{i,t'}\z_{i,t'}^T\vb\w^T}\right)]
\\
&=
\wt T^2\E[\tr\left(\z^T\w\right)\tr\left({\z\z^T\vb\w^T}\right)] = \wt T^2\E[\tr\left( (\z^T\w) \otimes (\z\z^T\vb\w^T)\right)]
\\
&=
\wt T^2\tr\left( \E[(\z^T\otimes \z\z^T)] (\w\otimes\vb\w^T)\right) = 0
\end{align*}
where the last equality follows by the zero third moment property in Assumption \ref{ass:noise}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finite-sample analysis: First and second gradient steps}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{assumption}
\red{In the following, we assume without explicit further reference that Ass. \ref{ass:rho general but small} holds (i.e. $\abs{\rho}<\wnorm/\qnorm$) and additionally that $\qnorm>\wnorm$. To simplify the results we further assume $\sigma\propto 1$ and $W\propto 1$.}
\end{assumption}


The lemma below studies the deviation of the first-step of GD $\what_1$ with respect to its population counterpart $\w_1$.  Provided that $n$ and $n\zeta T /d$ are larger than appropriate functions of other problem parameters, then the deviations are of small multiplicative order. We remark that the constants below have not been optimized (eg. the factor $1/2$ in \eqref{eq:w1hat corr} is arbitrary and can be replaced by and small positive constant by appropriately increasing the constant $C$ in \eqref{eq:large n lemma}).
\begin{lemma}[First gradient step]\label{lem:1st gradient step}
Consider the one-step population and finite updates $\w_1=\eta\G_\w(0,0)$ and $\what_1=\eta\Ghat_\w(0,0)$, respectively. For convenience denote $\corw=\w_1^T\wstar, \corq=\w_1^T\qstar$ and $\hcorw=\what_1^T\wstar, \hcorq=\what_1^T\qstar$ their finite-sample counterparts. 

For any $u>0$ and any small constant $c_0>0$, there exist absolute constants $c,c'>0$ and large enough  constant $C>0$ such that if
\begin{align}\label{eq:large n lemma}
    \red{\sqrt{n}}&\red{\geq C u}
    %\left(1\maxi \abs{\rho}\qnorm/\wnorm \right)
    \qquad\text{and}\qquad
    \sqrt{n\zeta T}\geq C u \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}\, ,
\end{align}
then, with probability at least $1-c'e^{-cu^2}$
    \begin{align}\label{eq:w1hat corr}
        \abs{\hcorw-\corw}\leq c_0\corw\qquad\text{and}\qquad\abs{\hcorq-\corq}\leq \red{c_0\eta \zeta \qnorm(\qnorm+\wnorm)}\,.
    \end{align}
    Additionally, if 
    \begin{align}
    \sqrt{n}&\geq Cu\qnorm/\wnorm
    \qquad\text{and}\qquad
    \sqrt{n\zeta T}\geq Cu \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}  \sqrt{d}
\end{align}
then with the same probability 
\begin{align}\label{eq:w1hat norm}
    \abs{\tn{\what_1}-\tn{\w_1}}\leq\red{c_0{\eta\zeta(\wnorm+\qnorm)}}.
\end{align}
\end{lemma}
\begin{proof}
Note that the conclusions of the lemma are all homogeneous in $\eta$. Hence, without loss of generality, set $\eta=1$.

    By Lemma \ref{lem:w_der_finite},
    \begin{align}\label{eq:what_1 first eq}
\what_1=\Ghat_\w(0,0)
&=  \zeta \w_\star + \zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ 
\frac{1}{n}\sum_{i}y_i\gammab_i.
\end{align}
and recall $\w_1=\G_\w(0,0)=\zeta\wstar$ (thus, $\corw=\zeta\wnorm^2$).
From these, and also using Lemma \ref{lem:psi} , for any $u>0$ with probability at least $1-2e^{-cu^2}$
\begin{align}
\abs{\hcorw-\corw}&=\abs{\wstar^T(\what_1-\w_1)}\leq \zeta  \abs{\rho}\wnorm\qnorm \abs{\frac{1}{n}\sum_{i\in[n]}y_i}+ 
\abs{\frac{1}{n}\sum_{i}y_i\gammab_i^T\wstar}\leq  \frac{Cu\zeta   \abs{\rho}\wnorm\qnorm}{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\wnorm}{\sqrt{n\zeta T}}\nn
\\
&\leq c_0{\zeta \wnorm^2}=c_0{\corw}.\nn
\end{align}
where the last inequality follows by assuming $n,\zeta T$ large enough as in the condition of the lemma \red{and using  Ass. \ref{ass:rho general but small} that $\abs{\rho}\leq W/Q.$}
Similarly,  
\begin{align*}
\abs{\hcorq-\corq}=\abs{\qstar^T(\what_1-\w_1)}&\leq \zeta  \qnorm^2 \abs{\frac{1}{n}\sum_{i\in[n]}y_i}+ 
\abs{\frac{1}{n}\sum_{i}y_i\gammab_i^T\qstar}
\leq  \frac{Cu\zeta  \qnorm^2}{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\qnorm}{\sqrt{n\zeta T}}\nn\leq 
c_0{\zeta(\qnorm^2+\qnorm\wnorm)}
%\red{\eps\zeta\qnorm(\qnorm+\wnorm)}
\end{align*}
for sufficiently large $n$ as in \eqref{eq:large n lemma}.

Finally, 
\begin{align}
    \tn{\what_1}-\tn{\w_1}\leq \tn{\what_1-\w_1}\leq \frac{Cu\zeta\qnorm }{\sqrt{n}} + \frac{Cu\sigma\sqrt{1-\zeta}\sqrt{\zeta}\sqrt{d}}{\sqrt{n\zeta T}}\leq \red{c_0{\zeta \left(Q+W\right)}}%\frac{\zeta\wnorm}{2}=\frac{\tn{\w_1}}{2} 
    \label{eq:w1 norm diff}
\end{align}
where, again, the last inequality follows by assuming $n,\zeta T$ large enough as stated in the lemma. In the second inequality, we used from Lemma \ref{lem:psi} that $\sum_{i\in[n]}y_i\gammab_i/n$ is $C\sigma\sqrt{1-\zeta}/\sqrt{nT}$-subGaussian and applied Fact \ref{fact:norm subg} to get a high-probability bound on its euclidean norm.
\end{proof}



Next, we move on to the second gradient update in the direction of $\Ghat_\qb(0,\what_1).$ Recall our goal of controlling the relevance scores of signal and noisy tokens. The first lemma below takes a step in this direction by computing the signal and noise relevance scores assuming access to the population gradient $\G_\qb(0,\what_1):=\E\left[\Ghat_\qb(0,\what_1)\right].$
%
\begin{lemma}[$\Ghat_\qb(0,\cdot)$ control: Expectation term]\label{lem:finite q1 expectation}Let $\G_\qb(0,\w_1)=\E\left[\Ghat_\qb(0,\w_1)\right]$ be the expectation of a step in the $\qb$-gradient evaluated at $(0,\what_1)$ and recall that $\what_1=\eta\Ghat_\w(0,0)$ for $\eta>0.$ Suppose $\what_1$ satisfies \eqref{eq:w1hat corr} and \eqref{eq:w1hat norm} \red{for sufficiently small enough constant $c_0>0$.}
Further assume that the step-size $\eta$ satisfies the following for sufficiently small absolute constant $c_\eta>0$:
    \begin{align}\label{eq:eta small deviation}
    \eta<c_\eta /\qnorm^{2}
    \end{align}
Then, for $y\in\{\pm1\}$ it holds that

\begin{align}
\left(\qstar+y\wstar\right)^T\G_\qb(0,\hat\w_1) &\geq  \eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm\left(\red{\left(1/4-\rho^2/8-2c_0-c_0\wnorm^{-2}\right)\qnorm - \left(4\abs{\rho}\right)\wnorm} \right)\,
   \label{eq:finite signal exp}
\end{align}
Moreover, for fresh noise variables $\z_t, t\in\Rcc$ satisfying Assumption \ref{ass:noise}, it holds that
\begin{align}
\z_t^T\G_\qb(0,\hat\w_1)\eqd\eta\zeta\left(\zeta-\zeta^2\right)\,\red{\sigma\sqrt{3}\left((9/4)\wnorm^2\qnorm+\sqrt{2}\wnorm^2+\sqrt{2}c_0\qnorm^2\wnorm+c_0\qnorm/2\right)} \cdot G_t,\quad G_t\sim\subg{1} \,.
\label{eq:finite noise exp}
\end{align}
\red{Finally, 
\begin{align}\label{eq:finite norm exp}
\tn{\G_\qb(0,\hat\w_1)}\leq\eta\zeta\left(\zeta-\zeta^2\right)\,\red{\sqrt{3}\left((9/4)\wnorm^2\qnorm+\sqrt{2}\wnorm^2+\sqrt{2}c_0\qnorm^2\wnorm+c_0\qnorm/2\right)}\,.
\label{eq:finite noise exp}
\end{align}
}
\end{lemma}

\begin{proof}
Fix any $\vb$ and recall the notation of Lemma \ref{lem:1st gradient step}. With these, we have from Lemma \ref{lem:conc_grad_q} that
\begin{align}
    \vb^T\G_\qb(0,\what_1)&=\left((\zeta-\zeta^2)\left(\hcorw+{\sigma^2\tn{\what_1}^2}/{T}\right)-(\zeta^2-\zeta^3)\left(\hcorw^2 + \hcorq^2\right)\right)\,\vb^T\qstar\nn
\\ 
&\qquad\qquad 
+\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\hcorw\right)\hcorq \,\vb^T\wstar\nn
-\sigma^2\left(1+{2}/{T}\right)(\zeta-\zeta^2)\hcorq\vb^T\what_1
\\
&=(\zeta-\zeta^2)\hcorw\left(1+{\sigma^2\tn{\what_1}^2}/({T}\hcorw)-\zeta\left(\hcorw + \hcorq^2/\hcorw\right)\right)\,\vb^T\qstar\nn
\\ 
&\qquad\qquad 
+(\zeta-\zeta^2)\hcorq \,\left(1-2\zeta\hcorw\right)\,\vb^T\wstar\nn
-\sigma^2\left(1+{2}/{T}\right)(\zeta-\zeta^2)\hcorq\vb^T\what_1
\\
&=(\zeta-\zeta^2)\hcorw\underbrace{\left(1+{\sigma^2\tn{\what_1}^2}/({T}\hcorw)-\zeta\left(\hcorw + \hcorq^2/\hcorw\right)\right)}_{:=\Chat_1}\,\vb^T\qstar\nn
\\ 
&\qquad
+(\zeta-\zeta^2)\hcorq \,\underbrace{\left(1-2\zeta\hcorw-\eta\zeta\sigma^2\left(1+{2}/{T}\right)\right)}_{:=\Chat_2}\,\vb^T\wstar -\underbrace{\eta\sigma^2\left(1+{2}/{T}\right)}_{:=\Chat_3}(\zeta-\zeta^2)\hcorq\vb^T\deltab_1\nn
%\label{eq:q1hat exp}
% \\
% &=:(\zeta-\zeta^2)\left(A\,\vb^T\qstar+B\,\vb^T\wstar +D\,\vb^T\deltab_1\right)\label{eq:q1hat exp}
\end{align}
where we used \eqref{eq:what_1 first eq} and set \[
\deltab_1:=(\what_1-\w_1)/\eta=\zeta  \qb_\star \left(\frac{1}{n}\sum_{i\in[n]}y_i\right)+ 
\frac{1}{n}\sum_{i}y_i\gammab_i.
\]

Recall from \eqref{eq:w1hat corr} and \eqref{eq:w1hat norm} that $\corw/2\leq \hcorw\leq 3\corw/2$, \red{$|\hcorq-\corq|\leq c_0\eta\zeta\qnorm^2$ and $\tn{\what_1}\leq \tn{\w_1}+c_0\eta\zeta\qnorm$.} Here and onwards, $c_0>0$ is a small enough absolute constant whose value may change from line to line. Also, $\corw=\eta\zeta\wnorm^2$, $\corq=\eta\zeta\rho\wnorm\qnorm$ and $\tn{\w_1}=\eta\zeta\wnorm$. With these, we can set step size $\eta$  small enough such that 
$\Chat_1\in[1/2,3/2]$, $\Chat_2\in[-1/8,1]$ and \red{$\Chat_3\in[0,(c_3/\zeta)/\qnorm^2]$ for constant $c_3>0$ to be made small enough later in the proof} .  
Also, recall from \eqref{eq:w1hat norm} that \red{
$
\tn{\deltab_1}\leq c_0\zeta\qnorm,.
$
}
Thus, \red{
\[
\Chat_3\abs{\hcorq}\tn{\deltab_1}\leq \frac{c_3}{\zeta\qnorm^2}\eta\zeta(c_0\qnorm^2+\rho\wnorm\qnorm)(c_0\zeta\qnorm)\leq c_3c_0\eta\zeta\,\qnorm\,.
\]}
\red{Moreover,
\begin{align*}
    \hat C_1 \hcorw \qnorm^2 &\geq \eta\zeta\wnorm^2\qnorm^2/4
    \\
    \hat C_2 \hcorq \rho\wnorm\qnorm &= \hat C_2 \rho\wnorm\qnorm\corq + C_2 \rho\wnorm\qnorm (\hcorq-\corq) \geq 
    -\eta\zeta\rho^2\qnorm^2\wnorm^2/8 - |\corq| c_0\eta\zeta\qnorm^2
        \\
        &\geq  
    -\eta\zeta\rho^2\qnorm^2\wnorm^2/8 - c_0\eta\zeta\wnorm^2\qnorm^2\,.
\end{align*}
}
Putting the above displays together we find that
\begin{align*}
    \qstar^T\G_\qb(0,\hat\w_1)&\geq \eta\zeta(\zeta-\zeta^2)\left(\wnorm^2\qnorm^2/4-\red{\rho^2\qnorm^2\wnorm^2/8 - c_0\wnorm^2\qnorm^2-c_3c_0\qnorm}\right)\,.
    % \\
    % &\geq  \eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm^2\left(15-8\rho^2-6\abs{\rho}\right)/64\nn
\end{align*}
\red{Similarly, we can compute that
\begin{align*}
    \abs{\hat C_1 \hcorw \rho \qnorm \wnorm} &\leq (9/4)\eta\zeta\wnorm^3\qnorm\abs{\rho}
    \\
    \abs{\hat C_2 \hcorq \wnorm^2} &\leq \eta\zeta(\abs{\rho}\wnorm^3\qnorm+c_0\qnorm^2\wnorm^2)\,.
\end{align*}
}
Hence, for $y\in\{\pm1\}$
\begin{align}
\abs{y\wstar^T\G_\qb(0,\hat\w_1)}\leq \eta\zeta\left(\zeta-\zeta^2\right)
\red{4\wnorm^3\qnorm\abs{\rho}+c_0\qnorm^2\wnorm^2+c_3c_0\qnorm}\,.\nn
\end{align}
The above two displays put together yield \eqref{eq:finite signal exp}.

To see \eqref{eq:finite noise exp}, note that
% \[
% \z_t^T\G_\qb(0,\hat\w_1)\Big/(\zeta-\zeta)^2=\left(\Chat_1\hcorw\qb+\Chat_2\hcorq+\Chat_3\deltab_1\right)^T\z_t
% \]
$\z_t^T\wstar\sim\subg{\sigma\wnorm},$ $\z_t^T\qstar\sim\subg{\sigma\qnorm}$ and $\z_t^T\deltab_1\sim\subg{\sigma\tn{\deltab_1}}.$ Thus,  the noise relevant scores are \iid subgaussian random variables with sub-gaussian constant $\sigmahat>0$ upper bounded as follows
\red{
\begin{align}
&\z_t^T\G_\qb(0,\hat\w_1)=\eta\zeta\left(\zeta-\zeta^2\right) \,\sigmahat \cdot G_t,~ G_t\sim\subg{1} \quad\text{and}
\label{eq:finite noise exp precise}
\\
&\qquad\qquad\sigmahat\leq \sigma\sqrt{3}\left((9/4)\wnorm^2\qnorm+\sqrt{2}\wnorm^2+\sqrt{2}c_0\qnorm^2\wnorm+c_3c_0\qnorm\right)\,.\nn
\end{align}
}
\end{proof}


The next lemma controls the effect on the relevance scores of the deviation  term $\Gtilde_\qb(0,\what)=\Ghat_\qb(0,\what)-\G_\qb(0,\what).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[$\Ghat_\qb(0,\cdot)$ control: Deviation term]
    \label{lem:finite q1 deviation}Let $\Gtilde_\qb(0,\what_1):=\Ghat_\qb(0,\what_1)-\G_\qb(0,\what_1)$ and suppose $\what_1$ satisfies \eqref{eq:w1hat corr} and \eqref{eq:w1hat norm}.
    %Further assume that the step-size $\eta$ satisfies \eqref{eq:eta small deviation} small absolute constant $c_\eta>0$. 
    Fix any $u>0$ and any small constant $c_1>0$. 
    Then, there exists small enough constant $c_\eta$ (dependent on $c_1$) such that if step-size $\eta$ is small enough as per \eqref{eq:eta small deviation} the  following statements hold with probability at least $1-c'e^{-cu^{2/3}}$ for positive constants $C,c',c>0$.

    
    First, for signal tokens, 
\begin{align}    
\abs{(\qstar+y\wstar)^T\Gtilde_\qb(0,\what_1)}\leq u\, C\,c_1\,\red{\qnorm^2}\left(1\maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}},\,\quad y\in\{\pm1\}\label{eq:finite signal dev}
\end{align}
Second, for fresh noise variables $\z_t, t\in\Rcc$ satisfying Assumption \ref{ass:noise}, it holds that
\begin{align}
\z_t^T\Gtilde_\qb(0,\hat\w_1)\sim\subg{\sigmatilde}\quad\text{where w.p. $\geq1-c'd\,e^{-cu^{2/3}}$}\quad 
\label{eq:finite noise dev}
\sigmatilde\leq u\,\sigma\, C\,c_1\,\left(\red{\qnorm} \maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}}\,.
\end{align}
\red{Third, 

\begin{align}\label{eq:finite norm dev}
    \tn{\Gtilde_\qb(0,\hat\w_1)}\leq u C\,c_1\,\left(\red{\qnorm} \maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}}\,.
    \end{align}
}
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
     We study each one of the terms of $\Gtilde_\qb(0,\what_1)$ in \eqref{eq:Ghat full} separately. We repeat the terms here for convenience, also noting the substitutions $\corw\leftarrow\hcorw=\what_1^T\wstar$ and $\corq\leftarrow\hcorq=\what_1^T\qstar.$
\begin{align} 
    \vb^T\Gtilde_\qb(0,\what_1)&=\left[\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\hcorw\right)\hcorq\corqv+\left((\zeta-\zeta^2)\hcorw-(\zeta^2-\zeta^3)\left(\hcorw^2+\hcorq^2\right)\right)\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\right) \nn
\\
&\qquad+\left[\left(-\zeta+2\zeta^2\right)\hcorq\corqv+\left(-\zeta+(-\zeta+2\zeta^2)\hcorw\right)\corwv+(1-\zeta)\what_1^T\Sigmab\vb\right]\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\hcorw - \zeta^2(\hcorq^2+\hcorw^2)+ \frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right] \left( \frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i\right) \nn
\\
&\qquad\qquad\qquad+\left[\left(-\zeta+(-\zeta+2\zeta^2)\hcorw\right)\corqv+\left(-\zeta+2\zeta^2\right)\hcorq\corwv\right]\left(\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\what_1\right)\right) \nn
\\
&\qquad\qquad\qquad+\left[\zeta\hcorq -2 \zeta^2\hcorq\hcorw\right]\left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad
+\zeta\corqv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right) \nn
\\
&\qquad\qquad\qquad+\zeta\corwv \left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2y_i\right) \nn
\\
&\qquad\qquad\qquad+\left[1-2\zeta\hcorw\right] \left( \frac{1}{n}\sum_{i=1}^{n}y_i\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)\right) \nn
\\
&\qquad+\left(1-\zeta\hcorw\right)\left(\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\what_1 \right) \nn
\\
&\qquad\qquad\qquad- 
\zeta \hcorq \left(\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\vb^T\Sigmab\what_1\right) \nn
\\
&\qquad-\left[2\zeta\hcorq\right]\left( \frac{1}{n}\sum_{i=1}^{n}\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\what_1\right) \nn
\\
&\qquad- \left(\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\what_1^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right)\right) \nn 
\\
&\qquad-\left(\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\left(\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\what_1^T\Sigmab\vb\right)\right) \,.\label{eq:Ghat full what}
\end{align}
Recall from the lemma assumption that \eqref{eq:w1hat corr} holds and from $\corw=\eta\zeta\wnorm^2$ and $\corq=\eta\zeta\rho\wnorm\qnorm$, that 
$1/2 \eta\zeta\wnorm^2\leq \hcorw\leq 3/2 \eta\zeta\wnorm^2$ and $\abs{\hcorq}\leq \red{\eta\zeta(\rho\wnorm\qnorm+c_0\qnorm^2)}$. The observation is that we can choose step-size $\eta$ small enough (as stated in \eqref{eq:eta small deviation}) to bound (in absolute value) all the coefficients in \eqref{eq:Ghat full what} (aka all terms in square brackets) that include  $\hcorw,\hcorq$.  Therefore, for any small positive constant $c_1>0$ it can be checked that there is sufficiently small constant $c_\eta$ that determines step-size $\eta$ in \eqref{eq:eta small deviation} such that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}    
\abs{\vb^T\Gtilde_\qb(0,\what_1)}&\leq c_1\left[\abs{\corqv}+\abs{\corwv}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i} \nn
\\
&\qquad+\left[c_1\abs{\corqv}+c_1\abs{\corwv}+(1-\zeta)\sigma^2\abs{\what_1^T\vb}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)}\nn
\\
&\qquad\qquad\qquad+\left[c_1+ \frac{(1-\zeta)}{T}\sigma^2\tn{\what_1}^2\right] \abs{\frac{1}{n}\sum_{i=1}^{n}\vb^T\gammab_i} \nn
\\
&\qquad\qquad\qquad+\left[c_1\abs{\corqv}+c_1\abs{\corwv}\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\left(\gammab_i^T\what_1\right)} \nn
\\
&\qquad\qquad\qquad+\left[c_1\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\left(\vb^T\gammab_i\right)}\nn
\\
&\qquad
+\zeta\abs{\corqv} \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1} \nn
\\
&\qquad\qquad\qquad+\zeta\abs{\corwv} \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)^2y_i} \nn
\\
&\qquad\qquad\qquad+\left[1+c_1\right] \abs{ \frac{1}{n}\sum_{i=1}^{n}y_i\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)} \nn
\\
&\qquad+\left[1+c_1\right]\abs{\frac{1}{n}\sum_{i=1}^{n}y_i\vb^T\hat\Sigmab_i\what_1}\nn
\\
&\qquad\qquad\qquad + c_1\abs{\frac{1}{n}\sum_{i=1}^{n}\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\vb^T\Sigmab\what_1}\nn
\\
&\qquad+\left[c_1\right]\abs{ \frac{1}{n}\sum_{i=1}^{n}\left(\what_1^T\gammab_i\right)\left(\vb^T\gammab_i\right)-\frac{1-\zeta}{T}\vb^T\Sigmab\what_1} \nn
\\
&\qquad + \abs{\frac{1}{n}\sum_{i=1}^{n}\left(\vb^T\gammab_i\right)\left(\left(\what_1^T\gammab_i\right)^2-\frac{(1-\zeta)}{T}\what_1^T\Sigmab\what_1\right)} \nn 
\\
&\qquad+\abs{\frac{1}{n}\sum_{i=1}^{n}\left(\gammab_i^T\what_1\right)\left(\vb^T\hat\Sigmab_i\what_1-(1-\zeta)\what_1^T\Sigmab\vb\right)}\,.\label{eq:Ghat full what simple}
\end{align}
Now, we use successively Lemma \ref{lem:conc_grad_q} to bound the random terms. Also note that $\abs{\corqv}\leq \qnorm\tn{\vb}$, $\abs{\corwv}\leq \wnorm\tn{\vb}$ and $\red{\tn{\what_1}\leq \eta\zeta(\wnorm+c_0\qnorm)=:\eta\zeta M}.$ For any $u>0$, with  probability at least $1-c'e^{-cu^{2/3}}$ we have

\begin{align}    
&\abs{\vb^T\Gtilde_\qb(0,\what_1)}\leq u\cdot\frac{C}{\sqrt{n}}\,\tn{\vb}\,c_1\left(\wnorm+\qnorm\right) \nn
\\
&+u\cdot\frac{C\sigma\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,\left( c_1\left(2\wnorm+2\qnorm+\eta\zeta(1-\zeta)\sigma^2 M\right)\eta\zeta M + \left(2c_1 + \sigma^2(1-\zeta)\eta^2\zeta^2 M^2/T\right) \right) \nn
\\
% %
% &\frac{C c_1\tn{\vb}\left(\wnorm+\qnorm+\eta\zeta(1-\zeta)\sigma^2\wnorm\right) \sigma\sqrt{1-\zeta}\eta\zeta\wnorm}{\sqrt{nT}}u\nn
% +\frac{C \left(c_1 + \sigma^2(1-\zeta)\eta^2\zeta^2W^2/T\right) \sigma\sqrt{1-\zeta}\tn{\vb}}{\sqrt{nT}}u\nn
% +\frac{C  c_1 \left(\wnorm+\qnorm\right)\tn{\vb}\sigma\sqrt{1-\zeta}\eta\zeta\wnorm}{\sqrt{nT}}u\nn
% \\
% &\qquad\qquad\qquad+\frac{C c_1 \sigma\sqrt{1-\zeta} \tn{\vb}}{\sqrt{nT}}u\nn
% \\
&+u\cdot\frac{C\sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,\left(\eta^2\zeta^3M^2\qnorm + \eta^2\zeta^3\wnorm M^2+(1+c_1)\eta\zeta M\right) \nn
% \\
% &
% +\frac{C (1-\zeta)\sigma^2\zeta\tn{\vb}\qnorm\eta^2\zeta^2\wnorm^2}{T\sqrt{n}}u \nn
% +\frac{C(1-\zeta)\sigma^2\zeta\tn{\vb}\wnorm\eta^2\zeta^2\wnorm^2}{T\sqrt{n}}u
%  \nn
% +
% \frac{C(1+c_1)(1-\zeta)\sigma^2\eta\zeta\wnorm\tn{\vb}}{T\sqrt{n}}u
%  \nn
\\
&+u\cdot\frac{C\sigma^2\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,\left((1+2c_1)\eta\zeta M\right)\nn
% \\
% &+\frac{C(1+c_1)\sigma^2\sqrt{1-\zeta}\eta\zeta\wnorm\tn{\vb}}{\sqrt{nT}}u\nn
% + \frac{C c_1 \sigma^2\sqrt{1-\zeta}\eta\zeta\wnorm\tn{\vb}}{\sqrt{nT}}u
\\
&+u\,\frac{C \sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,\left(c_1\eta\zeta M\right) \nn
\\
&+
u\,\frac{C\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}\,\tn{\vb}\,\left( \eta^2\zeta^2 M^2\right)
 \nn 
\\
&+
u\,\frac{C\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}\,\tn{\vb}\,\eta^2\zeta^2 M^2
\,.\label{eq:Ghat full what simple with concentration}
\end{align}

Now, again  using small step size $\eta$ as per \eqref{eq:eta small deviation} (recall that $M=\wnorm+c_0\qnorm\leq(1+c_0)\qnorm$), this can be further simplified to the following (here the value of constant $c_1$ might be different from \eqref{eq:Ghat full what simple with concentration})
\begin{align}    
\abs{\vb^T\Gtilde_\qb(0,\what_1)}&\leq u\cdot\frac{C}{\sqrt{n}}\,\tn{\vb}\,c_1\left(\wnorm+\qnorm\right)
+u\cdot\frac{C\sigma\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,c_1\nn
+u\cdot\frac{C\sigma^2(1-\zeta)}{T\sqrt{n}}\,\tn{\vb}\,c_1 \nn
\\
&\quad+u\cdot\frac{C\sigma^2\sqrt{1-\zeta}}{\sqrt{nT}}\,\tn{\vb}\,c_1
+
u\,\frac{C\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}\,\tn{\vb}\,c_1
 \nn 
+
u\,\frac{C\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}\,\tn{\vb}\,c_1
\,
\\
&\leq u\cdot\tn{\vb}\cdot \frac{C}{\sqrt{n}} \cdot c_1 \left(\qnorm\maxi\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^2}{T}\maxi\frac{\sigma^3\log(n)}{T^{3/2}}\maxi\frac{\sigma^3\log(n)}{T}\right) \nn
\\
&\leq u\cdot\tn{\vb}\cdot \frac{C\,\log(n)}{\sqrt{n}} \cdot c_1 \left(\qnorm\maxi\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right) \label{eq:Ghat full what simple with concentration very simple to use}
\end{align}

%.\label{eq:Ghat full what simple with concentration very simple}
% \begin{align}    
% \frac{\abs{\vb^T\Gtilde_\qb(0,\what_1)}}{\tn{\vb}}&\leq \frac{C c_1\left(\wnorm+\qnorm\right)}{\sqrt{n}}u \nn
% +\frac{C c_1\sigma\sqrt{1-\zeta}}{\sqrt{nT}}u\nn
% +\frac{C c_1 (1-\zeta)\sigma^2\zeta}{T\sqrt{n}}u \nn
% + \frac{C c_1 \sigma\sqrt{1-\zeta}}{\sqrt{nT}}u
% \\
% &\qquad\qquad\qquad\qquad+
% \frac{Cc_1\sigma^3(1-\zeta)^{3/2}\log(n)}{T^{3/2}\sqrt{n}}u
% +
% \frac{Cc_1\sigma^3(1-\zeta)\log(n)}{T\sqrt{n}}u
% \\
% &\leq \frac{Cc_1(\wnorm+\qnorm)\poly{\sigma}\log(n)}{\sqrt{n}}u
% \,.\label{eq:Gtilde full what simple with concentration}
% \end{align}


Now, we can compute the deviation of the relevance scores. For signal tokens we have for both $y\in\{\pm1\}$, and all $u>0$ with probability at least $1-c'e^{-cu^{2/3}}$, there exist constant $C>0$ such that
\begin{align}    
\abs{(\qstar+y\wstar)^T\Gtilde_\qb(0,\what_1)}\leq u\, C\left\qnorm\left(\qnorm\maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}} \label{eq:finite signal dev 2}
\end{align}

For a noisy token $\z_t,t\in\Rcc$ note that $ \z_t^T\Gtilde_\qb(0,\what_1)\sim\subg{\sigma\tn{\Gtilde_\qb(0,\what_1)}}$. We can bound $\tn{\Gtilde_\qb(0,\what_1)}$ applying \eqref{eq:Ghat full what simple with concentration very simple to use} for all standard basis vectors $\vb=\eb_j, j\in[n]$ and union bounding. This gives for all $u>0$ with probability at least $1-c'de^{-cu^{2/3}},$
\[
\tn{\Gtilde_\qb(0,\what_1)}\leq u\, C\left(\qnorm \maxi \frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T}\right)\frac{\log(n)}{\sqrt{n}}\,.
\]

% for all $t\in\Rcc$ and all $u>0$ with probability at least $1-c'de^{-cu^{2/3}},$
% \begin{align}
%     \z_t^T\Gtilde_\qb(0,\what_1)\sim \subg{\sigmatilde}\qquad \sigmatilde\leq Cc_1(\wnorm+\qnorm)\sigma\poly{\sigma}\frac{\log(n)}{\sqrt{n}}u
%     \label{eq:finite noise dev}
% \end{align}
% where to bound $\tn{\Gtilde_\qb(0,\what_1)}$, we applied union bound.
\end{proof}

With lemmas \ref{lem:finite q1 expectation} and \ref{lem:finite q1 deviation} at hand, we are now ready to put things together stating our final bounds for relevance scores. The finding is presented as a stand-alone lemma below.
\begin{lemma}[Put things together]\label{putogether1}
    Consider the finite-sample gradient step
    $\qhat_1=\Ghat_\qb(0,\what_1)$, where recall that $\what_1=\eta\Ghat_\w(0,0).$
    Fix any $u_0,u_1,u_2,u_3>0$ and any small constants $\red{\wt{c}_0,} \wt{c}_1>0$.
    Suppose step-size $\eta$ of first gradient step satisfies \eqref{eq:eta small deviation} for sufficiently small constant $c_\eta>0$ (dependent on $\wt{c}_1$) and further assume
\begin{align}
    \red{\sqrt{n}}&\red{\geq u_0\cdot C_0}%  \frac{\qnorm}{\wnorm}
    \qquad\text{and}\qquad
    \sqrt{\frac{n\zeta T}{d}}\geq   u_0 \cdot C_0  \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}.
\end{align}
for some large enough  constant $C_0>0$. Finally, assume for simplicity that
\begin{align}\label{eq:strignent for convenience}
\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T} \leq \red{ \qnorm.}
\end{align}
Consider a fresh dataset $(\X_i,y_i)_{i\in[n]}$ and consider the signal and noise relevance scores $\rhat_{i,t}:=r_{i,0}:=\left(\qstar+y_i\wstar\right)^T\qhat_1, t\in\Rc$ and $\rhat_{i,t}:=\z_{i,t}^T\qhat_1, t\in\Rcc$, respectively.  
Then, there exist positive absolute constants $c_i,c_i',i=0,1,2,3$ such that the following statements hold
\begin{itemize}
    \item With probability at least $1-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}},$ the signal relevance scores satisfy
    \begin{align}
    \label{eqcomb1}
        \min_{i\in[n]} r_{i,0} \geq  \eta\zeta
        (\zeta-\zeta^2)\wnorm^2\qnorm\red{\left(\left(1/4-\rho^2/8-2\wt{c_0}-\wt{c_0} W^{-2}\right)\qnorm - 4\abs{\rho}\wnorm \right)
        - 
        u_1\, \wt{c}_1\, \qnorm^2\frac{\log(n)}{\sqrt{n}}}=:B(u_1)\,.
        %u_1 \cdot C_1(\wnorm+\qnorm)^2\poly{\sigma}\log(n) /\sqrt{n}
    \end{align}
    \item With probability at least $1-c_0'e^{-c_0u_0^2}-c_2'n(1-\zeta)Te^{-c_2u_2^2}-c_3'dn(1-\zeta)Te^{c_3u_3^{2/3}},$ the noise relevance scores satisfy
    \begin{align}
    \label{eqcomb2}
        \max_{i\in[n],t\in\Rcc}r_{i,t} \leq  u_2\,\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \red{\,\sigma \left(1+\wt{c_0}\qnorm\right)  + u_3\,\sigma\, \wt{c}_1\,\qnorm \frac{\log(n)}{\sqrt{n}}}=:M(u_2,u_3)
    \end{align}
\end{itemize}

\end{lemma}
\begin{proof} The lemma follows by collecting \eqref{eq:finite signal exp}, \eqref{eq:finite signal dev}, \eqref{eq:finite noise exp}, \eqref{eq:finite noise dev}, and applying union bound for the noise terms over $i\in[n],t\in\Rcc$.
\end{proof}

\begin{corollary}
In the setting of Lemma \ref{putogether1}. Suppose $n$ is large enough such that
\begin{align}
    \red{\sqrt{n}}&\red{\geq u_0\cdot C_0}%  \frac{\qnorm}{\wnorm}
    ,\qquad
    \sqrt{\frac{n\zeta T}{d}}\geq   u_0 \cdot C_0  \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}
    ,\qquad
    \sqrt{n}
\end{align}
Suppose 
\begin{align}\label{eq:key finite q_1 condition}
    \wnorm^2\left(\left(1/4-\rho^2/8-2\wt{c_0}-\wt{c_0} W^{-2}\right)\qnorm - 4\abs{\rho}\wnorm \right) \gtrsim Q
\end{align}

\end{corollary}
\begin{proof}
    Set $u_1\propto u_3 = \eta\zeta^2\frac{\sqrt{n}}{\log(n)}$.
    Suppose \eqref{eq:key finite q_1 condition} and denote for simplicity $A_Q:=\left(\left(1/4-\rho^2/8-2\wt{c_0}-\wt{c_0} W^{-2}\right)\qnorm - 4\abs{\rho}\wnorm \right).$ Then,
    \[
\eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm \cdot A_Q > 2 u_1 \wt c_1\qnorm^2 \frac{\log{n}}{\sqrt{n}}
    \]
    Similarly
    \[
\eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm > u_3 \wt c_1\qnorm \frac{\log{n}}{\sqrt{n}}
    \]
\end{proof}

==> initial_trajectory_results.tex <==
\section{Gradient-based analysis of prompt-attention}
\label{sec:gradient-algo}

This section investigates how gradient-descent optimization of the prompt-attention model learns \eqref{eq:CGMM}. Concretely, it shows that a few gradient steps can provably attend to the context-relevant tokens leading to high-classification accuracy. Our results capture requirements on sample complexity in terms of all problem parameters, i.e. dimension $d$, correlation $\rho$, context / signal energies $\qnorm$ / $\wnorm$, number of tokens $T$, and sparsity $\zeta$. This allows studying tradeoffs in different regimes. 

Our analysis in this section concerns the prompt-attention model $\fat_{\thetab}$, so we simply write $f_{\theta}$. {Also, without any further explicit reference, we focus on the \textit{core dataset model}, i.e. \eqref{eq:CGMM} with $\delta=(0,0)$. 
All our results here hold under the mild noise and correlation assumptions: Assumption \ref{ass:noise} and Assumption \ref{ass:rho general but small} (we will not further state these). Finally, for simplicity of presentation we assume here isotropic noise $\Sigmab=\sigma^2\Id$ and handle the general case in the appendix.}

\subsection{Gradient-based algorithm}
For data generated from \eqref{eq:CGMM}, we show the three-step gradient-based algorithm described below achieves high test accuracy. Our analysis also explains why three appropriately chosen steps suffice.


\noindent\textbf{Algorithm:} We split the train set in three separate subsets $\Sc_1,\Sc_2,\Sc_3$ of size $n$ each. Starting from $\w_0=0,\qb_0=0$, the algorithm proceeds in three gradient steps for step sizes $\eta>0$ and $\gamma>0$ and a final debiasing step as follows:
\begin{subequations}\label{eq:algo}
\begin{align}
&\what_1:=-\eta\nabla_{\w}\Lch_{\Sc_1}(0,0),\label{step1}\\
&\qhat_1:=-\gamma \nabla_{\qb}\Lch_{\Sc_2}(0,\what_1), \label{step2}\\
&{\what_2:=-\eta \nabla_{\w}\Lch_{\Sc_3}(\qhat_1,\what_1),} \label{step4}
% &\w_2=  \Fb^\dagger \y.\label{step3}
\end{align}    
\end{subequations}
where $\Lch_{\Sc_j}, j=1,2,3$ is the loss in \eqref{eq:loss} evaluated on sets $\Sc_j$. {The debiasing step is defined in Section~\ref{sec:finite analysis}.}
%\ct{Need to say that samples are fresh for each iteration}
% where $\Fb:=\Fb_{\qb_1}\in\R^{N\times d}$ is a feature matrix with $i$th row equal to $\X_i^\top\sft{\X_i\qb_1}$. The last row is same as running (infinite) gradient iterations on $\w$ with fixed $\qb_1$.


%where depending on using softmax or element-wise activation, $\sftd(\vb) = \diag{\sft(\vb)} - \sft(\vb)\sft(\vb)^\top$ or $\sftd(\vb)=\diag{\sftd(\vb)}$, respectively.  



\subsection{Population analysis}\label{sec:population analysis main}
To gain intuition
%on how Algorithm \eqref{eq:algo} can achieve high test accuracy and on what enables attending to relevant tokens, 
we first present results on the population counterpart of the algorithm, i.e., %\eqref{eq:algo} 
substituting $\Lch(\w,\qb)$ with its population version $\Lc(\w,\qb)=\E\left[\Lch(\w,\qb)\right]$ in all three steps in \eqref{eq:algo}.
%In this section, we focus on $\Lc(\cdot)$ rather than $\Lch(\cdot)$. 
It is convenient to introduce the following shorthand notation for the negative gradient steps
$\G_\qb(\qb,\w):=-\nabla_{\qb}\Lc_{\Dc}(\thetab) = \E_{(\X, y)\sim \Dc}\big[ (y-f_{\thetab}(\X))\nabla_{\qb}f_{\thetab}(\X) \big] $ and 
$\G_\w(\qb,\w):=-\nabla_{\w}\Lc_{\Dc}(\thetab) = \E_{(\X, y)\sim \Dc}\big[ (y-f_{\thetab}(\X))\nabla_{\w}f_{\thetab}(\X) \big]\,. 
$
% where the gradients of $\fat$ are evaluated as follows:
% $
% \nabla_\qb \fat_{\thetab}(\X) = 
% \X^\top\sftd {\X\qb}\X \w, 
% $
% and
% $\nabla_\w \fat_{\thetab}(\X) = 
% \X^\top\sft{\X\qb},
% $
% with $\sftd{\vb} := \diag{\sft{\vb}} - \sft{\vb}\sft{\vb}^\top$.

%We analyze each of the algorithm's three steps separately to investigate their roles.
The first gradient step (cf.~\eqref{step1}) is easy to calculate and returns a classifier estimate that is already in the direction of $\wstar.$
\begin{lemma}[Population first step]\label{lem:w_der_pop}
 %Under dataset model \eqref{eq:CGMM}, 
 The first population gradient step $\w_1=\eta\G_\w(0,0)$ satisfies $\w_1=\eta\zeta\wstar$ since under \eqref{eq:CGMM}, 
$\G_\w(0,0)={\E_{(\X, y)}[ y\X^\top\ones]}/{T} = \zeta  \wstar.$
\end{lemma}


The second gradient step $\qb_1=\gamma\G_\w(\w_1,0)$ is more intricate: unless $\qstar\perp\wstar$, $\qb_1$ also has nonzero components in both directions $\qstar$ and $\wstar.$

% Intuitively, we would like that $\qb_1$ is in the direction of $\qstar$ so that prompt-attention attends to the context-relevant tokens. As the next lemma shows in the general scenario where $\qstar\not\perp\wstar$, $\qb_1$ also has nonzero components in the direction of $\wstar.$

\begin{lemma}[Population second step]\label{lem:q_der_pop}The second population gradient step $\qb_1=\gamma\G_\w(\w_1,0)$ satisfies for $\alpha:=\eta\zeta$
\begin{align}
\hspace{-0.1in}\qb_1
&= \gamma\alpha\wnorm^2(\zeta-\zeta^2)\big(1+\frac{\alpha\sigma^2}{T}-\alpha\zeta(\wnorm^2 +\rho^2\qnorm^2)\big)\qstar
\label{eq:pop_one_step_grad_q}
%\label{eq:pop_one_step_grad_q_Isotropic}
\\ 
&\quad+\gamma\alpha\rho\qnorm\wnorm(\zeta-\zeta^2) \big(1-2\zeta\alpha\wnorm^2-(1+\frac{2}{T})\alpha\sigma^2\big)\,\wstar\,.\nn
\end{align}


% \begin{align}
% \G_\qb(0,\alpha\wstar)
% &= \left((\zeta-\zeta^2)\left(\alpha\wnorm^2+\alpha^2{\wstar^\top\Sigmab\wstar}/{T}\right)-\alpha^2(\zeta^2-\zeta^3)\left(\wnorm^4 + \left(\wstar^\top\qstar\right)^2\right)\right)\,\qstar\nn
% \\ 
% &\qquad\qquad 
% +\left(\left((\zeta-\zeta^2)-2(\zeta^2-\zeta^3)\alpha\wnorm^2\right)\alpha\left(\wstar^\top\qstar\right) \right)\,\wstar\nn
% \\
% &\qquad\qquad -\left(\left(1+{2}/{T}\right)(\zeta-\zeta^2)\alpha\left(\wstar^\top\qstar\right)\right)\alpha\Sigmab\wstar
% \label{eq:pop_one_step_grad_q}
% \end{align}
% Specifically, if $\Sigmab=\sigma^2I_d$, then
% \begin{align}
% \G_\qb(0,\alpha\wstar)
% &= \alpha\wnorm^2(\zeta-\zeta^2)\left(\left(1+\alpha\sigma^2/{T}\right)-\alpha\zeta\left(\wnorm^2 + \left(\wstar^\top\qstar\big/\wnorm\right)^2\right)\right)\,\qstar\nn
% \\ 
% &\qquad\qquad +\alpha\left(\wstar^\top\qstar\right)(\zeta-\zeta^2) \left(1-2\zeta\alpha\wnorm^2-\left(1+2/T\right)\alpha\sigma^2\right)\,\wstar
% \label{eq:pop_one_step_grad_q_Isotropic}
% \end{align}
\end{lemma}

\begin{proof} Since this computation involves several terms, we defer  complete proof to Appendix \ref{sec:proof lemma q population}. The above simplification is  made possible by leveraging the assumption on the third-moment of noise (cf.~Assumption \ref{ass:noise}).
\end{proof}

 Lemma \ref{lem:q_der_pop} highlights the following key aspects: (i) As mentioned, $\qb_1$ also picks up the  $\wstar$ direction unless $\rho=0$. However,  we can control the magnitude of this undesired term by choosing small step-size $\eta$ (see Cor. \ref{cor1}). (ii) As $\alpha\wnorm^2$ grows, the gradient component in the $\qstar$ direction might end up pointing in the direction of $-\qstar$. This is because large signal along the $\wstar$ direction might still allow to predict $\pm 1$ label. However, this can always be avoided by choosing sufficiently small step-size $\eta$ (see Cor. \ref{cor1}). (iii) Similarly,  as the noise strength $\sigma^2$ grows, gradient in the $\qb_\star$ direction grows as well. This is because, going along $\qstar$ direction attenuates the noise and cleans up the prediction. (iv) Finally, as $\zeta\rightarrow 1$ and $\zeta-\zetab\rightarrow 0$ the magnitude of the gradient decays because all tokens contain signal information and there is no need for $\qstar$.

% \begin{corollary} \label{cor1}Suppose $\zeta$ and $T$ are such that $\zetab\leq \zeta/2$. Also suppose learning rate obeys\footnote{Note that, this condition is guaranteed to hold if noise level is large.} $\eta( \wnorm^2-\sigma^2/T)\leq {1}/{2\zeta}$. For $C\geq 1/4$, we have that
% \[
% \G_\qb(0,\w_1)=C   {\eta\zeta}\zeta\wnorm^2\qb_\star
% \]
% \end{corollary}


% $\eta \zeta\big(\zeta(\wnorm^2+\qnorm^2)-\sigma^2/T\big)\leq {1}/{2},$
% $
% \eta\zeta\left(2\zeta\wnorm^2+(1+2/T)\sigma^2\right)\leq {5}/{4},$ 
% $ 
% and
% \eta\zeta\left(\sigma^2/T\right)\leq{1}/2.$

To see how $\qb_1$ selects good tokens, we  investigate the relevance scores (normalized by the step size $\gamma$) $r_t:=\x_t^\top\qb_1/\gamma$ of relevant vs irrelevant tokens. Attending to context-relevant tokens requires %the signal/context
their relevance scores to be larger than those of the noisy ones. Concretely, suppose we have
\begin{align}\label{eq:relevance scores desired}
  \hspace{-0.1in}  B:=\min_{t\in\Rc}\{r_t = \frac{(\qstar+y\wstar^\top)\qb_1}{\gamma}\} \geq 2\,\max_{t\in\Rcc} \{ r_t =\frac{ \z_t^\top\qb_1}{\gamma}\}.
\end{align}
Note above that the relevance scores are the same for each $t\in\Rc$.
%{\color{red}[Ankit]: Should we make clear all the $|\mathcal{R}|$ terms on the LHS above are actually equal (for our next bound to be true).}
Thus,  $|\Rc|\, e^{\gamma B} + |\Rcc| \,e^{\gamma B/2}\geq S:=\sum_{t'\in[T]}e^{\gamma r_{t'}}\geq |\Rc| \,e^{\gamma B},$
which implies the following for the attention weights 
%$a_t=[\phi(\X\qb_1)]_t=e^{\gamma r_t}/\sum_{t'\in[T]}e^{\gamma r_{t'}}$ 
as step size increases $\gamma\rightarrow\infty$:
\begin{align}
    a_t = [\phi(\X\qb_1)]_t = e^{\gamma r_t}/ S \begin{cases}=\frac{e^{\gamma B}}{S}\rightarrow \frac{1}{\zeta T
    } & t\in\Rc
    \\
    \leq \frac{e^{\gamma B/2}}{S}\rightarrow 0 & t\in\Rcc
    \end{cases}.
\end{align}
Provided \eqref{eq:relevance scores desired} holds, a large enough second gradient step (i.e. large $\gamma$) finds $\qb_1$ that attends (nearly) perfectly to context-relevant tokens in $\Rc$ and attenuates (almost) all irrelevant tokens in $\Rcc$. 
%After this critical step, it is rather intuitive that only one additional update $\what_2$ in the $\w$ direction suffices for good prediction. %\red{(The argument is similar to Section \ref{sec:samet's section}.)}
The following theorem formalizes the above intuition. 
%and computes the accuracy of the population version of Algorithm \ref{eq:algo} without the bias term with appropriate step-size choices. 
We defer the complete proof to Appendix \ref{sec:proof of gradient pop}. 
%We also remark that the asympytotic nature of the result with respect to $\gamma$ can be relaxed. Indeed, we show in Section \ref{sec:finite analysis} for finite-sample gradient updates that it suffices for $\gamma$  to be large enough.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ct{I have not finished the thm }
\begin{theorem}[Main theorem: Population] \label{thm:main grad pop}
% Assume for some $\alpha>1$
%$C>1$ (specifically, $C=1$ for Gaussian noise)
Consider the model $\thetab^\gamma=(\w_2^\gamma,\qb_1^\gamma)$ where $\qb_1^\gamma=\gamma \G_{\qb}(\w_1,0)$, $\w_2^\gamma=\G_\w(0,\qb_1^\gamma)$ and $\w_1=\eta\G_\w(0,0)$ for step-size $\eta$ small enough (see Eq. \eqref{eq:eta small pop} for details). Then,
there exists an absolute constant $c>0$, {sufficiently large context strength $Q$} 
%\red{[Why do we add ``sufficiently large'' here? I believe this is true for any $\alpha$ obeying the condition.]} 
and step-size $\gamma>0$ such that
% % In the proof, we simply set it as failure prob $1/T^{\alpha-1}=\delta$
% \begin{align}\label{eq:? gamma infty}
%     \wnorm\left(\wnorm-\rho\qnorm\right)&\geq \frac{C}{T^{\alpha-1}}\left(\left(-\wnorm^2+\qnorm^2+\abs{\rho}\qnorm\wnorm\right)+ \left(-\wnorm+\qnorm\right)\sigma\sqrt{d}\sqrt{\log\left(2(1-\zeta)T^{2-\alpha}\right)}\right)\nn
% \end{align}
%then in the limit of $\gamma\rightarrow\infty$, the error of the model obeys
%\lim_{\gamma\rightarrow\infty}
% \[
% \acc\left({f_{\thetab^\gamma}}\right)\leq 2/T^{\alpha-1}\,,
% \]
\[
% \red{\acc\left({f_{\thetab^\gamma}}\right)\leq 2e^{-{(\alpha-1)}\log(T)}\,,}
{\acc\left({f_{\thetab^\gamma}}\right)\leq 2Te^{-c{\frac{\alpha^2\qnorm^2}{\sigma^2}}}\,,}
\]
provided %\footnote{{Specifically for isotropic Gaussian noise $\z\sim\Nc(0,\sigma^2 I)$ we have $c=\sqrt{2}\big/4$ in \eqref{eq:clean noise condition}.}}
% \begin{align}\label{eq:clean noise condition}
%    \sigma\sqrt{\log\left(2(1-\zeta)T^\alpha\right)} \leq \frac{({1-\rho^2/2})\qnorm - {2\abs{\rho}}\wnorm}{
%    %2\sqrt{2}
%    {\sqrt{1+3\rho^2}}}\,.
% \end{align}
{
\begin{align}\label{eq:clean noise condition}
    \frac{({1-\rho^2/2})\qnorm - {2\abs{\rho}}\wnorm}{
   %2\sqrt{2}
   {\sqrt{1+3\rho^2}}} \geq \alpha \qnorm\,.
\end{align}
}
%is no larger than $1/T^{\alpha-1}.$
%\red{Check statement and proof}
% The test risk obeys
% \[
% \lim_{\gamma\rightarrow\infty }\Lc(\thetab^\gamma) {=\frac{\rho^2\qnorm^2}{2\wnorm^2}.}
% %=0.
% \]
\end{theorem}
% The proof of the theorem is given in Section \ref{sec:proof of gradient pop}.

Eq. \eqref{eq:clean noise condition} guarantees the desired condition \eqref{eq:relevance scores desired} holds. When $\rho=0$ ($\qstar\perp\wstar$), 
{$\alpha$ can be as large as $1$ in \eqref{eq:clean noise condition} in which case the rate is $2Te^{-c\qnorm^2/\sigma^2}$.} %it requires 
% $Q=\Omega(\sqrt{\log(T)})$
%in order to attend to context-relevant tokens irrespective of  sparsity level $\zeta.$ 
For $\rho\neq0$, \eqref{eq:clean noise condition} imposes $\abs{\rho}<\frac{Q}{2W}$, in which the role of $Q,W$ is reversed compared to $\abs{\rho}\leq \frac{W}{Q}$ in  Assumption \ref{ass:rho general but small}: the latter guarantees classifier energy is larger so that signal $y\wstar$ dominates $\qstar$, while for prompt-attention to attend to relevant tokens it is favorable that energy of $\qstar$ dominates $\wstar.$
{Finally, we compare the theorem's error to the error $Q(\sqrt{\frac{\zeta^2W^2T}{1-\zeta}})$ of the linear model in Fact \ref{lin func fact}. For concreteness, consider a setting of  extreme sparsity $\zeta=O(1/\sqrt{T})$ and $\wnorm=O(1)$. Then the error of linear model is $O(1)$, while the (population) algorithm in \eqref{eq:algo} for \prml achieves an error of ${e^{-O(\qnorm^2)}}$, which is exponentially decreasing in $\qnorm.$}
% and extreme sparsity $\zeta=O(1/\sqrt{T})$. Then the error of linear model is $O(1)$, while the (population) algorithm in \eqref{eq:algo} achieves an error of $O(1/T^{\alpha-1})={e^{-O(Q^2)}}$ for \prml, which is decreasing in $T$. 


% For concreteness, fix  $\wnorm=O(1)$, $\qnorm=O({\sqrt{\log(T)}})$ satisfying \eqref{eq:clean noise condition} and extreme sparsity $\zeta=O(1/\sqrt{T})$. Then the error of linear model is $O(1)$, while the (population) algorithm in \eqref{eq:algo} achieves an error of $O(1/T^{\alpha-1})={e^{-O(Q^2)}}$ for \prml, which is decreasing in $T$. 
%the error $O(1/T^{\alpha-1})={e^{-O(Q^2)}}$ of (population) Algorithm \ref{eq:algo} for prompt-attention is decreasing in $T.$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finite-sample analysis}\label{sec:finite analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here, we investigate the behavior of the algorithm in \eqref{eq:algo} with finite sample-size $n$. For convenience, we first introduce an additional de-biasing step after calculating the three gradients in \eqref{eq:algo}. Specifically, for a sample $\Sc_4$ of size $n$ we compute a bias variable
$
\widehat{b}:=\frac{1}{n}\sum_{i=1}^n f_{(\qhat_1,\what_2)}(\X_i)\,,%\label{stepb}
$
and use it to de-bias the model's prediction by outputting 
% and $\X_i^{(\Sc_4)}$ denotes the input examples of the fourth set $\Sc_4$. Here, $\hat{b}$ is a bias variable that helps with adjusting the decision boundary. During prediction, we will use the bias-enabled model 
$f_{(\thetab,b)}(\X):=f_{\thetab}(\X)-b$. While this extra step is not necessary, it simplifies the statement of our results. Intuitively, $\widehat{b}$ helps with adjusting the decision boundary by removing contributions of the context vector in the final prediction (the context vector is useful only for token-selection rather than final prediction).

Below we provide a simplified version of our main result where noise variance $\sigma\propto 1$ and $\gtrsim$ subsumes constants. Refer to Theorem \ref{thm:main finite appendix} {in the appendix} for precise details.
%For clarity,  and .
%$\wedge$ denotes the minimum of two numbers, and 
%\sout{and use $\gtrsim,\ordet{}$  to suppress logarithmic dependencies on $T,n$}. 

\begin{theorem}[Main theorem: Finite-sample]\label{thm:main finite appendix}
    Suppose $\qnorm, \wnorm$ and $\rho$ are such that there exists $\alpha\in(0,3/16)$ for which 
    \[
    \left(3/16-\rho^2/8\right)\qnorm - \left(9/4\abs{\rho}+1/16\right)\wnorm \geq \alpha \cdot Q\,\gtrsim \sqrt{\log(nT)}.
    %\log(n+T).
    \]
Fix any $\eps>0$. For sufficiently small step-size $\eta\lesssim\qnorm^{-2}$,  sufficiently large step-size $\gamma=\gamma(\eps)$, and 
\[
n\gtrsim d(Q/\zeta W)^4\log^5(nd),
\]
the following statements hold with high probability (see Eq. \eqref{long prob bound}) over the training set:

\noindent~\textbf{1. Prompt attends to relevant tokens.} Concretely, for any fresh sample $(\X,y)$, with probability at least $1-2Te^{-c\alpha^2\qnorm^2}$, the attention coefficients $a_t=\left[\sft{\X\qhat_1}\right]_t$ satisfy:
\begin{align*}
    a_t \begin{cases}
    \geq \frac{1-\eps}{\zeta T} & , t\in\Rc\,,
    \\
    \leq \frac{\eps}{(1-\zeta) T} & , t\notin\Rc\,.
    \end{cases}
\end{align*}

\noindent~\textbf{2. Prompt-attention learns relevant features.} Concretely, for some absolute constant $c>0$, 
\[
\Pro_{(\X,y)}\left(\tn{\X^\top\sft{\X\qhat_1}- (\qstar+y\wstar)}< \eps \right) \leq 2Te^{-c\alpha^2\qnorm^2}\,.
\]

\noindent~\textbf{3. The test error} of the model $f_{\thetab}'$ similarly satisfies
\[
\err(f'_{\thetab})\leq 2Te^{-c\alpha^2\qnorm^2}\,.
\]
\end{theorem}
\comment{
\begin{theorem}[Error rate]\label{mainbodyfinite}
Consider $\thetab=(\what_2,\qhat_1)$ as per \sout{Algorithm \ref{eq:algo}} \eqref{eq:algo} with bias $\widehat{b}$ as explained above. Choose step sizes $\eta\propto \frac{1}{Q^2\zeta}$ and $\gamma$ large enough. Suppose $Q\gtrsim 1+W$, $\zeta\leq 0.9$. Declare $\rate_{\lin}=\zeta^2W^2 T$ and set error rate to
\[
\rate:=\red{Q^2}\wedge Q\sqrt{d}\wedge n^{1/3}\zeta^{2/3}(W/Q)^{4/3}\wedge (n/d)\rate_{\lin}.
\]
For a constant $c>0$, with probability $1-ce^{-\ordet{\rate\wedge d}}$ over the training process, the classification error {\color{blue} of the model defined by $(\thetab, \widehat{b})$} obeys
\[
\acc(f_{(\thetab,\widehat{b})})\leq ce^{-\ordet{\rate}}.
\]
\end{theorem}
}
Assuming small correlation coefficient $\rho$ and $W<Q$, we can set $\alpha=\order{1}$. Then, similar to Theorem \ref{thm:main grad pop}, prompt attention achieves a test error rate of $e^{-\order{Q^2}}$ which is a strict improvement over the linear baseline of Fact \ref{lin func fact} whenever $Q^2\gtrsim \zeta^2W^2T$. Secondly, our bound achieves a sample complexity of $n\gtrsim d(Q/\zeta W)^4$. The linear growth in $d$ is intuitive from counting degrees of freedom. Interestingly, large $Q$ does improve the test error, however, it degrades sample complexity. This is because it makes the estimation of parameters more challenging. Finally, larger $\zeta W$ improves sample complexity since $\zeta W$ (combining sparsity level and magnitude) captures the strength of the label-relevant information within relevant tokens $t\in\Rc$.

%$\rate_{\lin}$ corresponds to the linear baseline $\flin$ as it is known that (see~Fact \ref{lin func fact}) its error rate (under gaussian noise) follows $\ratl$. This rate appears in our theorem with $(n/d)\rate_{\lin}$; thus, as soon as $n\propto d$, gradient-descent can (potentially) beat the linear model. The remaining components of our \rate~are regularity conditions: Importantly, we ask for $Q$ to be large enough so that the attention weights $\phi(\X\hat{\qb}_1)$ provably select the relevant tokens and discard those irrelevant. This is analogous to its population-counterpart condition in \eqref{eq:clean noise condition}. We also need $n\gtrsim (W/Q)^4\zeta^2$ to suppress the variance due to the $\qstar$ terms during perturbation analysis of $\hat{\w}_1$. Observe that, by letting $n\rightarrow\infty$ in Theorem \ref{mainbodyfinite}, we end up with $\rate=Q(Q\wedge \sqrt{d})$ to obtain an error rate of $e^{-cQ(Q\wedge \sqrt{d})}$. This is a very distinct learning regime compared to $\flin$ and provably beats it whenever $Q(Q\wedge \sqrt{d})\geq \zeta^2W^2 T$. This conclusion is consistent with the discussion following Theorem \ref{thm:main grad pop}.

\noindent\textbf{Sharp error rates:} Finally, in Appendix \ref{sharp characterization} we provide an exact analysis of the classification error when $\qstar$ is known and only $\wstar$ is estimated from data. This analysis exactly quantifies the value of context-information and how prompt-tuning retrieves it. Specifically, we prove a sharp asymptotic error rate of $\Qc\left(\frac{e^{Q^2/4}}{\sqrt{1+\isnr{n/d}}}\cdot \sqrt{\frac{\zeta^2W^2T}{1-\zeta}}\right)$ where $\isnr{\alpha}:=\alpha^{-1}\frac{(1-\zeta)e^{-Q^2/2}}{\ratl}$, %\sout{$\Qc(\cdot)$ is the Gaussian tail function and noise is isotropic Gaussian.}
%\todoasr{Again, we may remove this to save space for camera ready.}
This uniformly (for all $Q\geq 0$ values) improves the optimal rates for (context-free) Gaussian mixture models thanks to the context information.



==> intro.tex <==
\section{Introduction}



%Large language models (LLMs) have achieved remarkable success in a wide range of natural language processing tasks, such as machine translation, language generation and question answering. One of the key techniques that have made these models so powerful is the ability to fine-tune them to specific tasks using a technique called prompt-tuning. In this method, the model learns a soft-prompt parameter from task-specific data, which guides the model's attention to the most relevant parts of the input. Despite its success, there is currently a lack of theoretical understanding of the power of prompt-tuning and the role of attention mechanisms in this process.

Transformer models have achieved remarkable success in a wide array of machine learning domains spanning language modeling, vision, and decision making. %One of the key techniques that have made transformers so powerful is their ability to adapt to multiple unseen tasks by conditioning their predictions through their inputs, a technique known as prompt-tuning 
Recently, one of the key techniques that has helped pave the way for the deployment of transformers to ever increasing application areas is their ability to adapt to multiple unseen tasks by conditioning their predictions through their inputs -- a technique known as prompt-tuning~\citep{lester2021power,li2021prefix}.
 Concretely, prompt-tuning provides a more efficient (cheaper/faster) alternative to fine-tuning the entire weights of the transformer by instead training (fewer) so-called prompt parameters that are appended on the input and can be thought of as an input interface. In fact, several recent works have demonstrated experimentally that prompt-tuning is not only more efficient, but often even becomes competitive to fine-tuning in terms of accuracy \citep{lester2021power,liu2023pre}. However, there is currently limited formal justification of such observations. This motivates the first question of this paper: 
\vspace{-3mm}
 \begin{center}
 \emph{How does prompt-tuning compare to fine-tuning in terms of  expressive power? Are there scenarios prompt-tuning outperforms fine-tuning in that regard?}
\end{center}
\vspace{-3mm}
%Intuitively, the success of prompt-tuning depends crucially on a model's ability to adapt to new tasks by conditioning its predictions through its input \cite{?}. Concretely, by its ability to train prompt parameters that can adjust the attention weights in accordance to the specific contextual information in a given new task. This high-level intuition forms the basis of the second question this paper aims to answer: \emph{How does the training of a prompt parameter enable learning new contextual information?} 
%tokens at the output
%Intuitively, the success of prompt-tuning depends crucially on a model's ability to adapt to new tasks by conditioning its predictions through prompting. 

%This high-level intuition forms the basis of the second question this paper aims to answer:\\\emph{How does optimizing the prompt parameter retrieves relevant contextual information?} 

 %by normalizing the attention weights to a similarity-based probability vector, 
 The core constituent of a transformer, and thus of prompt-tuning, is the attention mechanism. Through the attention layer, prompts get to interact with other input features, create/modify attention weights, and facilitate the model to attend on latent task-specific information. The standard attention layer relies on softmax nonlinearities. Operationally, the softmax function allows a model to selectively focus on certain parts of the input tokens when generating attention outputs. However, there is little rigorous understanding of attention-based prompt-tuning. Concretely, 
 \vspace{-3mm}
\begin{center}
\emph{What is the role of the softmax-attention in prompt-tuning in terms of optimization and generalization? How does it locate and extract relevant contextual information?}
\end{center}
\vspace{-2mm}
 
 %enable attending only on the (useful) context-relevant information of the input?} 

%optimization and generalization dynamics of prompt-tuning what is its role in the process of fine-tuning. 

%This work makes a significant step towards understanding the power of prompt-tuning and the role of attention mechanisms in this process, and provides valuable insights for future research in this area.



\noindent\textbf{Contributions.} Our contributions are as follows:
\vspace{-2mm}
\iffalse
\noindent$\bullet$~We show that a particular form of attention which we refer to as \emph{prompt-attention} naturally arises from the self-attention model with prompt-tuning\todoasr{Different from `prompt-tuning`, we are also updating $w$ in our analysis. Do we need a footnote somewhere highlighting/justifying this? Updating `w' is still cheaper compared to updating the whole model.}. We rigorously show that prompt-attention is superior compared to linear-prompt-attention baselines and also identify regimes where it is even more expressive than self-attention. This separation result  demonstrates provable scenarios where prompt-tuning can be superior to fine-tuning with self-attention. 

%\item identify advantage of prompt-attention with respect to baselines aka separation, prompt-attention can be even more expressive than self attention

%promptuning with prompt-attention can even beat fine-tunning with self attention
\noindent$\bullet$~We develop new statistical foundations for gradient-based prompt-tuning: we study the optimization and generalization dynamics of the initial trajectory of gradient descent for optimizing prompt-attention. We show the first few iterations learn the prompt and prediction head with near-optimal sample complexity while achieving high accuracy.

\noindent$\bullet$~Our results provide insights into the critical role of softmax in facilitating attention: we show how the initial trajectory of gradient descent utilizes softmax to provably attend to sparse context-relevant tokens, ignoring noisy/nuisance tokens.

\noindent$\bullet$~We also characterize the exact finite sample performance of prompt-attention assuming known prompt but unknown prediction head. This reveals the fundamental performance limits and the precise benefit of the context information.

\noindent$\bullet$~Our results allow studying various tradeoffs between different model parameters (i) the role of sparsity, i.e.,~the fraction of context-relevant tokens and (ii) the relative effects of the different constituents of context-relevant tokens.

\noindent$\bullet$~Finally, we empirically validate our theoretical insights on both synthetic contextual-mixture datasets and image-classification datasets. We compared multiple variants of prompt-tuning against standard fine-tuning on the latter. Furthermore, we highlight the role of prompt-attention in selecting relevant tokens in the image classification setting.
\fi

\begin{itemize}[leftmargin=*, itemsep=1mm, partopsep=0pt,parsep=0pt]
\item We show that a particular form of attention which we refer to as \emph{prompt-attention} naturally arises from the self-attention model with prompt-tuning.
% \todoasr{Different from `prompt-tuning`, we are also updating $w$ in our analysis. Do we need a footnote somewhere highlighting/justifying this? Updating `w' is still cheaper compared to updating the whole model.} 
We identify provable scenarios where it is more expressive than self-attention and linear-prompt-attention. \footnote{Our emphasis is on the role of attention (whether prompt- or self-). However, we analyze the general problem where attention weights are optimized jointly with the linear classifier head.} This separation result reveals insightful data models where prompt-tuning can be superior to fine-tuning with self-attention.

%more expressive than self-attention. that prompt-attention is superior compared to linear-prompt-attention baselines and also where  This separation result  demonstrates provable scenarios where prompt-tuning can be superior to fine-tuning with self-attention.

\item We develop new statistical foundations for gradient-based prompt-tuning: we study the optimization and generalization dynamics of the initial trajectory of gradient descent for optimizing prompt-attention. Concretely, we show the first few iterations learn the prompt and prediction head with near-optimal sample complexity while achieving high accuracy.

\item Our results provide insights into the critical role of softmax in facilitating attention: we show how the initial trajectory of gradient descent utilizes softmax to provably attend to sparse context-relevant tokens, ignoring noisy/nuisance tokens.

\item We also characterize the exact finite sample performance of prompt-attention assuming known prompt but unknown prediction head. This reveals the fundamental performance limits and precisely quantifies the benefits of context information.

\item Our results highlight various trade-offs among different model parameters: (i) the role of sparsity, i.e.,~the fraction of context-relevant tokens, and (ii) the relative effects of the different constituents of context-relevant tokens.

\item Finally, we empirically validate our theoretical insights on both synthetic contextual-mixture datasets and image-classification datasets. Specifically, we compare multiple variants of prompt-tuning against standard fine-tuning on the latter. Our results highlight the role of prompt-attention in selecting relevant tokens in the image classification setting.
\end{itemize}
\vspace{-2mm}

%\item Can prompt-tuning (\PT)
%beat Self-\Attn?
%\item Role of softmax in \PT
%\item Statistical analysis of \PT both population and finite-sample

\paragraph{Related works.} Attention, specifically the so-called self-\Attn, is the backbone mechanism of transformers~\citep{vaswani2017attention}. It differs from conventional models (e.g., multi-layer perceptrons and convolutional neural networks) in that it computes feature representations by globally modeling interactions between different parts of an input sequence. Despite tremendous empirical success~\citep[see, e.g.,][and references therein]{vaswani2017attention,brown2020language,saharia2022photorealistic,ramesh2022hierarchical,chatgpt,narayanan2021efficient,reed2022generalist}, the underlying mechanisms of the \Attn layer remain largely unknown: {How does it learn? What makes it better (and when) compared to conventional architectures?} \citet{Yun2020Are} show that self-attention based transformers with large enough depth are universal approximators of seq2seq functions. Focusing on the self-attention component, \citet{edelman2021inductive} show %undertakes investigation of 
%self-\Attn's approximation ability by showing that it 
that self-\Attn can efficiently represent sparse functions of its input space, while \citet{sahiner2022unraveling,ergen2022convexifying} analyze convex-relaxations of Self-\Attn, and \citet{baldi2022quarks,dong2021attention} study the expressive ability of \Attn layers.
However, these works do \emph{not} characterize the optimization and generalization dynamics of \Attn. To the best of our knowledge, the only prior works attempting this are \citet{jelassi2022vision} and \citet{ICLRsub2022}. \citet{jelassi2022vision} assume a simplified \Attn structure in which the \Attn matrix is \emph{not} directly parameterized in terms of the input sequence. Our paper also distinguishes itself from  contemporaneous work by \citet{ICLRsub2022} in several ways: (1) Unlike their data model, ours incorporates a context vector and employs a sub-Gaussian noise model instead of assuming bounded noise. (2) We provide a precise asymptotic analysis that elucidates the role of various problem parameters. (3) While \citet{ICLRsub2022} primarily focuses on vanilla self-attention, our study centers on understanding the potential benefits of prompt-tuning through prompt-attention.


% In the contemporaneous  
% work \citet{ICLRsub2022}, the authors study optimization/generalization of training a full self-attention model. Our paper differs from theirs in a variety of ways including: (1) The data model in \citet{ICLRsub2022} is different as it has no notion of context vector and the noise in the data is assumed to be bounded whereas our model captures the role of context and our noise model is sub-Gaussian. (2) Unlike \citet{ICLRsub2022}, we develop a precise asymptotic analysis that reveals the precise role of various problem parameters. (3) Different from \citet{ICLRsub2022}, which focuses on vanilla self-attention, our focus is on understanding prompt-tuning via prompt-attention and when it can potentially improve upon vanilla self-attention. 

% (which is the focus of \citet{ICLRsub2022}).



==> misc.tex <==
\section{Miscellaneous Results}
\begin{lemma}[Debiasing predictions]\label{debiasing} Suppose $\qb_1$ is such that a test example $(y,\X)$ obeys
\[
\Pro(\tn{\X^\top \phi(\X\qb_1)-(\qstar+y\wstar)}\leq \eps)\geq 1-\delta.
\]
Given a fresh dataset $\Sc=(y_i,\X_i)_{i=1}^n$, set $b=\frac{1}{n}\sum_{i=1}^n f_{\thetab}(\X_i)=\frac{1}{n}\sum_{i=1}^n \w_2^\top \vb_i$ where $\vb_i:=\X_i^\top \phi(\X_i\qb_1)$. Set the debiased classifier $f'_{\thetab}(\X)=f_{\thetab}(\X)-b$. Set $\Delta=\w_2^\top \wstar/\tn{\w_2}$. Suppose $n\geq 8\log\left(\frac{2}{\delta n}\right)$ and $\eps>0$ is such that $\eps<\Delta/4$. Then, with probability $1-2\delta n$ over $\Sc$, the test error of $f'_{\thetab}$ obeys
\[
\err(f'_{\thetab})\leq \delta.
\]
\end{lemma}
\begin{proof} %Decompose $\w_2=\alpha \wstar+\beta \qstar+\pb$ where $\pb\perp (\wstar,\qstar)$. 
First, let us prove the following intermediate statement: With probability $1-2\delta n$ over $\Sc$, for a new test sample $(y,\X)$, with probability $1-\delta$,% we have that
\begin{align}
|yf'_{\thetab}(\X)-\w_2^\top \wstar|\leq\sqrt{\frac{2\log(2/\delta n)}{n}}\cdot \w_2^\top \wstar+ 2{\eps\tn{\w_2}}.\label{debias bound}%_{\text{original perturb terms}}.
\end{align}
Based on the choice of $C$, observe that, with probability $1-n\delta$ over the dataset $(y_i,\X_i)_{i=1}^n$, for each $\vb_i$,
\[
|\w_2^\top\vb_i-\w_2^\top(\qstar+y_i\wstar)|\leq \eps\tn{\w_2}.%+\leq  \bar{\eps}:=\eps_0\eps+C(\eps_0+\eps).
\]
Set $\bar{b}=\w_2^\top\qstar$. Set $\bar{y}=|\frac{1}{n}\sum_{i=1}^n y_i|$. With probability $1-\delta n$, $\bar{y}\leq \sqrt{\frac{2\log(2/\delta n)}{n}}$. Combining, with overall probability at least $1-2\delta n$, the classifier bias obeys%outputs
\[
|b-\bar{b}|\leq \left|\w_2^\top\wstar\right| \sqrt{\frac{2\log(2/\delta n)}{n}}+\eps\tn{\w_2}.
\]
To finalize, for a new sample $(y,\X)$, with probability $1-\delta$, we have that $|\w_2^\top\vb-\w_2^\top(\qstar+y\wstar)|\leq \eps\tn{\w_2}$ where $\vb=\X^\top \phi(\X\qb_1)$. Thus, the prediction $f'(\X)=f(\X)-b$ obeys
\begin{align}\label{above debias eq}
|yf'_{\thetab}(\X)- y (f_{\thetab}(\X)-\bar{b})|\leq |b-\bar{b}|\leq\left|\w_2^\top\wstar\right| \sqrt{\frac{2\log(2/\delta n)}{n}}+\eps\tn{\w_2}.
\end{align}
To conclude with \eqref{debias bound}, note that
\[
| y (f_{\thetab}(\X)-\bar{b})-\w_2^\top\wstar|\leq \eps\tn{\w_2},
\]
and apply triangle inequality with \eqref{above debias eq}. 

To prove the statement of the theorem, note that, when $n\geq 8\log(2/\delta n)$ and $\w_2^\top \wstar> 4\eps\tn{\w_2}$, a test sample (with $\geq 1-\delta$ probability) obeys
\begin{align}
y f'_{\thetab}(\X)\geq \w_2^\top\wstar-\sqrt{\frac{2\log(2/\delta n)}{n}}\w_2^\top\wstar-2\eps\tn{\w_2}\geq 0.5\w_2^\top\wstar-2\eps\tn{\w_2}>0.
\end{align}
Thus, classifier makes the correct decision with the same probability.
%This leads to the following\[
%|yf'_{\thetab}(\X)-\underbrace{(\alpha \tn{\wstar}^2+\beta\wstar^\top\qstar)}_{\text{desired $\w_2^\top \wstar$}}|\leq\sqrt{\frac{2\log(2/\delta n)}{n}}\cdot \underbrace{\left|\alpha \tn{\wstar}^2+\beta \qstar^\top\wstar\right|}_{\text{from debiasing $\w_2^\top \qstar$}}+ 2{\eps\tn{\w_2}}%_{\text{original perturb terms}}.\]
% with probability $1-2\delta n$ over dataset, with probability $1-\delta$ over a fresh sample $yf'_{\thetab}(\X)>0$. Thus, 
\end{proof}


==> old.tex <==
\newpage
\newpage


\section{\red{EARLIER DISCUSSIONS}}

\begin{align*}
\langle \nabla\mathbb{E} \mathcal{L}(q), q-q^*\rangle \ge \alpha \|q-q^*\|_2^2%+\beta\|\nabla \mathcal{L}\|_2^2
\end{align*}
and
\begin{align*}
\|\nabla \mathcal{L}-E\big[\nabla \mathcal{L}\big]\|_2\le \delta\|q-q^*\|_2
\end{align*}

\begin{remark}
 Then,
$$
f_{(0,\wstar)}(\X)=\zeta\|\wstar\|_2^2\cdot y +(1-\zeta)\wstar^\top\qstar^\perp
$$
while 
$$
f_{(\qstar,\wstar)}(\X)= \frac{1}{\zeta e^{\|\qstar\|^2} + (1-\zeta)}\left( e^{\|\qstar\|^2} \zeta\|\wstar\|_2^2\cdot y +(1-\zeta)\wstar^\top\qstar^\perp \right).
$$

\end{remark}


At $(\qb=0, \w=0)$, the output is $f_{\thetab}(\X)|_{(\qb,\w)=(0,0)} = 0$ and the gradients:
\begin{align}
\G_\qb(0,0)&= 0 \nn
\\
\G_\w(0,0)&=\E_{y,\X}\Big[ y\X^\top\rho(0)\Big] = \rho(0)\E_{y,\X}\Big[ y\X^\top\ones\Big] 
 = \rho(0)
\zeta T \wstar
\end{align}
At $(\qb=0, \w=\wstar)$, the output is $f_{\thetab}(\X)|_{(\qb,\w)=(0,\wstar)} = \rho(0)\wstar^\top\X^\top\ones
$ 
and the gradients are as follows
\begin{align}
\G_\qb(0,\wstar)&=  \frac{1}{T}\E_{y,\X}\Big[ (y-f_{\thetab}(\X)) \X^\top \X\wstar\Big] - \frac{1}{T^2}\E_{y,\X}\Big[ (y-f_{\thetab}(\X)) \X^\top\ones \ones^\top\X\wstar\Big] 
\end{align}
(The equation above is for softmax nonlinearity.)

\begin{align}
\frac{1}{T}\E_{y,\X}\Big[ y \X^\top \X\wstar\Big] &= 
\zeta\E_{y,\X}\Big[ y (\qstar+y\wstar)(\qstar+y\wstar)^\top \wstar\Big]+(1-\zeta)\E_{y,\X}\Big[ y (\qstar^\perp)(\qstar^\perp)^\top \wstar\Big] + {\E_{y,\X}\Big[ y \wstar\Big]}\nn
\\
&= 
\zeta\E_{y,\X}\Big[ y (\qstar+y\wstar)(\qstar+y\wstar)^\top \wstar\Big] 
\\&=  
\zeta \qstar\tn{\wstar}^2 + \zeta\wstar(\qstar^\top\wstar)
\end{align}

\begin{align*}
&\frac{1}{T^2}\E_{y,\X}\Big[  (\wstar^\top\X^\top\ones) \X^\top \X\wstar\Big] = 
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=1}^\top\wstar^\top\x_t \Big) \Big(\sum_{\tau=1}^\top\x_\tau\x_\tau^\top \Big)\wstar\Big]\\
&= 
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=1}^{\zeta T}\wstar^\top(\qstar+y\wstar+\xi_t) \Big) \Big(\sum_{\tau=1}^{\zeta T}(\qstar+y\wstar+\xi_t)(\qstar+y\wstar+\xi_t)^\top \Big)\wstar\Big]
\\&+
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=\zeta T+1}^\top\wstar^\top(\qstar^\perp+\xi_t) \Big) \Big(\sum_{\tau=1}^{\zeta T}(\qstar+y\wstar+\xi_t)(\qstar+y\wstar+\xi_t)^\top \Big)\wstar\Big]
\\&+
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=\zeta T+1}^\top\wstar^\top(\qstar^\perp+\xi_t) \Big) \Big(\sum_{\tau=\zeta T+1}^{T}(\qstar^\perp+\xi_t)(\qstar^\perp+\xi_t)^\top \Big)\wstar\Big]
\\&+
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=1}^{\zeta T}\wstar^\top(\qstar+y\wstar+\xi_t) \Big)\Big(\sum_{\tau=\zeta T+1}^{T}(\qstar^\perp+\xi_t)(\qstar^\perp+\xi_t)^\top \Big)\wstar\Big]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
&= 
\frac{1}{T^2}\E_{y,\X}\Big[  \Big(\sum_{t=1}^{\zeta T}\wstar^\top(y\wstar+\xi_t) \Big) \Big(\sum_{\tau=1}^{\zeta T}(\wstar\wstar^\top+\xi_t\xi_t^\top+y\qstar\wstar^\top+y\wstar\xi_t^\top+y\wstar\xi_t^\top+y\qstar\xi_t^\top )\Big)\wstar\Big]
\end{align*}

\begin{equation}
\x_t | y = \begin{cases}
\qstar + y \wstar & \text{w.p.}~ \zeta
\\
\qb_{t,\star}^\perp & \text{w.p.}~ 1-\zeta
\end{cases}
\,+\, \xib_t,\qquad\xib_t\sim\Nn(0,\Id_d)
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage

Assume a simplified model where
\begin{align}\label{eq:primal_attn}
\fat(\X) = \ab^\top \X\w  = \w^\top \sum_{t\in[T]} \big(\ab\big)_t \x_t =   \sum_{t\in[T]} \big(\sft{\X\qb} \big)_t \w^\top\x_t,
\end{align}
i.e. the attention weights are now given by 
$
\ab = \sft{\X\qb}
$ where $\qb\in\R^d$ is the query vector indicating a direction favored by the attention model. For, $\sft$, we may consider the softmax activation $ \nicefrac{\exp(\X\qb)}{\ones^\top\exp(\X\qb)}\in\R^\top$ or a simpler ``separable" activation.

\begin{remark}
\label{rem:attn_variants}
Note that the simplified model in \eqref{eq:primal_attn} employs a single query vector $\qb$, resulting in a single `contextualized vector'
\begin{align}
h(\qb; \X) =  \ab^\top \X =  \big(\sft{\X\qb} \big)^\top\X  =  \sum_{t\in[T]} \big(\sft{\X\qb} \big)_t \x_t. 
\end{align}
One can extend this model by employing $m$ query vectors
$$
\Q = \begin{bmatrix}
\qb^\top_1
\\
\vdots
\\
\qb^\top_m
\end{bmatrix}\in\R^{m\times d}.
$$
This results in $m$ `contextualized vectors'
\begin{align}
\label{eq:multiq_attn}
h(\Q; \X) =  \A \X =  \big(\sft(\Q\X^\top) \big)\X  = \begin{bmatrix}
\big(\sft{\X\qb_1} \big)^\top\X
\\
\cdots
\\
\big(\sft{\X\qb_m} \big)^\top\X
\end{bmatrix}\in\R^{m\times d},
\end{align}
where $\A = \sft(\Q\X^\top) \in \R^{m \times T}$ denotes the attention weight matrix obtained by performing the softmax operation on each row of the matrix $\Q\X^\top$.  Setting $\Q = \X$ in \eqref{eq:multiq_attn} leads to the (vanilla) dot-product based self-attention model:
\begin{align}
h(\X; \X) = \big(\sft{\X\X^\top} \big)\X,
\end{align}
or working with $Q = \X\W_Q$ and $K = \X\W_K$ as queries and keys, respectively, gives {\color{red} [...note that these notations are slightly different from the ones used in these notes earlier...]}
\begin{align}
h(\X\W_Q; \X\W_K) = \big(\sft{\X\W_Q\W_K^\top\X^\top} \big)\X,
\end{align}
\end{remark}

\begin{remark}[Pooling]
Given a multi-output attention model (cf.~\eqref{eq:multiq_attn}), one can define a general learning model (cf.~\eqref{eq:gen_model}):
\begin{align}
\label{eq:gen_model2}
f_{\thetab}(\x) = \inp{\W}{h(\Q; \X)}.
\end{align}
Alternatively, it's a common practice in the literature to work with a pooled embedding (contextualized vector) as opposed to directly utilizing the $m$ contextualized vectors $h(\Q; \X)$. Towards this, mean-pooling is a one the most commonly used approach, where
\begin{align}
{\rm MeanPool}\big( h(\Q; \X) \big) = \frac{1}{T}\cdot\mathbf{1}^\top h(\Q; \X).
\end{align}
Now, the learning model (or scoring function) takes the following form
\begin{align}
f_{\thetab}(\x) = {\rm MeanPool}\big( h(\Q; \X) \big)\w.
\end{align}
\end{remark}

\begin{remark}
Is the following model appropriate for this setting?
\begin{align}\label{eq:simple_noise_signal_token_model_0}
\x_t = \xib_t + \begin{cases}\mub & \text{ w.p. } \zeta  \\ 0_d & \text{ w.p. } 1-\zeta \end{cases},
\qquad \xib_t\sim\Nn(0,\Id_d)
\end{align}
or even mode simplified:
\begin{align}\label{eq:simple_noise_signal_token_model}
\x_t =  \begin{cases}\mub & \text{ w.p. } \zeta  \\ \xib_t & \text{ w.p. } 1-\zeta \end{cases},
\qquad\xib_t\sim\Nn(0,\Id_d-\bar\mub\bar\mub^\top).
%\x_t = \xib_t + \delta_t\mub,
%\qquad \xib_t\sim\Nn\big(0,(1-\delta_t)\Id_d\big),\qquad \delta_t=\begin{cases}1 & \text{ w.p. } s/d  \\ 0 & \text{ w.p. } 1-s/d \end{cases}
\end{align}
Above, $\|\mub\|_2^2=S$ and $\bar\mub=\mub/\sqrt{S}.$ 
%Idea here is that $\qb$ be set to $\mub$ ends up weighting more the ``clean" data patches/tokens. Are the following reasonable label models then:
%$$
%y = \rm{sign}(\wstar^\top\mub)
%\qquad\text{or}\qquad
%y = \sum_{t\,:\, \x_t=\mub} \wstar^\top \x_t = s \wstar^\top\mub + \sum_{t} \xib_t.
%$$
%Alternatively, we could assume the planted model:
Assume
$
y=\wstar^\top\X^\top \sft{\X\qstar}$. 
In particular, set $\qstar=\mub$. Then,  
\begin{align}\label{eq:simple_noise_signal_token_model_y}
\x_t~\text{ following }~\eqref{eq:simple_noise_signal_token_model_0} \implies y=\sum_{t\in[T]}\rho_{t,\star} \wstar^\top\x_t,~\text{where}~ \rho_{t,\star}=\frac{e^{\mub^\top\x_t}}{\sum_{t\in[T]}e^{\mub^\top\x_t}}
\end{align}

\begin{align}\label{eq:simple_noise_signal_token_model_y}
\x_t~\text{ following }~\eqref{eq:simple_noise_signal_token_model_0} \implies y=\wstar^\top\Big(\sum_{t\,:\,\x_t=\mub+\xi_t} \rho_{t,\text{restricted}}  \x_t \Big),\qquad\text{where}~~\rho_{t,\text{restricted}}=\frac{e^{\mub^\top\x_t}}{\sum_{t\,:\,\x_t=\mub+\xi_t}e^{\mub^\top\x_t}}
\end{align}

and
\begin{align}\label{eq:simple_noise_signal_token_model_y}
\x_t~\text{ following }~\eqref{eq:simple_noise_signal_token_model} \implies y=\big(\frac{1}{{1+(e^S-1)\zeta}}\big)\,\wstar^\top \Big(\zeta{e^S} \mub  + \sum_{t\,:\,\x_t\neq\mub} \xib_t  \Big).
\end{align}

\textbf{Baselines:}

\begin{enumerate}
\item In this case, we should compare the attention model \eqref{eq:primal_attn} to the following bi-linear model
\begin{align}\label{eq:baseline}
f_{\text{\emph{pool}}}(\X) = \sum_{t\in[T]}\rho_t\w^\top\x_t = \w^\top\X^\top\rhob  
\end{align}
where now $\rhob\in\R^{T\times1}$ is trainable. Thus, we train $d+T$ parameters here compared to $2d$ in the simple attention model in \eqref{eq:primal_attn}. In fact, let's fix for now $\w=\w_*$ and only train $\rhob$ for the baseline $f_{\text{\emph{lin}}}$ and $\qb$ for simple attention $f_{\text{\emph{attn}}}$. 

\item 
$$f_{\text{Full-scale}}(\X)=\inp{\W}{\X}.$$


\end{enumerate}

(Note: In terms of DOF both models above have O(d) dof. )
\end{remark}

\paragraph{Gradients.} The gradient of the model with respect to the query vector is as follows:
\begin{align}
\nabla_\qb f_{\thetab}(\X) &= \sum_{t\in[T]} \partialf{\big(\sft{\X\qb} \big)_t}{\qb} \w^\top\x_t = \sum_{t\in[T]} \Big(\partialf{\sft{\X\qb}}{\qb}\Big)^\top\eb_t \w^\top\x_t,\nn\\
&= \sum_{t\in[T]} \Big(\partialf{\sft(\vb) }{\vb} \partialf{\vb}{\qb}\Big)^\top\eb_t \w^\top\x_t,\nn
\\
&= \sum_{t\in[T]} \X^\top \sftd{\X\qb} \eb_t \x_t^\top\w 
%= \sum_{t\in[T]} \w^\top \x_t \eb_t^\top\sftd(\X\qb)\, \X  =  \w^\top \sum_{t\in[T]}\x_t \eb_t^\top\sftd(\X\qb)\, \X \nn
%\\
%%\\
\\
&= \X^\top\sftd{\X\qb}\, \X \w
\end{align}
where $\sftd{\X\qb} = \diag{\ab} - \ab\ab^\top  = \diag{\sft{\X\qb}} - \sft{\X\qb}\sft{\X\qb}^\top$.

\paragraph{Loss gradients.} Suppose $\Lc_{\thetab}(\X,\y):=\frac{1}{2}\E(y-f_{\thetab}(\X))^2$. Then,
\begin{align}
-\nabla_{\qb}\Lc_{\thetab}(\X,\y) &= \E_{\X}\Big[ (y-f_{\thetab}(\X))\nabla_{\qb}f_{\thetab}(\X) \Big] \\
& \E_{\X}\Big[ (y-f_{\thetab}(\X)) \X^\top\sftd{\X\qb}\,\X \w \Big]
\end{align}
At $\qb=0$, the output is
\begin{align}
f_{\thetab}(\X)|_{\qb=0} = \frac{1}{T}\Big(\ones_T^\top\X\w\Big).
\end{align}


$$
\rho(0) = \frac{1}{T}\ones_T\qquad\text{and}\qquad\rho^\prime_0:=\rho^\prime(0) = \frac{1}{T}\Id_T- \frac{1}{T^2}\ones\ones^\top
$$

For convenience denote $y(\X):=y=\wstar^\top\X^\top \sft{\X\qstar}$. Then,

\begin{align}
&\E_\X\left[ 
y(\X) \X^\top \rho^\prime_0 \X
\right]\w = \frac{1}{T} \E_\X\left[ 
y(\X) \X^\top \X \right]\w
-\frac{1}{T^2} \E_\X\left[ 
y(\X) \X^\top\ones_T \ones_T^\top \X
\right]\w\nn
\end{align}

 Note in the above that for $\X$ zero-mean Gaussian, $T\gg d\implies \frac{1}{T}\X^\top\X\approx\Id_d$. Thus,  
$$
\E_\X\left[ 
y(\X) \X^\top \rho^\prime_0 \X
\right]\w  \approx \tr(\rho^\prime_0)\,\E_\X\left[ 
y(\X) 
\right]\w = (T-1)\E_\X\left[ 
y(\X) \right]\w$$
Instead, suppose that the feature matrix $\X$ is as in \eqref{eq:simple_noise_signal_token_model}. Then, 
\begin{align}
\frac{1}{T}\X^\top\X=\zeta\mub\mub^\top + (1-\zeta)\Xib\Xib^\top\approx \zeta\mub\mub^\top + (1-\zeta)(\Id_d-\bar\mub\bar\mub^\top) = \Id_d + (S-1)\zeta\mub\mub^\top.
\end{align}
Ignore for now the rank one component in $\rho^\prime_0$, then
\begin{align}
\E_\X\left[ 
y(\X) \X^\top \rho^\prime_0 \X
\right]\w  &\approx \E_\X\left[ 
y(\X) 
\X^\top\X\right]\w \nn
\\ &\approx \zeta(S-1)(\mub^\top\w)\E[y(\X)] \, \mub + (1-\zeta)\E[y(\X)]\w.
\end{align}


==> old_finite.tex <==
\section{OLD FINITE}
\subsection{Finishing the finite sample analysis: Third gradient step}




With the characterization of the relevant scores from Lemma \ref{putogether1} in hand we are now ready to turn our attention to the third gradient step and finish the finite sample analysis. To this aim we first formally state our finite sample result before turning our attention to its proof. {We note that Theorem \ref{mainbodyfinite} stated in the main paper follows immediately from this theorem as discussed in Appendix \ref{mainbodyprove}.} 


%Suppose $n\gtrsim \zeta^{-2}[(Q/W)^4+d/T]$.

\begin{theorem}\label{mainfinite}
Consider Algorithm \ref{eq:algo} with step size $\eta$ obeying
\begin{align*}
\eta\le& \frac{c_\eta}{\max\left(Q+W,cu_4\sigma\sqrt{\alpha \log(ndT)}\right)\max\left(Q+W,cu_4\sigma \sqrt{d}\right)\zeta}
\end{align*}
for small enough constant $c_\eta$ and with $\gamma$ sufficiently large. Furthermore, assume the sample size $n$ obeys
\begin{align*}
    \sqrt{n}&\geq u_0\cdot C_0  
    %\abs{\rho}^{-1}
    \frac{\qnorm}{\wnorm}
    \qquad\text{and}\qquad
    \sqrt{\frac{n\zeta T}{d}}\geq   u_0 \cdot C_0 %\abs{\rho}^{-1} 
    \frac{\sigma}{\wnorm}\sqrt{\zeta^{-1}-1}.
\end{align*}
for large enough constant $C_0>0$ and some $u_0>0$. For simplicity we also assume
\begin{align*}
\frac{\sigma\maxi \sigma^2}{\sqrt{T}}\maxi\frac{\sigma^3}{T} \leq \wnorm\maxi\qnorm \,.
\end{align*}
Recall \eqref{eqcomb1}, \eqref{eqcomb2} and suppose that $B(u_1)\geq 2 M(u_2,u_3)$.
Also define
\begin{align*}
\delta:=\frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-u_4d}+c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}
\end{align*}
Then, we can conclude that
\[
\err(f'_{\thetab})\leq \delta:=\frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-u_4d}+c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}
\]
holds with probability at least 
\begin{align*}
&1-2e^{cu_5^2}-(1-\zeta)Te^{-cu_4d}-\frac{nT(d+2)}{(ndT)^\alpha}-2(d+1)e^{-u_6^2}\\
&\quad\quad-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}}-c_2'n(1-\zeta)Te^{-c_2u_2^2}-c_3'dn(1-\zeta)Te^{c_3u_3^{2/3}}\\
&\quad\quad-2n\left(\frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-cu_4d}+c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}\right)\,.
\end{align*}
Above we remark that $u_7$ is free variables. Because it can be chosen arbitrarily large by picking a sufficiently large $\gamma$ and consequently, its associated failure events can be made arbitrarily small.
\end{theorem}

% \begin{lemma}\label{puttingtogether2}[Putting everything together] Consider the event $\mathcal{E}$ such that $\mathcal{E}^c$ is the union of the failure events of Lemma \ref{putogether1} associated with equations \eqref{eqcomb1} and \eqref{eqcomb2} so that 
% \begin{align*}
% \mathbb{P}\{\mathcal{E}^c\}\le 4e^{-c''u_4^2}+c' e^{cu_1^{2/3}}+c'dn(1-\zeta)Te^{cu_2^{2/3}}+c'n(1-\zeta)Te^{cu^2}
% \end{align*}
% Furthermore, assume we have
% \begin{align*}
% M:=u\cdot C\wnorm^2\qnorm\sigma  + u_2 \cdot &C_2(\wnorm+\qnorm)\sigma\poly{\sigma}\log(n) u /\sqrt{n}\\
% &\quad\le \frac{1}{2}\left(C\wnorm^2\qnorm\left((8-6\rho^2-\abs{\rho})\qnorm-57\abs{\rho}\wnorm\right) - u_1 \cdot C_1(\wnorm+\qnorm)^2\poly{\sigma}\log(n) /\sqrt{n}\right):=\frac{1}{2}B
% \end{align*}

% Then 
% \begin{align*}
% w_2^T\w_\star\ge \Delta\tn{\w_2}
% \end{align*}
% holds with 
% \begin{align*}
% \Delta=\frac{(\frac{1}{2}-\epsilon_\gamma)W^2-\left(\frac{u_5}{\sqrt{n}}+\epsilon_\gamma\right)QW\abs{\rho}-c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)W}{\frac{u_5}{\sqrt{n}}Q+\frac{3}{2}W+\left(Q+W\right)\epsilon_\gamma+c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)}
% \end{align*}
% with probability at least
% \begin{align*}
% 1-(1-\zeta)Te^{-cd}-4e^{-c''u_4^2}-c' e^{cu_1^{2/3}}-c'dn(1-\zeta)Te^{cu_2^{2/3}}-c'n(1-\zeta)Te^{cu^2}-2e^{c\widetilde{\eta}^2}-\frac{nT(d+2)}{(ndT)^\alpha}-2(d+1)e^{-u_6^2}
% \end{align*}
% \end{lemma}




\subsubsection{Proving Theorem \ref{mainbodyfinite} as a Corollary}\label{mainbodyprove}

\textbf{Setting variables in light of Theorem \ref{mainfinite}:} The log factors will be hidden under $\ordet{}$ notation. $\sigma\propto 1$ and set $\gamma$ to sufficiently large in terms of all other variables. Set $Q\gtrsim 1+W$ and $\zeta\leq 0.9$ so that $1-\zeta\gtrsim 1$. Set $\eta \propto 1/Q^2\zeta$ and $u_4\propto Q/\sqrt{d}$ and $\alpha\propto \ordet{d}$ (sufficiently large constant). $\alpha$ results in a failure rate of $1-e^{-\ordet{d}}$ however this will only appear in the probability of failure of the training (and not the classification error). In contrast, $u_4$ results in an error rate of
\[
e^{-\ordet{Q\sqrt{d}}}:=Te^{-cu_4 d}.
\]
For variables $u_1,u_3$, \eqref{eqcomb1} and \eqref{eqcomb2} yield that
\[
\eta \zeta^2 W^2Q^2\gtrsim (u_1Q^2+u_3Q)\log(n)/\sqrt{n}
\]
Now, set $u_1\propto u_3\propto \eta \sqrt{n}\zeta^2W^2/\log(n)$ and plug in $\eta$. This yields an error rate of 
\[
e^{-\ordet{n^{1/3}\zeta^{2/3}(W/Q)^{4/3}}}:=e^{-\ordet{\eta^{2/3}n^{1/3}\zeta^{4/3}W^{4/3}}}.
\]
Secondly, we satisfy the $u_2$ term in \eqref{eqcomb2} via $u_2\propto Q$ which yields another $e^{-\ordet{Q^2}}$ rate. These satisfy all conditions of Theorem \ref{mainfinite} with the exception of condition for $u_0$. To proceed, $u_0$ is chosen to be
\[
u_0^2\propto n[(W/Q)^2\wedge \zeta^2 W^2T/d],
\]
resulting in an error rate of 
\[
e^{-n[(W/Q)^2\wedge \zeta^2 W^2T/d]}.
\]
Combining these, we find
\begin{align}
\log\del&\leq -\ordet{Q(\sqrt{d}\wedge Q)\wedge n^{1/3}\zeta^{2/3}(W/Q)^{4/3}\wedge n(W/Q)^2\wedge n\zeta^2W^2 T/d}\\
&=-\ordet{Q(\sqrt{d}\wedge Q)\wedge n^{1/3}\zeta^{2/3}(W/Q)^{4/3}\wedge n\zeta^2W^2 T/d}.
\end{align}
To proceed, note that, the failure probability over the dataset is $cn\times\del+e^{-\ordet{d}}$, thus the advertised failure probability (under $\ordet{}$ which subsumes $\times n$) applies to the training process.

In contrast, recall that the linear model achieves a log-error rate of $\log\Qc(\sqrt{\zeta^2T/(1-\zeta)})\tn{\wstar}\propto -\zeta^2TW^2$.

\subsubsection{Proof of Theorem \ref{mainfinite}}\label{sec:proof of theorem finite full}
% We assume that the inequality \eqref{eq:noise separation} (stated again below) holds for all $i=1,2,\ldots,n$ samples used to estimate $w_2$ as well as for the a new test data point. That is
% \begin{align*}
% \Gamma\cdot \max_{t\in\Rcc} G_{t,i} \leq \frac{1}{2} \min                                 _{y\in\{\pm1\}} B_{y_i}:=\frac{1}{2}B.
% \end{align*}
% and
% \begin{align*}
% \Gamma\cdot \max_{t\in\Rcc} G_{t} \leq \frac{1}{2} \min                                 _{y\in\{\pm1\}} B_y:=\frac{1}{2}B.
% \end{align*}
Note that under the assumption of the theorem, Lemma \ref{putogether1} holds. For convenience we shall use the notation in that lemma. We also define 
\begin{align*}
M(u_2,u_3):=&u_2\,\eta\zeta\left(\zeta-\zeta^2\right)\wnorm^2\qnorm \,\sigma\,C  + u_3\,\sigma\, C\,\wt{c}_1\,\left(\wnorm\maxi\qnorm \right)\frac{\log(n)}{\sqrt{n}}\\
B(u_1):=&\eta\zeta
        (\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(15-8\rho^2-6\abs{\rho}\right)\qnorm - \left(210\abs{\rho}+33\right)\wnorm \right)/64
        %(\zeta-\zeta^2)\wnorm^2\qnorm\left(\left(8-6\rho^2-\abs{\rho}\right)\qnorm - 121\abs{\rho}\wnorm \right)/32\ 
        - 
        u_1\, C\,\wt{c}_1\,(\wnorm^2\maxi \qnorm^2)\frac{\log(n)}{\sqrt{n}}
        %u_1 \cdot C_1(\wnorm+\qnorm)^2\poly{\sigma}\log(n) /\sqrt{n}
\end{align*}
As per theorem assumption, note that $B\geq 2M$.

We define the events
\begin{align*}
\Ec_i:=
\left\{\max_{t\in\Rcc} r_{i,t}\leq M\right\}\cap \left\{\min_{t\in\R} r_{i,t}\ge \frac{B}{2}\right\}
\end{align*}
Also note that using the theorem assumption that $B\geq 2M$ we have
\begin{align*}
\frac{\zeta T e^{\gamma r_{i,0}}}{\zeta T e^{\gamma r_{i,0}} + \sum_{t\in\Rcc}e^{\gamma r_{i,t}}}=&\frac{1}{1 + \frac{1}{\zeta T}\sum_{t\in\Rcc}e^{\gamma \left( r_{i,t}-r_{i,0}\right)}}\\
\ge& \frac{1}{1 + \frac{1}{\zeta T}\sum_{t\in\Rcc}e^{\gamma \left(\max_{t\in\Rcc}r_{i,t}-B\right)}}\\
\ge& \frac{1}{1 + \frac{1}{\zeta T}\sum_{t\in\Rcc}e^{-\frac{\gamma}{2}B}}\\
=&\frac{1}{1 + \frac{1-\zeta}{\zeta}e^{-\frac{\gamma}{2}B}}
\end{align*}

Thus
\begin{align*}
\mathbb{1}_{\mathcal{R}_i^c}^T\phi(\X_i\qb)=&1-\frac{\zeta T e^{\gamma r_{i,0}}}{\zeta T e^{\gamma r_{i,0}} + \sum_{t\in\Rcc}e^{\gamma r_{i,t}}}\\
\le&\frac{\frac{1-\zeta}{\zeta}e^{-\frac{\gamma}{2}B}}{1 + \frac{1-\zeta}{\zeta}e^{-\frac{\gamma}{2}B}}\\
=&\frac{1-\zeta}{\zeta e^{\frac{\gamma}{2}B}+ (1-\zeta)}:=\epsilon_\gamma
\end{align*}
The latter also implies that 
\begin{align}\label{eq:softmax gamma approx}
\abs{\mathbb{1}_{\mathcal{R}_i}^T\phi(\X_i\qb)-1}=\mathbb{1}_{\mathcal{R}_i^c}^T\phi(\X_i\qb)\le \epsilon_\gamma
\end{align}
Note that
\begin{align*}
\Ghat_\w(\qb,\w):=-\nabla_{\w}\Lch_{\Dc}(\thetab) = \frac{1}{n}\sum_{i\in[n]} (y_i-f_{\thetab}(\X_i)) \X_i^\top\sft{(\X_i\qb)} .
\end{align*}
Thus
\begin{align*}
\w_2:=\Ghat_\w(\qb,\hat{\w}_1)=&\frac{1}{n}\sum_{i\in[n]} y_i \X_i^\top\sft{\X_i\qb}-\frac{1}{n}\sum_{i\in[n]}\left(\what_1^T\X_i^\top\sft{\X_i\qb}\right)\X_i^\top\sft{\X_i\qb}\\
=&\frac{1}{n}\sum_{i\in[n]} y_i\left(\qb_\star+y_i\w_\star\right)\mathbb{1}_{\mathcal{R}_i}^T\phi(\X_i\qb)+\frac{1}{n}\sum_{i\in[n]} y_i \Z_i^\top\sft{\X_i\qb}\\
&-\frac{1}{n}\sum_{i\in[n]}\left(\what_1^T\X_i^\top\sft{\X_i\qb}\right)\X_i^\top\sft{\X_i\qb}\\
=&\frac{1}{n}\sum_{i\in[n]} \left(y_i\qb_\star+\w_\star\right)+\frac{1}{n}\sum_{i\in[n]} \left(y_i\qb_\star+\w_\star\right)\left(\mathbb{1}_{\mathcal{R}_i}^T\phi(\X_i\qb)-1\right)+\frac{1}{n}\sum_{i\in[n]} y_i \Z_i^\top\sft{\X_i\qb}\\
&-\frac{1}{n}\sum_{i\in[n]}\left(\what_1^T\X_i^\top\sft{\X_i\qb}\right)\X_i^\top\sft{\X_i\qb}\\
=&\left(\frac{1}{n}\sum_{i\in[n]}y_i\right) \qb_\star+\w_\star+\frac{1}{n}\sum_{i\in[n]} \left(y_i\qb_\star+\w_\star\right)\left(\mathbb{1}_{\mathcal{R}_i}^T\phi(\X_i\qb)-1\right)+\frac{1}{n}\sum_{i\in[n]} y_i \Z_i^\top\sft{\X_i\qb}\\
&-\frac{1}{n}\sum_{i\in[n]}\left(\what_1^T\X_i^\top\sft{\X_i\qb}\right)\X_i^\top\sft{\X_i\qb}
\end{align*}
Let us focus on bounding the penultimate term in a unit norm direct $\vb$. That is 
\begin{align*}
\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}.
\end{align*}
To this aim we define the events
\begin{align*}
\mathcal{E}_{\vb,i}:=\big\{\tinf{\Z_i\vb}\le \sigma\sqrt{c\alpha \log \left(ndT\right)}\big\}\,,
\end{align*}
and focus on the truncated sum
\begin{align*}
\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}\,.
\end{align*}
To continue note that $y_i\vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}$ is a sub-Gaussian random variable as it is bounded due to the fact that
\begin{align*}
\abs{y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}}\le \tinf{\Z_i\vb}\mathbb{1}_{\mathcal{R}_i^c}^T\phi(\X_i\qb)\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}\le \sigma\sqrt{c\alpha \log(ndT)}\epsilon_\gamma
\end{align*}
Thus by concentration of sum of i.i.d. Sub-Gaussian random variables we have
\begin{align*}
\abs{\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}-\E\Big[y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}\Big]}\le cu_6 \sigma\frac{\sqrt{c\alpha \log(ndT)}\epsilon_\gamma}{\sqrt{n}}
\end{align*}
holds with probability at least $1-2e^{-u_6^2}$. Furthermore, note that by Jensen's inequalities 
\begin{align*}
\abs{\E\Big[y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}\Big]}\le \E\Big[\abs{y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}}\Big]\le \E\big[\tinf{Z_i\vb}\mathbb{1}_{\mathcal{R}_i^c}^T\phi(\X_i\qb)\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}\big]\le \sigma\sqrt{c\alpha \log(ndT)}\epsilon_\gamma
\end{align*}
Now use the fact that 
\begin{align*}
\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}=\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}\mathbb{1}_{\mathcal{E}_{\vb,i}}\mathbb{1}_{\mathcal{E}_i}
\end{align*}
holds with probability at least $1-\frac{nT}{(ndT)^\alpha}-\sum_{i=1}^n\mathbb{P}\{\mathcal{E}_{i}^c\}$. Combining this with the latter two inequalities (via the triangular inequality) we conclude that
\begin{align}
\label{tmpnoise}
\abs{\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}}\le c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)
\end{align}
holds with probability at least $1-\frac{nT}{(ndT)^\alpha}-\sum_{i=1}^n\mathbb{P}\{\mathcal{E}_{i}^c\}-2e^{-u_6^2}$. Applying the above to standard basis vectors $\eb_j\in\R^{d}, j\in[d]$ we can conclude that
\begin{align*}
\tn{\frac{1}{n}\sum_{i\in[n]} y_i \vb^T\Z_i^\top\sft{\X_i\qb}}\le c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)
\end{align*}
holds with probability at least $1-\frac{ndT}{(ndT)^\alpha}-2de^{-u_6^2}-
%\red{d}
\sum_{i=1}^n\mathbb{P}\{\mathcal{E}_{i}^c\}$.

To control the last term note that we have
\begin{align*}
\tn{\frac{1}{n}\sum_{i\in[n]}\left(\what_1^T\X_i^\top\sft{\X_i\qb}\right)\X_i^\top\sft{\X_i\qb}}\le& \frac{1}{n}\sum_{i\in[n]}\tinf{\X_i\hat{\w}_1}\left(\max_t \tn{\eb_t^T\X_i}\right)\\
\le&\max\left(\tn{\qb_\star}+\tn{\w_\star},cu_4\sigma\sqrt{\alpha \log(ndT)}\right)\max\left(\tn{\qb_\star}+\tn{\w_\star},cu_4\sigma \sqrt{d}\right)\tn{\hat{\w}_1}\\
\le&\max\left(\tn{\qb_\star}+\tn{\w_\star},cu_4\sigma\sqrt{\alpha \log(ndT)}\right)\max\left(\tn{\qb_\star}+\tn{\w_\star},cu_4\sigma \sqrt{d}\right)\frac{3}{2}\eta\zeta W\\
=&\max\left(Q+W,cu_4\sigma\sqrt{\alpha \log(ndT)}\right)\max\left(Q+W,cu_4\sigma \sqrt{d}\right)\frac{3}{2}\eta\zeta W
\end{align*}
holds with probability at least $1-\frac{nT}{(ndT)^\alpha}-(1-\zeta)Te^{-cu_4d}$ where in the penultimate line we used \eqref{eq:w1 norm diff}. Assuming 
\begin{align*}
\eta\le \frac{1}{3\max\left(Q+W,cu_4\sigma\sqrt{\alpha \log(ndT)}\right)\max\left(Q+W,cu_4\sigma \sqrt{d}\right)\zeta}
\end{align*}
the latter is less than $\frac{1}{2}W$.

Using the above together with triangular inequality on $\w_2$
\begin{align*}
\tn{\w_2}\le& \abs{\frac{1}{n}\sum_{i\in[n]}y_i}\tn{\qb_\star}+\tn{\w_\star}+\left(\tn{\qb_\star}+\tn{\w_\star}\right)\epsilon_\gamma+c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)+\frac{W}{2}\\
\le& \frac{u_5}{\sqrt{n}}\tn{\qb_\star}+\tn{\w_\star}+\left(\tn{\qb_\star}+\tn{\w_\star}\right)\epsilon_\gamma+c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)+\frac{W}{2}\\
=& \frac{u_5}{\sqrt{n}}Q+W+\left(Q+W\right)\epsilon_\gamma+c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)+\frac{W}{2}\\
\end{align*}
holds with probability at least $1-(1-\zeta)Te^{-cu_4d}-2e^{cu_5^2}-\frac{nT(d+1)}{(ndT)^\alpha}-2de^{-u_6^2}-\sum_{i=1}^n\mathbb{P}\{\mathcal{E}_{i}^c\}$.

Furthermore, using \eqref{tmpnoise} we also have
\begin{align*}
\abs{\frac{1}{n}\sum_{i\in[n]} y_i \w_\star^T\Z_i^\top\sft{\X_i\qb}}\le c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)\tn{\w_\star}
\end{align*}
with an added failure probability of $\frac{nT}{(ndT)^\alpha}+2e^{-u_6^2}$. Therefore,
\begin{align*}
\w_2^T\w_\star\ge& \tn{\w_\star}^2-\frac{u_5}{\sqrt{n}}\abs{\qb_\star^T\w_\star}-\left(\abs{\qb_\star^T\w_\star}+\tn{\w_\star}^2\right)\epsilon_\gamma-c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)\tn{\w_\star}-\frac{W^2}{2}\\
=&(\frac{1}{2}-\epsilon_\gamma)W^2-\left(\frac{u_5}{\sqrt{n}}+\epsilon_\gamma\right)QW\abs{\rho}-c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)W
\end{align*}
Combining the upper bound on $\tn{\w_2}$ and lower bound on $\w_2^T\w_\star$ we can thus conclude that
\begin{align*}
\frac{\w_2^T\w_\star}{\tn{\w_2}}=\frac{(\frac{1}{2}-\epsilon_\gamma)W^2-\left(\frac{u_5}{\sqrt{n}}+\epsilon_\gamma\right)QW\abs{\rho}-c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)W}{\frac{u_5}{\sqrt{n}}Q+\frac{3}{2}W+\left(Q+W\right)\epsilon_\gamma+c\sigma\epsilon_\gamma\sqrt{c\alpha \log(ndT)}\left(\frac{Cu_6}{\sqrt{n}}+1\right)}
\end{align*}
with probability at least 
\begin{align*}
&1-2e^{cu_5^2}-\frac{nT(d+2)}{(ndT)^\alpha}-2(d+1)e^{-u_6^2}-\sum_{i=1}^n\mathbb{P}\{\mathcal{E}_{i}^c\}\\
&\quad=1-2e^{cu_5^2}-(1-\zeta)Te^{-cu_4d}-\frac{nT(d+2)}{(ndT)^\alpha}-2(d+1)e^{-u_6^2}\\
&\quad\quad-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}}-c_0'e^{-c_0u_0^2}-c_2'n(1-\zeta)Te^{-c_2u_2^2}-c_3'dn(1-\zeta)Te^{c_3u_3^{2/3}}.
\end{align*}

Finally note that 
\begin{align*}
\tn{\X^T \phi(\X\qb)-(\qb_\star+y\w_\star)}=& \tn{(\qb_\star+y\w_\star)\left(\mathbb{1}_{\mathcal{R}}^T\phi(\X\qb)-1\right)+\Z^T\phi(\X\qb)}\\
\le&(Q+W+\max_t\tn{\z_t})\epsilon_\gamma\\
\le&(Q+W+cu_4\sigma\sqrt{d})\epsilon_\gamma:=\epsilon
\end{align*}
which holds with probability at least $1-(1-\zeta)Te^{-cu_4d}-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}}-c_0'e^{-c_0u_0^2}-c_2'(1-\zeta)Te^{-c_2u_2^2}-c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}$. 

Note that by picking 
\begin{align*}
\delta:= \frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-cu_4d}-c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_0'e^{-c_0u_0^2}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}
\end{align*}
we also automatically have $n\ge 8\log\left(\frac{2}{\delta n}\right)$. Thus by picking $\gamma$ sufficiently large the assumptions of Lemma \ref{debiasing} holds with $\delta$ and $\epsilon$ as defined above. Therefore, we can conclude that
\[
\err(f'_{\thetab})\leq \delta:=\frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-cu_4d}+c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_0'e^{-c_0u_0^2}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}
\]
holds with probability at least 
\begin{align*}
&1-2e^{cu_5^2}-(1-\zeta)Te^{-cu_4d}-\frac{nT(d+2)}{(ndT)^\alpha}-2(d+1)e^{-u_6^2}\\
&\quad\quad-c_0'e^{-c_0u_0^2}-c_1' e^{c_1u_1^{2/3}}-c_0'e^{-c_0u_0^2}-c_2'n(1-\zeta)Te^{-c_2u_2^2}-c_3'dn(1-\zeta)Te^{c_3u_3^{2/3}}\\
&\quad\quad-2n\left(\frac{2}{n}e^{-\frac{n}{8}}+(1-\zeta)Te^{-cd}+c_0'e^{-c_0u_0^2}+c_1' e^{c_1u_1^{2/3}}+c_0'e^{-c_0u_0^2}+c_2'(1-\zeta)Te^{-c_2u_2^2}+c_3'd(1-\zeta)Te^{c_3u_3^{2/3}}\right)
\end{align*}


==> related_work.tex <==
\section{Related work}
\label{sec:related_work}

Recently, \cite{jelassi2022vision} studied the ability to learn spatial structure via Transformers. They focused on data distributions where $T$ tokens/patches in each sample $\X$ can be partitioned into $L$ disjoint subsets and the true \emph{labeling function} respects this partitioning. In particular,
\begin{enumerate}
    \item $\Sc_1, \Sc_2,\ldots, \Sc_L$ are $L$ disjoint subsets such that $[T] = \bigcup_{\ell \in [L]}\Sc_{\ell}$ and $|\Sc_{\ell}| = C,~\forall \ell \in [L]$.
    \item we have $\mathbb{P}[yf^{\ast}(\X) > 0] = 1 - o(1)$\footnote{I am being imprecise here.} for a labeling function $f^{\ast}$ that satisfies
    \begin{align}
     f^{\ast}(\X) := \sum_{\ell \in [L]} \phi\big(\X_{\Sc_{\ell}}\big),
    \end{align}
    where $\phi: \R^{C \times d} \to \R$ is an arbitrary function.
\end{enumerate}
They further assume that the each only one of the $L$ subsets, namely \emph{signal set}, consistently contain the informative feature. Specifically, conditioned on the label $y$, tokens $\x_t, t \in [T]$ are distributed as follows:
\begin{equation}\label{eq:JSL22}
\x_t | y = \begin{cases}
y \wstar + \z_t & 
t\in\Sc_{\ell(\X)}
~~~~~~~~~~~~~~\text{(signal set)}
\\
\delta_t \wstar + \z_t & 
t \in [T] \backslash \Sc_{\ell(\X)}
~~~~~~~~\text{(random set)},%-\qstar\qstar^\top
\end{cases}
\end{equation}
where $z_t \sim \Nc\big(0, \sigma^2(\mathbf{I}_d - \wstar\wstar^{T})\big)$ and $\delta_t$ is a random variable that takes value in $\{-1, 0, +1\}$.
 % \sim \subg{\bSi}
 \begin{remark}
When $\delta_t := 0,~\forall~t$, the data model in \eqref{eq:JSL22} shares some similarity with that in \eqref{eq:CGMM} with $q^{\ast} = 0$. However, there is a key difference that our data model allows for different (random) signal set for each data points, whereas the data model in \eqref{eq:JSL22} restricts the signal set to be one of the $L$ sets $\Sc_1,\ldots, \Sc_L$.

Since, \cite{jelassi2022vision} only allow for $L$ signal sets, they analysed a much simpler attention mechanism, namely \emph{positional attention}, where attention weights do not depend on the value of tokens. In contrast, in our attention mechanism, the attention weight do depend of the value of $\X$.
\end{remark}

\section{Equivalence of Prompt-tuning and Primal Attention}
We can utilize our data model to understand the behavior/utility of prompt-tuning. One way we can proceed in this direction is as follows:
\begin{enumerate}
\item Assume that the original data model is as follows:
\begin{equation}
\x_t | y = \begin{cases}
\qstar + y \wstar & 
t\in\Rc
~~~~~~~~\text{(label-relevant token)}
\\
\z_t \sim \subg{\bSi}
& 
t\not\in\Rc~~~~~~~~\text{(label-\textbf{ir}relevant token)}%-\qstar\qstar^\top
\end{cases}
\end{equation}
Given $n$ samples from this data model, we learn $\hat{\qb}$ and $\hat{\w}$.
\item Subsequently, we are presented with a few-shot setting with $m$ samples $\{(\tilde{\X}^j, y^j)\}_{j \in [m]}$ generated according to the following data model:
\begin{equation}
\tilde{\x}_t | y = \begin{cases}
{\color{red}\qtar} + y \wstar & 
t\in \tilde{\Rc}
~~~~~~~~\text{(label-relevant token)}
\\
\z_t \sim \subg{\bSi}
& 
t\not\in \tilde{\Rc}~~~~~~~~\text{(label-\textbf{ir}relevant token)}%-\qstar\qstar^\top
\end{cases}
\end{equation}
The prompt tuning with the former model would require us to learn only ${\color{red}\qtar}$ by utilizing $m$ new samples and the estimate $\hat{\w}$.
\end{enumerate}

\noindent\textbf{Question.}~Since $q$ is part of the original model, is it better to characterize the above as \emph{parameter-efficient} fine-tuning which is an umbrella term for many approaches, including prompt-tuning? \\


Another possibility for the distribution of the few-shot samples is to assume that
\begin{equation}
\tilde{\x}_t | y = \begin{cases}
\qstar + y {\color{red}\wtar} & 
t\in\Rc
~~~~~~~~\text{(label-relevant token)}
\\
\z_t \sim \subg{\bSi}
& 
t\not\in\Rc~~~~~~~~\text{(label-\textbf{ir}relevant token)}.
\end{cases}
\end{equation}
This is very closely related to the fine-tuning setting considered in \cite[Section 5]{jelassi2022vision}, where original and downstream data distribution share the same signal sets $\Sc_1, \Sc_2,\ldots, \Sc_L$.

%$yhat=TF(X)$ => $yhat= TF([X, p]) \approx TF(X) + primal(X,P)$ it will be like prompt-tuning 

%self-atten(X) => self-atten(X) + primal(X,P) => prompt-tuning


    




% \vp
% Additional token that we obtain:
% \begin{align}
% [\sft{\X_{\pb}\X_{\pb}^\top}\X_{\pb}]_{1:}%-\sft{\X\X^\top}\X
% = \sft{[\tn{\pb}^2,\X\pb]}^\top\begin{bmatrix}\pb^\top\\\X\end{bmatrix}\approx \sft{[\X\pb]}^\top\X
% \end{align}

% \begin{align}
% [\sft{\X_{\pb}\X^\top}\X]_{1:}%-\sft{\X\X^\top}\X
% =\sft{[\X\pb]}^\top\X
% \end{align}

% \begin{align}
% TF(X)=<W,self-atten(X)>\rightarrow TF(X,p)=<[W,w],self-atten(X_p)>
% \end{align}

%TF(X)
%TF(X) doesn’t work well
%TF(X) + prompt-tuning(X)
%prediction(X) = TF(X) + prompt-tuning(X)

==> sharp_gradient_asymptotics.tex <==
\section{Sharp gradient asymptotics} \red{Kill for ICML}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Infinite $T$] 
Assume $\abs{\rho}<\wnorm/\qnorm$, Gaussian noise and consider the model $\thetab^\gamma=(\w_2^\gamma,\qb_1^\gamma)$ where $\qb_1^\gamma=-\gamma \nabla_{\qb}\Lch_{\Dc}(\w_1,0)$ from \eqref{step2} and $\w_2^\gamma=\G_\w(0,\qb_1^\gamma)$ for some $\gamma>0$. 

For constants $C_1,C_2$ defined in \eqref{eq:C1} and \eqref{eq:C2} and  for $y\in\{\pm1\}$, denote
\begin{subequations}
\begin{align}
B_y&:=\eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm\left(
(C_1+C_2\rho^2)\qnorm + y\rho (C_1+C_2)\wnorm
    \right)
\\
\Gamma&:=\eta\zeta(\zeta-\zeta^2)\wnorm^2\qnorm\sigma \sqrt{C_1^2+\rho^2 C_2(C_2+2C_1)}
\\
S_{*,y}&:=\zeta e^{\gamma B_y}+(1-\zeta) e^{\gamma^2\Gamma^2/2}
\\
H_*&:=\frac{C_1\sqrt{1-\rho^2}}{\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}},\qquad E_*:=\frac{C_2\rho\sqrt{1-\rho^2}}{\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}
\end{align}
\end{subequations}
With these further define constants
\begin{subequations}
\begin{align}
\cwn &:= \frac{\zeta}{2}\left(\frac{e^{\gamma B_1}}{{S_{*,1}}}+\frac{e^{\gamma B_{-1}}}{{S_{*,-1}}}\right)\wnorm + \frac{(1-\zeta)\gamma\Gamma e^{\gamma \Gamma^2/2}}{2\sqrt{1-\rho^2}}\left(S_{*,1}^{-1}-S_{*,-1}^{-1}\right) E_*  
\\
\cqn &:= \frac{\zeta}{2}\left(\frac{e^{\gamma B_1}}{{S_{*,1}}}-\frac{e^{\gamma B_{-1}}}{{S_{*,-1}}}\right)\qnorm + \frac{(1-\zeta)\gamma\Gamma e^{\gamma \Gamma^2/2}}{2\sqrt{1-\rho^2}}\left(S_{*,1}^{-1}-S_{*,-1}^{-1}\right) H_*\,.
\end{align}
\end{subequations}
Finally, define
\begin{subequations}
\begin{align}
J&:=\frac{\cqn(C_1+C_2\rho^2)+\cwn\rho(C_1+C_2)}{\sigma^2\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}
\\
M_{y}&:={\zeta e^{\gamma B_y}}\left( \cwn\left(\wnorm+y\rho\qnorm\right)+\cqn\left(\rho\wnorm+y\qnorm\right) \right) +y\,(1-\zeta)\sigma \gamma \Gamma e^{\gamma^2\Gamma^2/2}\cdot J\,{\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}  
  \\
  V_{y}&:={(1-\zeta)\sigma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}\cdot\sqrt{
e^{\gamma^2\Gamma^2/2}-J^2\,\gamma^2\Gamma^2\left(e^{\gamma^2\Gamma^2}-e^{\gamma^2\Gamma^2/2}\right)}
\end{align}    
\end{subequations}
Then, 
\begin{align}
\lim_{T\rightarrow\infty}\acc\left({f_{\thetab}(\X)}\right) = \frac{1}{2}Q\left(M_{+1}/V_{+1}\right) + \frac{1}{2}Q\left(M_{-1}/V_{-1}\right)
\end{align}
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof} 
We first calculate $\w_{2,T=\infty}.$ Recall that
\begin{align}\label{eq:w2T}
\w_{2,T}=\E\left[\zeta T a_{0,y} (\wstar+y\qstar)\right] + \sum_{t\in\Rcc}\E\left[a_{t,y} y \z_t\right].
\end{align}
First note the following concentration as $T\rightarrow\infty,$ by weak law of large numbers (WLLN)
$$
\frac{1}{T}\sum_{t\in\Rcc}e^{\gamma \Gamma G_t} \rightarrow (1-\zeta)\E\left[e^{\gamma \Gamma G_t}\right] = (1-\zeta) e^{\gamma^2\Gamma^2/2}.
$$
Thus, as $T\rightarrow\infty$:
\begin{align}\label{eq:denominator S_y limit T}
S_y/T\rightarrow \zeta e^{\gamma B_y}+(1-\zeta) e^{\gamma^2\Gamma^2/2}=:S_{*,y}
\end{align}
implying
$
\zeta Ta_{0,y} \rightarrow \alpha_{*,y}:={\zeta e^{\gamma B_y}}/{S_{*,y}},\quad y\in\{\pm 1\}.
$


From these, we can evaluate the limit of the first term in \eqref{eq:w2T}
\begin{align}\label{eq:first term w2 inf T}
\E\left[\zeta T a_{0,y} (\wstar+y\qstar)\right]\rightarrow  \frac{1}{2}\left(\alpha_{*,1}+\alpha_{*,-1}\right) \wstar + \frac{1}{2}\left(\alpha_{*,1}-\alpha_{*,-1}\right) \qstar
\end{align}

Similarly, we evaluate next the second term in \eqref{eq:w2T}. First, we decompose $\z_t$ in  along $\qstar,\wstar$ and their orthogonal complement for which  we denote $P^\perp$ its projection:
\begin{align*}
\z_t &=(\qstarnorm^T\z_t)\qstarnorm + \left((\wstarnorm-\rho\qstarnorm)^T\z_t\right)\frac{\wstarnorm-\rho\qstarnorm}{\|\wstarnorm-\rho\qstarnorm\|_2^2} + P^\perp\z_t 
\\
&=
\frac{1}{1-\rho^2}(\qstarnorm^T\z_t - \rho\wstarnorm^T\z_t)\qstarnorm + 
\frac{1}{1-\rho^2}(\wstarnorm^T\z_t - \rho\qstarnorm^T\z_t)\wstarnorm + P^\perp\z_t.    
\end{align*}
For convenience, denote 
\begin{align*}
H_t:=\frac{\qstarnorm^T\z_t - \rho\wstarnorm^T\z_t}{\sigma\sqrt{1-\rho^2}}\sim\subg{1} \nn
\qquad\text{and}\qquad
E_t:=\frac{\wstarnorm^T\z_t - \rho\qstarnorm^T\z_t}{\sigma\sqrt{1-\rho^2}}\sim\subg{1}
\end{align*}
and recall from \eqref{eq:in distribution noise tokens pop gd} that
\begin{align}\nn
G_t = \frac{C_1\qstarnorm^T\z_t+\rho C_2\wstarnorm^T\z_t}{\sigma\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}\sim\subg{1}.\end{align}
Thus, we compute for later use:
\begin{align}
    \E[G_tH_t] = \frac{C_1\sqrt{1-\rho^2}}{\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}=:H_*, \qquad\text{and}\qquad
    \E[G_tE_t] = \frac{C_2\rho\sqrt{1-\rho^2}}{\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}=:E_*
\end{align}
With this decomposition, the second term in  \eqref{eq:w2T} becomes
\begin{align}\label{eq:second term of w2 T inf}
\sum_{t\in\Rcc}\E\left[a_{t,y} y \z_t\right] =\frac{1}{\sqrt{1-\rho^2}}\sum_{t\in\Rcc}\E\left[a_{t,y} y H_t\right]\qstarnorm + 
\frac{1}{\sqrt{1-\rho^2}}\sum_{t\in\Rcc}\E\left[a_{t,y} y E_t\right]\wstarnorm + \sum_{t\in\Rcc}\underbrace{\E\left[a_{t,y} y P^\perp\z_t\right]}_{=0}.
\end{align}
The last term is zero because $P^\perp\z_t$ is by construction orthogonal to $G_t$ and zero-mean. To compute the other two terms we write $$\sum_{t\in\Rcc}a_{t,y}H_t=\frac{\left(\sum_{t\in\Rcc}e^{\gamma \Gamma G_t}H_t\right)/T}{S/T}$$
Now, as $T\rightarrow\infty$ by WLLN the denominator converges to $S_{*,y}$, while for the numerator we have by integration by parts
\begin{align}
    \frac{1}{(1-\zeta)T}
\sum_{t\in\Rcc}e^{\gamma \Gamma G_t}H_t\rightarrow\E[e^{\gamma \Gamma G_t}H_t]=\gamma \Gamma\,\E[G_tH_t]\,\E\left[e^{\gamma \Gamma G_t}\right] = \gamma \Gamma H_* e^{\gamma^2\Gamma^2/2}
\end{align}
Similarly, we can compute
\begin{align}
    \frac{1}{(1-\zeta)T}
\sum_{t\in\Rcc}e^{\gamma \Gamma G_t}E_t\rightarrow \gamma \Gamma E_* e^{\gamma^2\Gamma^2/2}
\end{align}
Thus, continuing from \eqref{eq:second term of w2 T inf}
$$
\sum_{t\in\Rcc}\E\left[a_{t,y} y \z_t\right] \rightarrow \frac{1-\zeta}{2\sqrt{1-\rho^2}}\gamma\Gamma e^{\gamma \Gamma^2/2}\left(S_{*,1}^{-1}-S_{*,-1}^{-1}\right)\left(H_*\qstarnorm + E_*\wstarnorm\right)
$$
Putting this display together with \eqref{eq:first term w2 inf T} yields as $T\rightarrow\infty$
\begin{align}\label{eq:w2 infty general}
    \w_{2,T}\rightarrow
    \frac{\zeta}{2}\left(\frac{e^{\gamma B_1}}{{S_{*,1}}}+\frac{e^{\gamma B_{-1}}}{{S_{*,-1}}}\right) \wstar + \frac{\zeta}{2}\left(\frac{e^{\gamma B_1}}{{S_{*,1}}}-\frac{e^{\gamma B_{-1}}}{{S_{*,-1}}}\right)\qstar + \frac{(1-\zeta)\gamma\Gamma e^{\gamma \Gamma^2/2}}{2\sqrt{1-\rho^2}}\left(S_{*,1}^{-1}-S_{*,-1}^{-1}\right)\left(H_*\qstarnorm + E_*\wstarnorm\right)
    =:\w_{2,\infty}
\end{align}
In the special case where $\rho=0$ recall that $B_1=B_{-1}=B$, thus also $S_{*,1}=S_{*,-1}$. Therefore, $\w_{2,\infty}$ simplifies to 
$
\w_{2,\infty} = \frac{\zeta e^{\gamma B}}{\zeta e^{\gamma B} + (1-\zeta)e^{\gamma^2\Gamma^2/2}}\wstar.
$
For convenience, express $\w_{2,\infty}$ compactly as $\w_{2,\infty}=\cwn\wstarnorm+\cqn\qstarnorm$, for constants $\cwn,\cqn$ specified by \eqref{eq:w2 infty general}. Set $\thetab=(\w_{2,\infty},\qb_1^\gamma).$ We will compute the value of the model's prediction $yf_{\thetab}(\X)$ in the limit of $T\rightarrow\infty.$
We have
\begin{align}
    yf_{\thetab}(\X) &= \frac{\zeta e^{\gamma B_y}}{(S_y/T)}\left( \cwn\left(\wnorm+y\rho\qnorm\right)+ \cqn\left(\rho\wnorm+y\qnorm\right) \right) \nn
    \\
  &\qquad+y\,\frac{1-\zeta}{(S_y/T)}\frac{1}{(1-\zeta)T}\sum_{t\in\Rcc}{e^{\gamma\Gamma G_t}}\left(\cqn\qstarnorm^T\z_t+\cwn\wstarnorm^T\z_t\right)
\end{align}


Now, we know from \eqref{eq:denominator S_y limit T} that $(S_y/T)\rightarrow S_{*,y}$.  Moreover, using the central limit theorem, we can compute the asymptotic distribution of the random variable $X:=e^{\gamma \Gamma G_t}J_t,$ where we use the shorthand 
$$
J_t:=\left(\cqn\qstarnorm^T\z_t+\cwn\wstarnorm^T\z_t\right)\big/\sigma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}\sim\subg{1}
$$
and recall
$
G_t = \left({C_1\qstarnorm^T\z_t+\rho C_2\wstarnorm^T\z_t}\right)\big/{\sigma\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}\sim\subg{1}.$ We compute the first and second moments of $X$ as follows:
\begin{align}
\E\left[X\right] &= 
\gamma \Gamma\,\E\left[G_tJ_t\right] \,\E\left[{e^{\gamma\Gamma G_t}}\right]\nn\\
&= 
\frac{\cqn(C_1+C_2\rho^2)+\cwn\rho(C_1+C_2)}{\sigma^2\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}\,\gamma \Gamma e^{\gamma^2\Gamma^2/2}\,.    
\end{align}
and
\begin{align}
\E\left[X^2\right]&=\E\left[J_t^2e^{\gamma\Gamma G_t}\right]
=\E\left[e^{\gamma\Gamma G_t}\right] + \E[J_tG_t]\,\gamma\Gamma\,\E\left[J_te^{\gamma\Gamma G_t}\right]\nn
\\
&=\left(1+\left(\E[J_tG_t]\right)^2\,\gamma^2\Gamma^2\right)e^{\gamma^2\Gamma^2/2}
\end{align}
Thus, from CLT as $T\rightarrow\infty$,
\begin{align}
\frac{1}{\sigma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}\frac{1}{(1-\zeta)T}\sum_{t\in\Rcc}{e^{\gamma\Gamma G_t}}\left(\cqn\qstarnorm^T\z_t+\cwn\wstarnorm^T\z_t\right)\sim \Nn\left(\E[X],\Var[X]\right).
\end{align}

Things put together, in the limit of $T\rightarrow\infty$ we have
\begin{align}
    yf_{\thetab}(\X) &\rightarrow \frac{\zeta e^{\gamma B_y}}{S_{*,y}}\left( \cwn\left(\wnorm+y\rho\qnorm\right)+ \cqn\left(\rho\wnorm+y\qnorm\right) \right) \nn
    \\
  &\qquad+y\,\cdot\frac{(1-\zeta)\sigma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}{S_{*,y}}\cdot\E[X]\nn
  \\
  &\qquad+y\,\cdot\frac{(1-\zeta)\sigma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}}{S_{*,y}}\cdot\sqrt{\Var[X]}\cdot G\nn,\qquad G\sim\Nn(0,1)
\end{align}

\end{proof}

% Now we work as above to study the limit of the terms in this expression. First, we know from \eqref{eq:denominator S_y limit T} that $(S_y/T)\rightarrow S_{*,y}.$ Second, setting $J_t:=\left(\cqn\qstarnorm^T\z_t+\cwn\wstarnorm^T\z_t\right)\big/\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}$, we have by the WLLN:
% \begin{align}
% \frac{1}{(1-\zeta)T}\sum_{t\in\Rcc}{e^{\gamma\Gamma G_t}}\left(\cqn\qstarnorm^T\z_t+\cwn\wstarnorm^T\z_t\right) &\rightarrow \sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}\,\E\left[{e^{\gamma\Gamma G_t}}J_t\right] \nn
% \\
% &= 
% \gamma \Gamma\sqrt{\cqn^2+\cwn^2+2\cqn\cwn\rho}\,\E\left[G_tJ_t\right] \,\E\left[{e^{\gamma\Gamma G_t}}\right]\nn\\
% &= 
% \frac{\cqn(C_1+C_2\rho^2)+\cwn\rho(C_1+C_2)}{\sigma\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}\,\gamma \Gamma e^{\gamma^2\Gamma^2/2}\,.
% \end{align}

% Put things together, we find in the limit of $T\rightarrow\infty$ that
% \begin{align}
%    yf_{\thetab}(\X) &\rightarrow \frac{\zeta e^{\gamma B_y}}{S_{*,y}}\left( \cwn\left(\wnorm+y\rho\qnorm\right)+ \cqn\left(\rho\wnorm+y\qnorm\right) \right) \nn
%     \\
%   &\qquad\qquad+\frac{\left(1-\zeta\right)}{S_{*,y}}\cdot\frac{\cqn(C_1+C_2\rho^2)+\cwn\rho(C_1+C_2)}{\sigma\sqrt{C_1^2+\rho^2C_2(C_2+2C_1)}}\cdot\gamma \Gamma e^{\gamma^2\Gamma^2/2}
% \end{align}

